Let's Share: A Game-Theoretic Framework for Resource Sharing in Mobile Edge Clouds

Mobile edge computing seeks to provide resources to different delay-sensitive applications. This is a challenging problem as an edge cloud-service provider may not have sufficient resources to satisfy all resource requests. Furthermore, allocating available resources optimally to different applications is also challenging. Resource sharing among different edge cloud-service providers can address the aforementioned limitation as certain service providers may have resources available that can be ``rented'' by other service providers. However, edge cloud service providers can have different objectives or \emph{utilities}. Therefore, there is a need for an efficient and effective mechanism to share resources among service providers, while considering the different objectives of various providers. We model resource sharing as a multi-objective optimization problem and present a solution framework based on \emph{Cooperative Game Theory} (CGT). We consider the strategy where each service provider allocates resources to its native applications first and shares the remaining resources with applications from other service providers. We prove that for a monotonic, non-decreasing utility function, the game is canonical and convex. Hence, the \emph{core} is not empty and the grand coalition is stable. We propose two algorithms \emph{Game-theoretic Pareto optimal allocation} (GPOA) and \emph{Polyandrous-Polygamous Matching based Pareto Optimal Allocation} (PPMPOA) that provide allocations from the core. Hence the obtained allocations are \emph{Pareto} optimal and the grand coalition of all the service providers is stable. Experimental results confirm that our proposed resource sharing framework improves utilities of edge cloud-service providers and application request satisfaction.

==> 01-intro.tex <==
%Over the last couple of years, the advent of novel paradigms such as Big Data, Internet of Things (IoT) and Machine Type Communications (MTC) have resulted in a wide range of services and applications. IoT and MTC intend to  connect different sensors or `things' with each other for providing better user experience resulting in generation of a large amount of data, while \emph{Big Data} deals with handling  large amount of data that is produced by various systems. Whether it is an IoT system or a Big Data system, the primary goal is to provide different services to the end users. However, all such systems and applications rely on resources such as CPU, Storage, Communication links etc.,  to work efficiently. Depending on the application, irrespective of the system in place (be it IoT or MTC etc.), the resource requirements vary. 
%Every IoT or MTC application (service) requires a particular amount of the aforementioned resources to be executed successfully. 


With the wide-scale proliferation of cloud computing, a large number of individuals and businesses have transitioned towards  the use of cloud computing platforms \cite{shi2017online}. Users (applications)\footnote{Throughout the paper, we use the term ``users'' and ``applications'' interchangeably.} request resources from a cloud service provider for a particular task and the service provider needs to provide those resources based on a \emph{Service Level Agreement} (SLA).  The goal for any service provider is to satisfy as many applications as possible by a timely provision  of resources, resulting in an increase in user satisfaction.  However, often the provider lacks sufficient available resources and thus allocation of resources to different users is not  straightforward requiring algorithms to satisfy use requests and also optimally use the limited resources. 
 %task and requires  algorithms to not only satisfy the user requests but also optimally use the limited resources.  
 \par 
Optimal allocation of resources in a cloud computing setting is a fundamental research problem \cite{xiao2013dynamic,lin2010dynamic,beloglazov2012energy}. Due to the recent advent of  paradigms such as Big Data \cite{john2014big}, Internet of Things (IoT) \cite{atzori2010internet},  and Machine to Machine (M2M) communication, the problem is further exacerbated as the demand for  limited resources has increased. Even when resources are available, allocating them optimally to different applications requires efficient algorithms and mechanisms. Hence, two fundamental problems that need to be addressed is the availability and allocation of the available resources.
\par To tackle the resource availability problem, numerous solutions have been proposed in the literature ranging from buying more resources to meet  peak demands, to creating shared resource pools among geographically co-located service providers. However,  different service providers may have different objectives and  existing resource pool based mechanisms do not take this into account. Ideally,  a resource sharing mechanism should take  objectives of different services into account, which  results in a multi-objective optimization (MOO) problem. Furthermore, while resource sharing or creation of a resource pool can tackle the resource availability problem, it does not address  resource allocation problem, i.e.,  optimally allocating the available resources to different users. Therefore, there is a need for a framework that not only ascertains resource availability by enabling resource sharing among different service providers, but also optimally allocates resources to users, while accounting for the service provider's objective. 
%Alicherry et al. \cite{alicherry2012network} present a 2-approximation algorithm for network resource allocation in a distributed cloud environment. The main objective of the system is to minimize the latency. Furthermore, they also propose a similar algorithm that selects the racks and servers where any particular VM requested by the user can be placed. Wei et al. \cite{wei2010game} propose a non-cooperative game theory based approach for resource allocation in the cloud. The objective of the algorithm is to maximize fairness among different users. They show that a Nash equilibrium is guaranteed to exist provided that the resource allocation problem has feasible solutions. Duan et al. \cite{duan2014multi} model scheduling in hybrid clouds as a sequential cooperative game. The authors proposed a storage and communication aware algorithm that jointly optimizes the execution time and economic cost of scheduling Bag-of-Tasks work flows. Shi et al. \cite{shi2018shapley} propose a Shapley value based mechanism for on demand bandwidth between data centers. They focus on network bandwidth and do not take computing and storage resources into account. Shi et al. \cite{shi2017online} also propose an online auction mechanism  for dynamically providing virtual clusters in geo-distributed clouds. However, our work in this paper differs from \cite{shi2017online,shi2018shapley,wei2010game,alicherry2012network,duan2014multi}, because we consider the multi-objective nature of the problem and allocate a  wide range of resources to different applications with the goal of maximizing the utility of service providers.%  but also  improving the user satisfaction. 
%\textbf{[Add Samiullah Khan's work and some other game theoretic work to application of game theory to cloud resource allocation particularly from this journal]}
%\par  Our approach in this paper deals with  multi-objective optimization resource allocation and sharing problem.
\par  We present a  cooperative game theory based framework that can be used for resource sharing and allocation in cloud computing. For resource availability, we allow resource sharing among different cloud service providers, while considering the objectives (utilities) of cloud service providers. Rather than consider a specific resource, % such as bandwidth \cite{shi2018shapley}, 
we consider a wide range of resources that are present across different cloud service providers.  
We show that different resource providers can benefit by creating a coalition among the clouds and then allocating them to users. We show that this coalition of resource providers is stable, where no resource provider will incur any loss (when compared with working alone) and the pay-off or utility the resource providers will obtain as part of the coalition is fair to all the resource providers. Also, we obtain a Pareto Optimal (details in Section~\ref{sec:prelim}) solution to our multi-objective resource sharing problem. 
 
%\par Such heavy reliance on resources for successfully running an application or providing a service means that there are two fundamental challenges that needs to be addressed


%\begin{itemize}
%	\item \textbf{Availability of Resources:} Resources are usually scarce, so it is not always possible to have resources available to perform a particular task or run a particular application.% It is also likely that the available resources e.g., processing power, might not be enough to perform a particular task or satisfy the needs of a particular service. 
%	\item \textbf{Resource Allocation:} Even if the resource availability issues is resolved, allocating resources for different tasks is in itself a research problem. Optimally allocating different resources to different jobs/tasks requires an efficient and effective framework. 
%\end{itemize}

%In this paper, we attempt to address the aforementioned challenges. To do so,  we propose a \emph{Cooperative Game Theory} (CGT) based resource sharing and allocation mechanism in which different entities (can be smartphones, servers or data centers) share their resources and form a coalition to satisfy the requests of different services and applications. Our CGT based framework takes into account the fact that different entities have different objectives, which is why traditional single objective optimization framework can't be used as we are dealing with a multi-objective optimization (MOO) problem. While we use IoT, MTC and Big Data as our motivating examples, our results and evaluations can be extended to resource allocation and sharing in other systems as well. 
The main contributions of this paper are:%\footnote{An earlier version of this paper has been accepted for publication in ACM Mobicom 2018 workshop}:
\begin{enumerate}
	\item We propose a cooperative game theory (CGT) based multi-objective resource sharing and allocation framework for cloud computing that guarantees \emph{Pareto} optimality and takes into account different  objectives of the service providers that share their resources.
	\item We show that the resource sharing and allocation problem can be modeled as a \emph{Canonical} game. Furthermore,  when service provider objectives are represented by monotone non-decreasing utilities, we show that our canonical game is convex. Due to the convexity of our game, the \emph{core} is non-empty and the grand coalition formed by all service providers that are geographically co-located is stable.% and the allocation decision obtained using Shapley value is fair to all service providers. 
	%and the \emph{Shapley} values in the core.  Hence, the grand coalition formed by all service providers that are geographically co-located is stable and the allocation decision obtained using Shapley value is fair to all service providers. 
\item For the case where each cloud service provider treats its own applications and applications of other service providers equally, i.e., the resources are allocated to those applications (irrespective of what cloud service provider they belong to) that cause the larger increase in the utility, we propose a computationally efficient  $\mathcal{O}(N)$ algorithm that provides an allocation from the core. 

\item For the case where each cloud service provider first allocates resources to its own applications and then shares the remaining resources with other service providers, we propose a family of computationally efficient $\mathcal{O}(N)$  algorithms that provide allocations from the core.% and is computationally more efficient than using Shapley value, i.e., we reduce the complexity from $\mathcal{O}(2^N)$ to $\mathcal{O}(N)$. 
	\item We evaluate the performance of our proposed framework through extensive experiments and show that the resource sharing improves the utility of all service providers. %it outperforms  single objective optimization frameworks in terms of the utility earned by resource owner. %Our framework also achieves a higher grand coalition utility and is more fair than using traditional MOO frameworks. 
\end{enumerate}
The paper is further structured as: %Section~\ref{sec:related} discusses some of work done in literature related to resource allocation and sharing.
  Section~\ref{sec:prelim} provides a primer on Multi-Objective Optimization (MOO), Cooperative Game theory (CGT), Canonical Games, and the Core. Section~\ref{sec:sysmodel} presents the system model used in this paper. It also presents the resource sharing and allocation optimization problem along with theoretical properties of the cooperative game used to obtain the Pareto optimal solution. Section~\ref{sec:exp_results} presents our experimental results. Section \ref{sec:related} provides a review of different solutions proposed in literature for  resource allocation  while Section~\ref{sec:conclusion} concludes the paper. 



%\subsection{Related Work}\label{sec:related}
%\input{related}

%\par The fundamental challenge is the availability of such resources. It is highly likely that a system might receive request for resources  by certain application (services) or users, which the system might not be able satisfy. Furthermore, even if the resources are available, allocating them efficiently to different users is a challenging problem in  itself. 
%have resulted in a number of useful services. While such  services certainly are useful, they give rise to a number of challenges as well as opportunities. Most of the devices that are part of IoT and MTC

%On one hand, IoT and MTC allow connecting different entities, `things' or sensors that produce a large amount of data which needs to be analyzed. On the other hand, Cloud Computing and Big data paradigm can be used to analyze large amount of data produced by the aforementioned systems. This means that IoT and MTC type systems would require computation, communication and storage resources to deal with the large amount of data that is generated. Systems such as cloud computing can be used to provide the required resources, however  there are two particular challenges that arise 


 %This coupled with the growth in the number of user devices such as smartphone requires the efficient utilization of communication, computation and storage resources. Communication, computation and storage resources are widely used by different applications around the world. From cloud computing to our smart phones, such resources are fundamental to carrying out any particular task. 

%\begin{itemize}
%	\item Availability of Resources: Resources are usually scarce, so it might not be always be possible to have resources available on the device to perform particular task. It is also likely that the available resources e.g., processing power, might not be enough to perform a particular task or satisfy the needs of a particular service. 
%	\item Resource Allocation: Even if the resource availability issues is resolved, allocating resources for different tasks is in itself a research problem. Optimally allocating different resources to different jobs/tasks requires an efficient and effective framework. 
%\end{itemize}
%Every task or job that can be assigned to a resource providing entity comes with an agreed upon \emph{Service Level Agreement} (SLA) such as specific amount of delay, packet loss, throughput etc. So when any requester asks for specific amount of resources to do a certain task, there is a chance that the resource provider might not have those resources available.  
%To illustrate this, we present an example using cloud computing paradigm. Research community has focused on providing resources to the users within the \emph{Service Level Agreement} (SLA), however it is possible that at any particular instance, the data centers might not have enough resources to respond to the requests of the users. 
%If the service provider\footnote{can be as small as a smartphone to as large as a data center} does not take any action, this will lead to greater SLA violations and customer dissatisfaction. In cloud computing setting,  techniques such as Virtual Machine (VM) migrations \cite{nanda2017tag} or allocating resources at a far-away data center or machine (belonging to the same vendor) can serve as a possible solution to such problems.  However, this can introduce overheads and result in extra delay. For any vendor A, rather than allocating resources at a far away data center (which will affect the response time), it is possible that resources belonging to any other party/vendor, say vendor B are in the nearby vicinity that  may be more efficient to use. The cooperation between two different vendors/service providers in such a scenario  to satisfy user requests and minimize SLA violation needs to be explored as a solution to tackle resource scarcity problem. Even if such cooperation is established, it introduces the problem of resource allocation to different users or jobs (services) that require resources.  Therefore, in this work we explore a Cooperative Game Theory Framework for resource sharing and  allocation among different users or jobs. While our aforementioned example is related to cloud computing system, the proposed framework is applicable to resource sharing and allocation in other domains as well including resource allocation in cellular communication, IoT and MTC, etc.  
%\par Figure shows the system of interest in this work. Every domain has a controller and consists of processing, communication and storage resources (may include other sort of resources as well). However, to the outside world, it only presents an abstraction of the resources rather than detailed information. A domain can range from a single computer to a large data center. Different domains with their controllers can negotiate and form a larger coalition with a virtual coalition controller that is responsible for resource sharing and allocation for the entire coalition. We present the details of the system model in Section \ref{sec:sysmodel}. The main contributions of this work are 

 % Before we get into details of the proposed system, we define some basic definitions
%\begin{enumerate}
%	\item Domain: A domain consists of processing, communication and storage resources. Each domain is aware of it resources. However, to the outside world, it only presents an abstraction of the resources rather than detailed information. A domain can range from a single computer to a large data center. %We assume that the resources across different computers in the data center are additive. 
%	An example of such a domain would be Amazon Inc. data center, that appears as an abstraction of the aforementioned resources and no private information is provided to the outside world. %The abstract information related to the 
%	\item Coalition/Slice: A slice/coalition consists of a combination of different domains that appear  as a single unit to the users who ask for resources. Each slice has a controller that coordinates the cooperation among different domains. The slice controller only has abstract information. All the requests from the users come to the slice that then, based on particular utility assigns resources (belonging to different domains) to the users. 
%\end{enumerate}


%Therefore, it is interesting to see  whether cooperation among different vendors or parties in such instances can be lead to an improved customer satisfaction and better resource utilization. 

%it is highly unlikely that we may always possess these resources to satisfy the application's needs. Different applications have different needs and allocating resources in such heterogeneous setting is a daunting task. Furthermore, every application has particular requirements in terms of storage, computation, communication and delay etc. Therefore, it is important to allocate resources in an optimal way so that we can response to as many user requests as possible. 


%Cloud computing allows different users to rent computing resources from different data centers. However, the ever growing reliance on technology and the widespread use of different data producing devices have challenged the existing communication infrastructure. Research community has focused on providing resources to the users within the \emph{Service Level Agreement} (SLA), however it is possible that at any particular instance, the data centers might not have enough resources to respond to the requests of the users. If no action is taken, this will lead to greater SLA violations and customer dissatisfaction. Techniques such as VM migrations or initiating instances at a different data center (belonging to the same vendor) can serve as a possible solution to such problems.  However, this can introduce overheads and result in extra delay. It is possible that resources belonging to any other party/vendor might be in the vicinity that  might be more efficient to use than using its owned resources at a far away data center. Therefore, it is interesting to see  whether cooperation among different vendors or parties in such instances can be lead to an improved customer satisfaction and better resource utilization. 


==> 02-sysmodel.tex <==
%Any entity that has specific resources such as CPU, storage and communication serve as the building block of our system as shown in Figure~\ref{fig:system_model} . We call this basic building block of our system a \emph{domain}. The domain can be as small as a sensor and as large as a data center.  Each domain has a \emph{domain controller} that is aware of all the resources available within the domain. The domain controller only communicates an abstraction of this information to the outside world and does not share the entire information\footnote{This can be due to a number of reasons including security and privacy. For example, Amazon and Dropbox can be in a coalition to satisfy their user's needs. However, they will not provide the entire information to each other.}. Different domains can be combined to form a coalition in the presence of a \emph{coalition controller}. The coalition controller can be either a separate controller or chosen from the domain controllers.  Below we model this coalition from game theory perspective.   

 \begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{figures/newDomains}
	\caption{Our system model with multiple cloud service providers}
	\protect\label{fig:system_model}
	\vspace{-0.2in}
\end{figure}


Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of all the cloud service providers that act as players in our game. % For simplicity, we drop the $P$ in $P_n$ and represent the players only with the subscript $n$. 
We assume that each player has a set of $\mathcal{K}=\{1,2,\cdots, K\}$ different types of resources such as communication, computation and storage resources.  The $n^{th}$ service provider represents its  available resources as $C^n = \{ C_1^{(n)},\cdots, C_K^{(n)}\}$. Here $C_k^{(n)}$ is the amount of resources of type $k$ available at service provider $n$. 
%All edge clouds can report their available resources  to any central entity, coalition controller \footnote{Coalition controller can be chosen from the edge clouds.},  where ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ represents the available resources $k \in \mathcal{K}$ for the player $n \in \mathcal{N}$. 
The vector $C=\{\sum_{n \in \mathcal{N}}C_{1}^{(n)}, \sum_{n \in \mathcal{N}}C_{2}^{(n)}, \cdots ,\sum_{n \in \mathcal{N}}C_{K}^{(n)}\}$ represents  all available resources at different service providers.  Each service provider $n$ has a set of  native applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$ that ask for resources. 

The set of all applications that ask for resources from the set of service providers (coalition of service providers) is given by $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset, \; \forall i \neq j,$ i.e., each application asks only  one service provider for resources. 
%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
Every player  $n \in \mathcal{N}$ has a request (requirement) matrix $R^{(n)}$.% from every player $n \in \mathcal{N}$ 
\begin{equation}
\label{eq:R_Req}
R^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{r^{(n)}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{(n)}_{{M}_n}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r^{(n)}_{11} & \cdots  &\cdots   & r^{(n)}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{(n)}_{M_{n}1}&\cdots  &\cdots   & r^{(n)}_{{M}_n{K}}
\end{smallmatrix}\Biggr]
\end{equation}
where the $i^{th}$ row corresponds to the $i^{th}$ application while  columns represent different resources, i.e., $r_{ij}^{(n)}$ is the amount of $j^{th}$ resource that application $i \in \mathcal{M}_n$ requests.
%The vector ${C}^{(n)}$ received by coalition controller shows different available resources at edge cloud $n$. 
Request matrix $R$ is an augmentation of all the request matrices (from all the service providers)  as given below. 
\begin{equation}
\label{eq:R_Reqco}
R^{}=\Biggl[\begin{smallmatrix}
\mathbf{r^{}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{}_{{M}}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r^{}_{11} & \cdots  &\cdots   & r^{}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{}_{M1}&\cdots  &\cdots   & r^{}_{{M}{K}}
\end{smallmatrix}\Biggr]
\end{equation}
where $r_{ij}$ is the amount of $j^{th}$ resource that application $i \in \mathcal{M}$ requests.
%We assume that a subset $\mathcal{N}_1 \subset \mathcal{N}$ have resource surplus, while a subset $\mathcal{{N}}_2 \subset \mathcal{N}$ has a resource deficit. Furthermore, we also assume that for any player $i \in \mathcal{{N}}_1$, $R^{(i)}> C^{(n)},\; \forall n \in \mathcal{{N}}_2$, i.e., no single player in $\mathcal{{N}}_2$ has a resource surplus that is more than the resource deficit of a player in $\mathcal{{N}}_1$. 

The resource sharing and allocation framework, based on $R$ and  $C$, has to make an allocation decision $\mathcal{X}$ that optimizes the utilities $u_n(\mathcal{X})$ of all the service providers $n \in \mathcal{N}$.  The allocation decision $\mathcal{X}$ is  a vector $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$ that indicates how much of each resource $k \in \mathcal{K}$ is allocated to application $i$ at service provider $n \in \mathcal{N}$. The matrix $X^{(n)}$ is an augmentation of different matrices $\{X_{i\in \mathcal{M}_1}^{(n)}, \cdots,X_{i\in \mathcal{M}_n}^{(n)},\cdots, X_{i\in \mathcal{M}_N}^{(n)} \}$, where $X_{i\in \mathcal{M}_j}^{(n)}$ is the allocation decision  at service provider $n$ for the applications $i$ originally belonging to service provider $j \in \mathcal{N}$ and $X_{i\in \mathcal{M}_n}^{(n)}$, $\forall j \in \mathcal{N}, j \neq n$ is the allocation decision at service provider $n$ for applications $i$ belonging to service provider $n$ i.e., the original applications of the service provider $n$. 
Mathematically, 

\begin{equation}
\label{eq:A_n}
X^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{{M}}}^{(n)}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{{M}}1}^{(n)}&\cdots  &\cdots   & x_{{{M}}{K}}^{(n)}
\end{smallmatrix}\Biggr]
\end{equation}
where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$. 


\begin{comment}
Each player has a utility function $u_n(\mathcal{X})$ that depends on the allocation decision $X$ (details for $X$ will be given later). We assume that each player has set of $\mathcal{K}=\{1,2,\cdots, K\}$ different resources such as communication, computation and storage resources. %Each player $n \in \mathcal{N}$ has complete information about its own resources $k \in \mathcal{K}$, however it reports only abstract information to a coalition controller 
All domains report their available resources  to the coalition controller where $C^{(n)}$ represent the available resources for the domain/player $n \in \mathcal{N}$. Each domain $n$ has a set of users or applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$ that ask for resources. Also $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset \; \forall i \neq j$ represents the set of all users that ask for resources from the coalition. 

%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
The coalition controller receives a matrix $R^{(n)}$ for every player $n \in \mathcal{N}$ 
	\begin{equation}
\label{eq:R_Req}
R^{(n)}=\Biggl(\begin{smallmatrix}
\mathbf{r^{(n)}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{(n)}_{{M}_n}}
\end{smallmatrix}\Biggr) = \Biggl(\begin{smallmatrix}
r^{(n)}_{11} & \cdots  &\cdots   & r^{(n)}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{(n)}_{M_{n}1}&\cdots  &\cdots   & r^{(n)}_{{M}_n{K}}
\end{smallmatrix}\Biggr)
\end{equation}
where the $i^{th}$ row corresponds to the $i^{th}$ user while  the columns represent different resources i.e., $r_{ij}$ is the amount of $j^{th}$ resource user $i \in \mathcal{M}$ requests.

The vector ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ received by coalition controller shows different available resources at domain $n$. 
The vector $C=\{\sum_{n \in \mathcal{N}}C_{1}^{(n)}, \sum_{n \in \mathcal{N}}C_{2}^{(n)}, \cdots ,\sum_{n \in \mathcal{N}}C_{K}^{(n)}\}$ consists of all the available resources at different domains. The coalition, based on $R$ and  $C$, has to make an allocation decision $\mathcal{X}$ that optimizes the utilities $u_n(\mathcal{X})$ of the domains.  The allocation decision $\mathcal{X}$ is  a vector $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$ that shows how much of each resource $k$ is allocated to user $i$ at domains $n \in \mathcal{N}$.

\begin{equation}
\label{eq:A_n}
X^{(n)}=\Biggl(\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{|\mathcal{M}|}}^{(n)}}
\end{smallmatrix}\Biggr) = \Biggl(\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{|\mathcal{M}|}1}^{(n)}&\cdots  &\cdots   & x_{{|\mathcal{M}|}{K}}^{(n)}
\end{smallmatrix}\Biggr)
\end{equation}
where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ allocated  to user $i$ at player $n$

 Since the utilities of different domains might be different (can be conflicting as well), this leads us to a multi-objective optimization (MOO) problem. Some of the assumptions in our model are given below
\subsection{Assumptions}
The assumptions made in our model are 
\begin{enumerate}
	\item The negotiation cost among different domains is negligible
	\item All the domains communicate their information to the coalition controller
	\item The coalition controller already exists% and do not discuss the selection of the coalition controller (can be explored in the future work)
	\item Resources across different domains are additive in nature i.e., if domain $X$ and $Y$ have $2$ GB RAM each, the coalition would have $4$ GB of RAM. 
	\item Each player has a single objective
	\item The objective of the coalition is a sum of the utilities of all the players with equal weight
%	\item Any new player/domain added into the coalition will have resources available
	\item All players or domains have the same number of users or jobs
\end{enumerate}
\end{comment}








==> 03-opt-problem2.tex <==
In this section, we first present the resource allocation problem for a single service provider (no resource sharing with other service providers). Then we present the MOO problem for resource sharing and allocation. %For a single domain $n \in \mathcal{N}$ (without being part of coalition), the optimization problem is given in Equation~\eqref{eq:opt_single}
For a single cloud  $n \in \mathcal{N}$ (not  part of a coalition), the allocation decision matrix $X_{SO}^{(n)}$, where $SO$ stands for single objective,  is given by: 

\begin{equation}
\label{eq:X_n}
X_{SO}^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{{M}_n}}^{(n)}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{{M}_n}1}^{(n)}&\cdots  &\cdots   & x_{{{M}_n}{K}}^{(n)}
\end{smallmatrix}\Biggr].
\end{equation}
%where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$. 



The optimization problem is: %given in Equation~\eqref{eq:opt_single}
\begin{subequations}\label{eq:opt_single}
	\begin{align}
	\max_{{X}_{SO}^{(n)}}\quad& u_n({X}_{SO}^{(n)})+ \sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}} \frac{x_{ik}^{(n)}}{r_{ik}^{(n)}} \quad \forall n \in \mathcal{N}, \label{eq:objsingle}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}_n, \label{eq:singlefirst} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq r^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecond} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}. \label{eq:singlethird} \displaybreak[2]
	\end{align}
\end{subequations}
The goal of this single objective optimization problem for every service provider is   to  maximize its utility by allocating available resources only to its own applications. $\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}} {x_{ik}^{(n)}}/{r_{ik}^{(n)}}$ captures the satisfaction of resource requests by applications.  %The first constraint \eqref{eq:singlefirst} indicates that the allocated resources to all the users $i \in \mathcal{M}_n$ cannot be more than the capacity. The second constraint \eqref{eq:singlesecond} indicates that the allocated resources cannot be more than the required resources, while the final constraint \eqref{eq:singlethird} indicates that the allocation cannot be negative.  
\par Next, we present the resource allocation problem for different service providers that share their resources with each other. In the resource sharing case,  each service provider aims to  maximize sum of utilities obtained by a) allocating resources to its native applications, i.e., $u_n({X}_{i \in \mathcal{M}_n}^{(n)})$;  b) allocating resources to  applications of other service providers, i.e.,  $u_j^n({X}_{i \in \mathcal{M}_j}^{(n)}),\; \forall j\in \mathcal{N}\backslash n$; and c) satisfying requests of applications. This leads to: 
%For the cooperative case, we aim to maximize the utility of our coalition in Equation~\eqref{eq:opt_higher}.  First constraint in Equation~\eqref{eq:obj1} indicates that the allocated resources cannot be more than the capacity. The second constraint \eqref{eq:obj2}  indicates that the allocated resources cannot be more than the required resources. The last constraint \eqref{eq:obj3}  implies that allocation decision can't be negative. 
\begin{subequations}\label{eq:opt_higher}
	\begin{align}
	\max_{\mathcal{X}}\quad&  \bigg(w_nu_n({X}_{i \in \mathcal{M}_n}^{(n)})+\zeta_{n} \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})+\nonumber \\
	&\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \mathcal{{N}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg) \quad \forall n \in \mathcal{N}, \label{eq:obj}\\ %\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in \mathcal{N},j\neq n}  u^{n}_j(\mathcal{X})\bigg) \quad \forall n \in \mathcal{N} \label{eq:obj}\\%\{u_1(\mathcal{A}),u_2(\mathcal{A}),\cdots,u_N(\mathcal{A})\} \label{eq:obj}\\%U(A)\label{eq:obj}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K},  \forall n \in \mathcal{N}, \forall i \in \mathcal{M}, \label{eq:obj1} \displaybreak[0]\\
	& \sum_{j \in \mathcal{N}}x_{ik}^{(j)} \leq r^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N},  \label{eq:obj2}\displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}. \label{eq:obj3} \displaybreak[2]
	\end{align}
\end{subequations}
The first constraint in both optimization problems, \eqref{eq:opt_single}  and \eqref{eq:opt_higher}, indicates that the allocated resources cannot be more than the capacity. The second constraint  in \eqref{eq:singlesecond} and \eqref{eq:obj2} indicates, that the allocated resources should not be more than the required resources.  The last constraint, \eqref{eq:singlethird} and \eqref{eq:obj3},  indicates that allocation decision cannot be negative. 

%The utility $u_n({X}_{i \in \mathcal{M}_n}^{(n)})$ given in \eqref{eq:obj}, that each player receives, is a payment that all users $i \in \mathcal{M}_n$  who use the resources pay the player. %Users of other domains $j \in \mathcal{N}\backslash n $ that use resources of domain $n$  will be charged at a rate that player $j$ would have charged the user $i \in \mathcal{M}_j$, had the request been fulfilled by player $j$. Hence, 
%$u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})$ is the utility that domain $n$ receives for sharing its resources with domain $j$. 
$w_n$ is the weight associated with the utility $u_n$ and $\zeta_n$ is the weight affiliated with all $u_j^n$. 
%\begin{itemize}
% so that each enclaves first facilitates its own users and then assign the remaining resource to the users of other enclaves. $w_n +w'_{n}=1$  where $w_n > w'_{n}$. E.g., $w_n=0.8$ and $w'_{n}=0.2$ would mean that each enclave has an incentive to first satisfy its own users (higher utility) and then share the excess resources for other users $j \in \mathcal{N}\backslash n $
%	\item The utility $u_n(\mathcal{X})$ in Equation~\eqref{eq:opt_higher} that each player receives can be thought of as a payment that all users $ \in \mathcal{M}_n$  who use the resources pay the player. The remaining available resources at domain $n$ 	can be used by users of other domains $j \in \mathcal{N}\backslash n $ that will be charged at a rate that player $j$ would have charged the user $i \in \mathcal{M}_j$ had the request been specified by player $j$. $u^{n}_j(\mathcal{X})$ is the utility that domain $n$ receives for sharing its resources with player $j$. There are different ways to capture this profit. However, for now, we can say that it would be equivalent to whatever domain $j$ would have earned had it satisfied the requests itself (however it can't as it does not have resources, so it borrows resources from domain $n$ and assigns all the profit it gains from the users to player $n$).
%	\item  $w_n$ is the weight assigned to the utility of player $n$. $\zeta_n$ is the weight assigned to the utility $u^{n}_j(\mathcal{X})$. 
%\end{itemize}
In this paper, we assume that utility of the service providers is a non-decreasing monotone function. %This is because in  cloud computing system,  the more the resources provided, the higher is the gain or utility for the service provider.
% It is highly unlikely that the utility of any service provider will decrease with an increase in the amount of resources allocated. 
 We also assume that a subset $\mathcal{N}_1 \subset \mathcal{N}$ of service providers has resource surplus, while a subset $\mathcal{{N}}_2 \subset \mathcal{N}$ has a resource deficit. %Furthermore, we also assume that for any player $i \in \mathcal{{N}}_1$, $R^{(i)}> C^{(n)},\; \forall n \in \mathcal{{N}}_2$, i.e., no single player in $\mathcal{{N}}_2$ has a resource surplus that is more than the resource deficit of a player in $\mathcal{{N}}_1$.  

\subsection{Game Theoretic Solution}
As mentioned earlier, %To obtain the solution for the MOO problem in \eqref{eq:opt_higher}, 
we model each cloud service provider as a player in our game to obtain the solution for the MOO problem in \eqref{eq:opt_higher}. Let $\mathcal{N}$ be the set of players that can play the resource sharing and allocation game. The \emph{value of coalition} for the game players $S \subseteq \mathcal{N}$ is given by \eqref{eq:payoff_function}, where $\mathcal{F}_S$ is the feasible set. 
% The characteristic function $v(S)$ in \eqref{eq:payoff_function} captures the \emph{value of coalition} of game players in $S \subseteq \mathcal{N}$, where $\mathcal{F}_S$ is the feasible set. 

%The characteristic function $v(S)$ in \eqref{eq:payoff_function} for our game  with feasible set $\mathcal{F}_S$, that solves  problem in~\eqref{eq:opt_higher}. 
%\begin{figure*}[!t]
%	\normalsize
\begin{align} \label{eq:payoff_function}
v({S})&=\sum_{{\substack{{n \in S}\\ {\mathcal{X} \in \mathcal{F}_S}}}}    %{\substack{\text{$n \in \mathcal{N}$} \\ \text{$C_{k}= \sum_{n \in \mathcal{N}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in \mathcal{N}$}\\ \text{$\sum_{j \in \mathcal{N}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}$}}}  
\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{\substack{j \in {S},\\j\neq n}} u^{n}_j(\mathcal{X})+\nonumber \\
&\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \mathcal{{S}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg).
\end{align}
%	\hrulefill
%	\vspace*{-4pt}
%\end{figure*}
 The payoff each player $n \in S$ receives depends on players' strategies as mentioned earlier. 



%\begin{remark}
%	The characteristic function in Equation~\eqref{eq:payoff_function} is for the grand coalition $\mathcal{N}$. For any $S \subseteq \mathcal{N}$, the characteristic function will be 
%\end{remark}

%\begin{figure*}[!t]
%	\normalsize
%\begin{align} \label{eq:payoff_s_function}
%v({S})=\sum_{\substack{\text{$n \in {S}$} \\ \text{$C_{k}= \sum_{n \in {S}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {S}$}\\ \text{$\sum_{j \in {S}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S}$}}} \bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in S,j\neq n} u^{n}_j(\mathcal{X})\bigg)
%\end{align}
%	\hrulefill
%	\vspace*{-4pt}
%\end{figure*}


\begin{theorem}
%	A Cooperative game $(\mathcal{N}, v)$ of $\mathcal{N}$ players and $v$ payoff function that can be used to solve the multi-objective optimization problem given in \eqref{eq:opt_higher}, is canonical\footnote{for monotonically non-decreasing utilities/pay-off function} with Transferable utility
Resource allocation and sharing problem (with multiple objectives) for the aforementioned system model  can be modeled as a canonical cooperative game with NTU. 
\end{theorem}
\begin{proof}
To prove this, we need to show that the characteristic function of resource sharing and allocation problem satisfies the following two conditions:
%	For a game to be canonical, we need to prove that the game  is superadditive and the payoff function is of characteristic form. 
	\begin{itemize}
		\item \textbf{Characteristic form of payoff:} As the utility function in a resource sharing and allocation problem  only relies on the service providers that are part of the coalition, the game or payoff function is of characteristic form.
		\item \textbf{Superadditivity:} %Super-additivity for TU games requires $v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset$ i.e. we have to prove that the pay-off or utility for a domain in the coalition is as good as domain working alone or in a smaller coalition. 
	%	Let $u_n(X_{SO}^{(n)})$ be the utility a player $n$ earns by allocating resources to application when it is not in a coalition with any other game player. Let $U_n(X)$\footnote{$U_n(X)=w_nu_n({X}_{i \in \mathcal{M}_n}^{(n)})+\zeta_{n} \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})$} be the utility a player earns when it is part of a larger  coalition. Due to monotonicity property of the utility functions used,  for all  players $n \in \mathcal{N}$,  $u_n(X_{SO}^{(n)})\leq u_n({X})$ as $X_{SO}^{(n)}\subset {X}$. Hence, the game is superadditive.  %This is {because $X_n^{C}$ can contain much more elements due to the increase in $C$ in the coalition} where $X_n^{C}$ and $X_n^{NC}$ are the allocation decisions in  a cooperative game  and independent setting respectively for domain $n$. 
	For any $S_1, S_2 \subseteq \mathcal{N}$ where $S_1 \cap S_2 =\emptyset$, $S_1,\; S_2 \subset (S_1 \cup S_2)$. The proof follows from definition of monotone utilities.
	%Let $S_1, S_2 \subseteq \mathcal{N}$ and $S_1 \cap S_2 =\emptyset$. Hence, $S_1,\; S_2 \subset (S_1 \cup S_2)$. The proof follows from definition of monotone utilities. 
%	\begin{equation}\label{eq:super}
%	\centering 
%	v(S_1 \cup S_2) \geq v(S_1)+v(S_2)
%	\end{equation}
	
	\end{itemize}
\end{proof}
%\vspace{-0.3in}
\begin{definition}[Convex Games]
	A coalition game is said to be convex if and only if for every player $n \in \mathcal{N}$, the marginal contribution of the player is non-decreasing W.R.T set inclusion. Mathematically, for $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash \{n\}$ 
	\begin{equation}\label{eq:convexgames}
	v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2).
	\end{equation} 
\end{definition}
%\vspace{-0.2in}
\begin{theorem}\label{thm:convex}
	Our canonical game is convex. 
\end{theorem}
\begin{proof}
	Let us consider two coalition $S_1$ and $S_2$, where $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash\{j\}$, $j \in \mathcal{N}$, and  $\mathcal{F}_{S1}$ and $\mathcal{F}_{S2}$ are the feasible sets for $S_1$ and $S_2$ respectively. We calculate $v(S_2 \cup \{j\})-v(S_1 \cup \{j\})$ in Equation \eqref{eq:convexityProof}, where $u_j^{(S_1)}$ and $u_j^{(S_2)}$ are the utilities of player $j$ in $S_1$ and $S_2$ respectively.  
	
	\begin{figure*}[!t]
		\normalsize
		\begin{align}\label{eq:convexityProof}
		& \sum_{\substack{\text{$n \in {S_2}$},\\ \text{$\mathcal{X} \in \mathcal{F}_{S2}$}}}
		\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{\substack{k \in {S_2}\cup j,\\ k\neq n}} u^{n}_k(\mathcal{X})+ \sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {{S}_2}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{\substack{n \in S_2,\\ n \neq j}} u^{j}_{n}(\mathcal{X})+\sum_{i \in \mathcal{M}_j}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {{S}_2}}x_{ik}^{(l)}}{r_{ik}^{(j)}} - \nonumber \\ 
	&	\Bigg(\sum_{\substack{\text{$n \in {S_1}$},\\ \text{$\mathcal{X} \in \mathcal{F}_{S1}$}}}
		\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{\substack{k \in {S_1}\cup j , \\k \neq n}} u^{n}_k(\mathcal{X})+\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {{S}_1}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg) + 
		  w_j u_j ^{(S_1)}(\mathcal{X}) + \zeta_j\sum_{\substack{n \in S_1,\\ n \neq j}} u^{j}_{n}(\mathcal{X})+ \sum_{i \in \mathcal{M}_j}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {{S}_1}}x_{ik}^{(l)}}{r_{ik}^{(j)}}\nonumber \Bigg)\\ 
		&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$},\\ \text{$\mathcal{X} \in \mathcal{F}_{S2}\backslash\mathcal{F}_{S1}$}}}
		\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{\substack{k \in {\{S_2 \backslash S_1\}},\\ k \neq n}} u^{n}_k(\mathcal{X})+\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {\{S_2\backslash S_1\}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}    \bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) 
		+ \zeta_j\sum_{\substack{n \in S_2,\\ n \neq j}} u^{j}_{n}(\mathcal{X}) - w_j u_j ^{(S_1)}(\mathcal{X}) -  \nonumber \\
		& \quad \zeta_j\sum_{\substack{n \in S_1, \\ n \neq j}} u^{j}_{n}(\mathcal{X})+\sum_{i \in \mathcal{M}_j}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \{S_2\backslash S_1\}}x_{ik}^{(l)}}{r_{ik}^{(j)}}\nonumber \\%-\sum_{i \in \mathcal{M}_j}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {{S}_1}}x_{ik}^{(l)}}{r_{ik}^{(j)}} \nonumber \\
		& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{\substack{n \in S_2,\\ n \neq j}} u^{j}_{n}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{\substack{n \in S_1,\\ n \neq j}} u^{j}_{n}(\mathcal{X})+\sum_{i \in \mathcal{M}_j}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \{S_2\backslash S_1\}}x_{ik}^{(l)}}{r_{ik}^{(j)}}  \nonumber \\
		& \geq v(S_2)- v(S_1)
		\end{align}
		\hrulefill
	%	\vspace*{-9pt}
	\vspace{-0.3in}
	\end{figure*}
	
	
	The last inequality in \eqref{eq:convexityProof} follows from the fact that $ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\geq 0$ (monotonicity of the utility).
\end{proof}

\begin{remark}
	The core of any convex game $(\mathcal{N},\mathcal{V})$ is non-empty and large \cite{sharkey1982cooperative}. 
\end{remark}

\begin{lemma}\label{lemma:MOOGame}
	Our canonical cooperative game $(\mathcal{N}, \mathcal{V})$ with NTU can be used to obtain the Pareto-optimal solutions for the multi-objective optimization problem given in \eqref{eq:opt_higher}.
\end{lemma}


While the existence of core, i.e., core being non-empty, guarantees the grand coalition is stable, finding a suitable allocation from the core is challenging particularly when the core is large (our game). Algorithm \ref{algo:alg1} provides an allocation from the core\footnote{Provided that the aforementioned assumptions hold.}, which we prove below after briefly discussing the algorithm. We first solve the single objective optimization problem \eqref{eq:opt_single} for all players $n \in \mathcal{N}$. We then solve the problem in \eqref{eq:opt_higher2} that provides the allocation from the core. $v(\{n\})$ in \eqref{eq:objh2} is the payoff a player $n$ receives when working alone.  Algorithm \ref{algo:alg1} requires solving $|\mathcal{{N}}|+1$ optimization problems. 


\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0%,  $ \boldsymbol{v} \leftarrow$0, $ \boldsymbol{O_2} \leftarrow$0, 
		\State \textbf{Step $2$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {v(\{n\})}\leftarrow$\texttt{Optimal objective function value in  \eqref{eq:opt_single}} 
	%		\State $ {X_{SO}^n}\leftarrow$\texttt{Optimal allocation decision from  \eqref{eq:opt_single}} 
		\EndFor
		\State \textbf{Step $3$:}   $ {\mathcal{X}}\leftarrow$\texttt{Optimal allocation decision  from  \eqref{eq:opt_higher2}} \\\quad \quad \quad \quad
		$ {\mathbf{u}(\mathcal{X})}\leftarrow$\texttt{Payoff vector from  \eqref{eq:opt_higher2}} %Solve \eqref{eq:opt_higher2}  to obtain ${X}^n$ and $v_n(\mathcal{{N}}), \forall n \in \mathcal{{N}}$       % Update $C$ and $R$ based on Step 2 \\  $\quad \quad \quad \;  C'\leftarrow$ $C_{updated}$,$\; R'\leftarrow$ $R_{updated}$
	%	\State \textbf{Step $4$:} Divide the players into two subsets $\mathcal{S}_1$ and $\mathcal{S}_2$ representing players \\ with resource deficit and resource surplus
	%	\State \textbf{Step $5$:}
	%	\For{\texttt{$n \in \mathcal{S}_1$}}
	%	\State $ {O_2^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single_j}}
	%	\State Update $C'$ and $R',\quad$ $ C'\leftarrow$ $C'$,$\; R'\leftarrow$ $R'$
	%	\EndFor
	%	\State \textbf{Step $6$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
	%	\State \textbf{Step $7$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{Game-theoretic Pareto optimal allocation }
	\label{algo:alg1}
	%\vspace{-0.5in}
\end{algorithm}

 \begin{theorem}\label{thm:alg1fromcore}
	The allocation decision obtained using Algorithm \ref{algo:alg1} lies in the core. 
\end{theorem}
\begin{proof}
	To prove the theorem, we need to show that the allocation decision obtained using Algorithm \ref{algo:alg1}:  a) is individually rational; b) is group rational; and c) no players  have the incentive to leave the grand coalition and form another sub-coalition $S \subset \mathcal{N}$. %	\indent
	\newline \indent\textbf{Individual Rationality:} For each player $n \in \mathcal{N}$, the solution obtained using \eqref{eq:opt_higher2} is individual rational due to the constraint in \eqref{eq:objh2}. 
	%	the solution $O_1^n$ obtained by solving the optimization problem in Equation \eqref{eq:opt_single} is the utility a player will obtain by working alone, i.e., it is $v\{n\}$. The value $O_2^n$ in Step 4 is either zero or positive but cannot be negative due to the nature of utility used, i.e., 
	%	\begin{align}
	%	u_n(R,\mathcal{X})&=O_1^n+O_2^n \quad \forall n \in \mathcal{N} \nonumber \\
	%	u_n(R,\mathcal{X})&\geq O_1^n \quad \forall n \in \mathcal{N}\nonumber 
	%	\end{align}
	Hence the solution obtained as a result of Algorithm \ref{algo:alg1} is individually rational.
	\newline \indent\textbf{Group Rationality:} The value of the grand coalition $v\{\mathcal{N}\}$ as per Equation \eqref{eq:objh1} is the sum of utilities of all players that they achieve from the pay-off vector  $\mathcal{V}(\mathcal{N})\subseteq \mathbb{R}^{|\mathcal{N}|}$. Hence the allocation obtained from Algorithm \ref{algo:alg1} is group rational.  %Steps 2, 4 and 5 of Algorithm \ref{algo:alg2} obtain the sum of the utilities as well. Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is group rational rational. 
	\par Furthermore, due to super-additivity of the game and monotonic non-decreasing nature of the utilities, no subgroup of players have an incentive to form a smaller coalition. Hence Algorithm \ref{algo:alg1} provides a solution from the core.  
\end{proof}

\begin{subequations}\label{eq:opt_higher2}
	\begin{align}
	\max_{\mathcal{X}}\quad& \sum_{n \in \mathcal{{N}}} \bigg(w_nu_n({X}_{i \in \mathcal{M}_n}^{(n)})+\zeta_{n} \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})+\nonumber \\
	&\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \mathcal{{N}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg),\label{eq:objh1}\\ 
	\text{s.t.}\quad & \texttt{constraints in \eqref{eq:obj1}-\eqref{eq:obj3}},  \nonumber \\
& \bigg(w_nu_n({X}_{i \in \mathcal{M}_n}^{(n)})+\zeta_{n} \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})+\nonumber \\
&\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \mathcal{{N}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg) \geq  {v(\{n\})}, \forall n \in \mathcal{N}\label{eq:objh2}. 
%&   \texttt{ \eqref{eq:objh1} $\geq$  \eqref{eq:objsingle}}, \forall n \in \mathcal{N}.
	\end{align}
\end{subequations}


 

In the next section, we evaluate the performance of our resource sharing and allocation framework. 


==> strategy-2 arxiv/01-intro.tex <==
%Over the last couple of years, the advent of novel paradigms such as Big Data, Internet of Things (IoT) and Machine Type Communications (MTC) have resulted in a wide range of services and applications. IoT and MTC intend to  connect different sensors or `things' with each other for providing better user experience resulting in generation of a large amount of data, while \emph{Big Data} deals with handling  large amount of data that is produced by various systems. Whether it is an IoT system or a Big Data system, the primary goal is to provide different services to the end users. However, all such systems and applications rely on resources such as CPU, Storage, Communication links etc.,  to work efficiently. Depending on the application, irrespective of the system in place (be it IoT or MTC etc.), the resource requirements vary. 
%Every IoT or MTC application (service) requires a particular amount of the aforementioned resources to be executed successfully. 


With the wide-scale proliferation of cloud computing, a large number of individuals and businesses have transitioned towards  the use of cloud computing platforms \cite{shi2017online}. Users (applications)\footnote{Throughout the paper, we use the term ``users'' and ``applications'' interchangeably.} request resources from a cloud service provider for a particular task and the service provider needs to provide those resources based on a \emph{Service Level Agreement} (SLA).  The goal for any service provider is to satisfy as many applications as possible by a timely provision  of resources, resulting in an increase in user satisfaction.  However, often the provider lacks sufficient available resources and thus allocation of resources to different users is not  straightforward requiring algorithms to satisfy use requests and also optimally use the limited resources. 
 %task and requires  algorithms to not only satisfy the user requests but also optimally use the limited resources.  
 \par 
Optimal allocation of resources in a cloud computing setting is a fundamental research problem \cite{xiao2013dynamic,lin2010dynamic,beloglazov2012energy}. Due to the recent advent of  paradigms such as Big Data \cite{john2014big}, Internet of Things (IoT) \cite{atzori2010internet},  and Machine to Machine (M2M) communication, the problem is further exacerbated as the demand for  limited resources has increased. Even when resources are available, allocating them optimally to different applications requires efficient algorithms and mechanisms. Hence, two fundamental problems that need to be addressed is the availability and allocation of the available resources.
\par To tackle the resource availability problem, numerous solutions have been proposed in the literature ranging from buying more resources to meet  peak demands, to creating shared resource pools among geographically co-located service providers. However,  different service providers may have different objectives and  existing resource pool based mechanisms do not take this into account. Ideally,  a resource sharing mechanism should take  objectives of different services into account, which  results in a multi-objective optimization (MOO) problem. Furthermore, while resource sharing or creation of a resource pool can tackle the resource availability problem, it does not address  resource allocation problem, i.e.,  optimally allocating the available resources to different users. Therefore, there is a need for a framework that not only ascertains resource availability by enabling resource sharing among different service providers, but also optimally allocates resources to users, while accounting for the service provider's objective. 
%Alicherry et al. \cite{alicherry2012network} present a 2-approximation algorithm for network resource allocation in a distributed cloud environment. The main objective of the system is to minimize the latency. Furthermore, they also propose a similar algorithm that selects the racks and servers where any particular VM requested by the user can be placed. Wei et al. \cite{wei2010game} propose a non-cooperative game theory based approach for resource allocation in the cloud. The objective of the algorithm is to maximize fairness among different users. They show that a Nash equilibrium is guaranteed to exist provided that the resource allocation problem has feasible solutions. Duan et al. \cite{duan2014multi} model scheduling in hybrid clouds as a sequential cooperative game. The authors proposed a storage and communication aware algorithm that jointly optimizes the execution time and economic cost of scheduling Bag-of-Tasks work flows. Shi et al. \cite{shi2018shapley} propose a Shapley value based mechanism for on demand bandwidth between data centers. They focus on network bandwidth and do not take computing and storage resources into account. Shi et al. \cite{shi2017online} also propose an online auction mechanism  for dynamically providing virtual clusters in geo-distributed clouds. However, our work in this paper differs from \cite{shi2017online,shi2018shapley,wei2010game,alicherry2012network,duan2014multi}, because we consider the multi-objective nature of the problem and allocate a  wide range of resources to different applications with the goal of maximizing the utility of service providers.%  but also  improving the user satisfaction. 
%\textbf{[Add Samiullah Khan's work and some other game theoretic work to application of game theory to cloud resource allocation particularly from this journal]}
%\par  Our approach in this paper deals with  multi-objective optimization resource allocation and sharing problem.
\par  We present a  cooperative game theory based framework that can be used for resource sharing and allocation in cloud computing. For resource availability, we allow resource sharing among different cloud service providers, while considering the objectives (utilities) of cloud service providers. Rather than consider a specific resource, % such as bandwidth \cite{shi2018shapley}, 
we consider a wide range of resources that are present across different cloud service providers.  
We show that different resource providers can benefit by creating a coalition among the clouds and then allocating them to users. We show that this coalition of resource providers is stable, where no resource provider will incur any loss (when compared with working alone) and the pay-off or utility the resource providers will obtain as part of the coalition is fair to all the resource providers. Also, we obtain a Pareto Optimal (details in Section~\ref{sec:prelim}) solution to our multi-objective resource sharing problem. 
 
%\par Such heavy reliance on resources for successfully running an application or providing a service means that there are two fundamental challenges that needs to be addressed


%\begin{itemize}
%	\item \textbf{Availability of Resources:} Resources are usually scarce, so it is not always possible to have resources available to perform a particular task or run a particular application.% It is also likely that the available resources e.g., processing power, might not be enough to perform a particular task or satisfy the needs of a particular service. 
%	\item \textbf{Resource Allocation:} Even if the resource availability issues is resolved, allocating resources for different tasks is in itself a research problem. Optimally allocating different resources to different jobs/tasks requires an efficient and effective framework. 
%\end{itemize}

%In this paper, we attempt to address the aforementioned challenges. To do so,  we propose a \emph{Cooperative Game Theory} (CGT) based resource sharing and allocation mechanism in which different entities (can be smartphones, servers or data centers) share their resources and form a coalition to satisfy the requests of different services and applications. Our CGT based framework takes into account the fact that different entities have different objectives, which is why traditional single objective optimization framework can't be used as we are dealing with a multi-objective optimization (MOO) problem. While we use IoT, MTC and Big Data as our motivating examples, our results and evaluations can be extended to resource allocation and sharing in other systems as well. 
The main contributions of this paper are:%\footnote{An earlier version of this paper has been accepted for publication in ACM Mobicom 2018 workshop}:
\begin{enumerate}
	\item We propose a cooperative game theory (CGT) based multi-objective resource sharing and allocation framework for cloud computing that guarantees \emph{Pareto} optimality and takes into account different  objectives of the service providers that share their resources.
	\item We show that the resource sharing and allocation problem can be modeled as a \emph{Canonical} game. Furthermore,  when service provider objectives are represented by monotone non-decreasing utilities, we show that our canonical game is convex. Due to the convexity of our game, the \emph{core} is non-empty and the grand coalition formed by all service providers that are geographically co-located is stable.% and the allocation decision obtained using Shapley value is fair to all service providers. 
	%and the \emph{Shapley} values in the core.  Hence, the grand coalition formed by all service providers that are geographically co-located is stable and the allocation decision obtained using Shapley value is fair to all service providers. 
\item For the case where each cloud service provider treats its own applications and applications of other service providers equally, i.e., the resources are allocated to those applications (irrespective of what cloud service provider they belong to) that cause the larger increase in the utility, we propose a computationally efficient  $\mathcal{O}(N)$ algorithm that provides an allocation from the core. 

\item For the case where each cloud service provider first allocates resources to its own applications and then shares the remaining resources with other service providers, we propose a family of computationally efficient $\mathcal{O}(N)$  algorithms that provide allocations from the core.% and is computationally more efficient than using Shapley value, i.e., we reduce the complexity from $\mathcal{O}(2^N)$ to $\mathcal{O}(N)$. 
	\item We evaluate the performance of our proposed framework through extensive experiments and show that the resource sharing improves the utility of all service providers. %it outperforms  single objective optimization frameworks in terms of the utility earned by resource owner. %Our framework also achieves a higher grand coalition utility and is more fair than using traditional MOO frameworks. 
\end{enumerate}
The paper is further structured as: %Section~\ref{sec:related} discusses some of work done in literature related to resource allocation and sharing.
  Section~\ref{sec:prelim} provides a primer on Multi-Objective Optimization (MOO), Cooperative Game theory (CGT), Canonical Games, and the Core. Section~\ref{sec:sysmodel} presents the system model used in this paper. It also presents the resource sharing and allocation optimization problem along with theoretical properties of the cooperative game used to obtain the Pareto optimal solution. Section~\ref{sec:exp_results} presents our experimental results. Section \ref{sec:related} provides a review of different solutions proposed in literature for  resource allocation  while Section~\ref{sec:conclusion} concludes the paper. 



%\subsection{Related Work}\label{sec:related}
%\input{related}

%\par The fundamental challenge is the availability of such resources. It is highly likely that a system might receive request for resources  by certain application (services) or users, which the system might not be able satisfy. Furthermore, even if the resources are available, allocating them efficiently to different users is a challenging problem in  itself. 
%have resulted in a number of useful services. While such  services certainly are useful, they give rise to a number of challenges as well as opportunities. Most of the devices that are part of IoT and MTC

%On one hand, IoT and MTC allow connecting different entities, `things' or sensors that produce a large amount of data which needs to be analyzed. On the other hand, Cloud Computing and Big data paradigm can be used to analyze large amount of data produced by the aforementioned systems. This means that IoT and MTC type systems would require computation, communication and storage resources to deal with the large amount of data that is generated. Systems such as cloud computing can be used to provide the required resources, however  there are two particular challenges that arise 


 %This coupled with the growth in the number of user devices such as smartphone requires the efficient utilization of communication, computation and storage resources. Communication, computation and storage resources are widely used by different applications around the world. From cloud computing to our smart phones, such resources are fundamental to carrying out any particular task. 

%\begin{itemize}
%	\item Availability of Resources: Resources are usually scarce, so it might not be always be possible to have resources available on the device to perform particular task. It is also likely that the available resources e.g., processing power, might not be enough to perform a particular task or satisfy the needs of a particular service. 
%	\item Resource Allocation: Even if the resource availability issues is resolved, allocating resources for different tasks is in itself a research problem. Optimally allocating different resources to different jobs/tasks requires an efficient and effective framework. 
%\end{itemize}
%Every task or job that can be assigned to a resource providing entity comes with an agreed upon \emph{Service Level Agreement} (SLA) such as specific amount of delay, packet loss, throughput etc. So when any requester asks for specific amount of resources to do a certain task, there is a chance that the resource provider might not have those resources available.  
%To illustrate this, we present an example using cloud computing paradigm. Research community has focused on providing resources to the users within the \emph{Service Level Agreement} (SLA), however it is possible that at any particular instance, the data centers might not have enough resources to respond to the requests of the users. 
%If the service provider\footnote{can be as small as a smartphone to as large as a data center} does not take any action, this will lead to greater SLA violations and customer dissatisfaction. In cloud computing setting,  techniques such as Virtual Machine (VM) migrations \cite{nanda2017tag} or allocating resources at a far-away data center or machine (belonging to the same vendor) can serve as a possible solution to such problems.  However, this can introduce overheads and result in extra delay. For any vendor A, rather than allocating resources at a far away data center (which will affect the response time), it is possible that resources belonging to any other party/vendor, say vendor B are in the nearby vicinity that  may be more efficient to use. The cooperation between two different vendors/service providers in such a scenario  to satisfy user requests and minimize SLA violation needs to be explored as a solution to tackle resource scarcity problem. Even if such cooperation is established, it introduces the problem of resource allocation to different users or jobs (services) that require resources.  Therefore, in this work we explore a Cooperative Game Theory Framework for resource sharing and  allocation among different users or jobs. While our aforementioned example is related to cloud computing system, the proposed framework is applicable to resource sharing and allocation in other domains as well including resource allocation in cellular communication, IoT and MTC, etc.  
%\par Figure shows the system of interest in this work. Every domain has a controller and consists of processing, communication and storage resources (may include other sort of resources as well). However, to the outside world, it only presents an abstraction of the resources rather than detailed information. A domain can range from a single computer to a large data center. Different domains with their controllers can negotiate and form a larger coalition with a virtual coalition controller that is responsible for resource sharing and allocation for the entire coalition. We present the details of the system model in Section \ref{sec:sysmodel}. The main contributions of this work are 

 % Before we get into details of the proposed system, we define some basic definitions
%\begin{enumerate}
%	\item Domain: A domain consists of processing, communication and storage resources. Each domain is aware of it resources. However, to the outside world, it only presents an abstraction of the resources rather than detailed information. A domain can range from a single computer to a large data center. %We assume that the resources across different computers in the data center are additive. 
%	An example of such a domain would be Amazon Inc. data center, that appears as an abstraction of the aforementioned resources and no private information is provided to the outside world. %The abstract information related to the 
%	\item Coalition/Slice: A slice/coalition consists of a combination of different domains that appear  as a single unit to the users who ask for resources. Each slice has a controller that coordinates the cooperation among different domains. The slice controller only has abstract information. All the requests from the users come to the slice that then, based on particular utility assigns resources (belonging to different domains) to the users. 
%\end{enumerate}


%Therefore, it is interesting to see  whether cooperation among different vendors or parties in such instances can be lead to an improved customer satisfaction and better resource utilization. 

%it is highly unlikely that we may always possess these resources to satisfy the application's needs. Different applications have different needs and allocating resources in such heterogeneous setting is a daunting task. Furthermore, every application has particular requirements in terms of storage, computation, communication and delay etc. Therefore, it is important to allocate resources in an optimal way so that we can response to as many user requests as possible. 


%Cloud computing allows different users to rent computing resources from different data centers. However, the ever growing reliance on technology and the widespread use of different data producing devices have challenged the existing communication infrastructure. Research community has focused on providing resources to the users within the \emph{Service Level Agreement} (SLA), however it is possible that at any particular instance, the data centers might not have enough resources to respond to the requests of the users. If no action is taken, this will lead to greater SLA violations and customer dissatisfaction. Techniques such as VM migrations or initiating instances at a different data center (belonging to the same vendor) can serve as a possible solution to such problems.  However, this can introduce overheads and result in extra delay. It is possible that resources belonging to any other party/vendor might be in the vicinity that  might be more efficient to use than using its owned resources at a far away data center. Therefore, it is interesting to see  whether cooperation among different vendors or parties in such instances can be lead to an improved customer satisfaction and better resource utilization. 


==> strategy-2 arxiv/01-intro2.tex <==
Mobile edge computing is a viable solution to support resource intensive applications (users)\footnote{Throughout the paper, we use the terms ``applications'' and ``users'' interchangeably.} that relies on mobile edge clouds (MECs) placed at the edge of any network \cite{he2018s}. This, in contrast with running applications on user devices (with limited processing capability) or deep in the Internet, usually allows  one-hop communication \cite{jia2015optimal} between  edge clouds and applications in order to  provide the required processing power and reduce application latency. %An MEC provides requested resources to applications (users) based on a \emph{Service Level Agreement} (SLA). 
%Applications request resources from an MEC that needs to provide  requested resources based on a \emph{Service Level Agreement} (SLA).  
The goal for any MEC service provider  is to 
provide resources to applications as much as possible, resulting in an increase in application  satisfaction and \emph{utility} for the provider.
However, a fundamental limitation of MEC is that in contrast to traditional cloud platforms and data centers,  edge clouds have  limited resources and may not always be able to satisfy  application demands for resources \cite{he2018s}.  In addition to commercial settings, this problem of limited resources also occurs in military networks.  For example, MEC service providers are equivalent to military coalition partners, who own various parts of the computing resources.
%Aware of this resource scarcity problem, research community has started several initiatives  to create an open edge computing platform  where  edge clouds in the same geographical location form a shared resource pool. However, allocating these resources efficiently from the shared pool to different applications in itself is a challenge. 
%\par There have been several  attempts in the literature  to address the resource allocation problem. He et al. \cite{he2018s} studied the allocation of edge resources to different applications by jointly considering request scheduling and service placement.  
%Jia et al. \cite{jia2015optimal} discussed edge cloud placement and allocation of  resources to mobile users in the edge cloud in a Wireless Metropolitan Area Network (WMAN). They proposed an algorithm that places edge clouds in application dense regions of the WMAN.  
%Xu et al. \cite{xu2016efficient} discussed edge cloud placement in a large-scale WMAN that contains multiple wireless access points (APs). The goal of the placement problem is to minimize the average access delay between  users and  edge clouds. 
\par  To address  resource scarcity, different solutions have been proposed in the literature such as purchasing more resources to meet  peak demands, using resources from the same service provider located at a distant location, or  sharing resources among  co-located mobile edge clouds. However, purchasing more resources to meet peak demands is not an efficient solution as the newly purchased resources may not always be used. Furthermore, it is not always possible to accurately predict peak demand. Hence, delays  in purchasing additional resources may introduce delays in satisfying the applications.  Similarly, using resources of the same provider at a distant location can increase latency. Creating shared resources among  co-located (or physically adjacent)   edge clouds is a promising approach as it accounts for the aforementioned shortcomings of buying more resources to meet peak demands or allocating resources at a distant location. However,  resources of  co-located mobile edge clouds belong to different service providers, each of which  may have a particular objective to optimize such as security, throughput, latency, etc.  when allocating and utilizing its resources. Therefore creating a resource pool and then allocating these resources requires taking different service provider objectives into account, which results in a multi-objective optimization \cite{cho2017survey} (MOO) problem. 

%To ensure the availability of resources, numerous solutions have been proposed in the literature ranging from buying more resources to meet  peak demands, to creating shared resource pools among geographically co-located service providers. However,  different service providers may have different objectives and  existing resource pool based mechanisms do not consider utilities of different service providers. Ideally,  a resource sharing mechanism should consider objectives of different service providers, which  results in a multi-objective optimization (MOO) problem. Furthermore, while resource sharing or creation of a resource pool may tackle the resource availability problem, it does not address  resource allocation problem, i.e.,  optimally allocating the available resources to different users. Therefore, there is a need for a framework that not only ascertains resource availability by enabling resource sharing among different service providers, but also optimally allocates resources to users, while accounting for the service providers' objectives. 


%However, most  work does not  account for the fact that edge resources can belong to different service providers where each service provider can have a particular objective to optimize such as security, throughput, latency, etc. Therefore creating a resource pool and then allocating these resources requires taking different service provider objectives into account, which results in a multi-objective optimization \cite{cho2017survey} (MOO) problem.  Furthermore, in certain cases,  each service provider may prioritize its own applications  applications of other service providers as customer loyalty is an important part of the cloud business model. %For example, \emph{Amazon Web Services} (AWS) and \emph{Microsoft Azure}  need to satisfy the demands of their own customers first before they ``rent''  resources to other service providers. 



 
\par In this paper, we attempt to address these issues. Specifically,  we consider a setting where multiple edge clouds reside at the network edge  belonging to different service providers. Each
MEC has a specific set and amount of resources and a number of applications
affiliated with the MEC demand for resources. We consider
 a strategy where all edge clouds initially allocate resources
 to their native applications. If an edge cloud satisfies its own
 applications and has free resources, it can share them with
 other edge clouds that might need them. This is because
 satisfying native applications helps the MEC service provider
 to retain its customers. We present a resource sharing and allocation framework based on \emph{cooperative game theory} 
(CGT), in
 which different edge clouds form
 a coalition to share their resources and satisfy the requests of different applications.
 Our CGT-based framework considers the fact that different
edge clouds may have different objectives, which makes the
 traditional single-objective optimization framework inapplicable to the MEC settings.

%Each MEC has a specific amount of resources and  applications  affiliated with the MEC  can ask for resources. %We consider two different strategies. In strategy $1$, the edge service providers does not distinguish between its native applications and applications of other service providers. In strategy $2$, 
%We consider a strategy where all edge clouds initially  allocate resources to their native applications. If an edge cloud satisfies its own applications and  has free resources, it can share them with other edge clouds that might need them. This is because satisfying native applications helps the MEC service provider to retain its customers.  % If a particular cloud is looking to ``rent'' resources for its applications, it can use the available resources of the other edge clouds by paying a certain cost or utility.  
%We present a \emph{cooperative game theory} (CGT) based resource sharing and allocation framework in which different edge clouds share their resources and form a coalition to satisfy the requests of different applications. Our CGT based framework considers the fact that different edge clouds  may have different objectives, which is why a traditional single objective optimization framework cannot be used. 

%\subsection{Related Work}\label{sec:related}
%\input{related}




\subsection{Summary of the contributions}
The main contributions of this paper are:
%\vspace{-6pt}
\begin{enumerate}
	\item %We present a novel multi-objective resource sharing and allocation problem formulation that considers both  service provider utilities and application request satisfaction in mobile edge clouds. 
	We present a novel multi-objective resource-sharing
	problem formulation that considers both
	service provider utilities and application request satisfaction
	in mobile edge clouds. 
	 We propose a cooperative game theory based framework to solve the formulated problem. We model each edge cloud service provider as a player in our game and  model  resource sharing and allocation problem  as a \emph{canonical} game with non-transferable utility (NTU). 
	%\item
	 We prove that the game is super-additive and convex, hence the \emph{core} is non-empty. Therefore, the grand coalition of all edge clouds is stable.  
	%\item For strategy $1$,  we address the problem of obtaining an allocation from the core by proposing a computationally efficient  $\mathcal{O}(N)$ algorithm  that is guaranteed to provide an allocation from the core.
%	\item We first propose  
\item We   propose  a distributed \emph{Game-theoretic Pareto Optimal Allocation} (GPOA) algorithm that provides an allocation from the core based on a strategy where all MECs first allocate resources to their native applications, and then MECs with resource surplus share their resources with those that have a resource deficit. %Since the allocation is from the core, it  is Pareto-optimal. 
\item To reduce resource fragmentation\footnote{We define resource fragmentation as splitting of the provisioned resources to applications of any player $n$ across different MECs. The higher the number of MECs that provide resources to a particular application, the higher will be the resource fragmentation. Ideally, for the applications of a resource deficit MEC, only one MEC with resource surplus should provide the resources. } due to resource sharing among MECs, we also propose  \emph{Polyandrous Polygamous Matching based Pareto Optimal Allocation} (PPMPOA) algorithm that aims to match resource deficit MECs with resource surplus MECs. % in an efficient manner. 
Using evaluations we show that PPMPOA:
\begin{itemize}
	\item Provides allocation from the core.
	\item Results in a \emph{stable} matching \cite{maschler2013}.
	\item Reduces resource fragmentation. 
\end{itemize}
% PPMPOA provides allocation from the core  and  that the match is  \emph{stable} \cite{maschler2013}. Furthermore, PPMPOA also reduces resource fragmentation.
\item We also prove that the proposed  algorithms, GPOA and PPMPOA,  enforce \emph{truth-telling}, i.e., no MEC service provider has the incentive to misreport its capacity and native application requests. 

%	\item  We  propose a family of   $\mathcal{O}(N)$ distributed algorithms that provide allocations from the core  based on a strategy where all MECs first allocate resources to their native applications, and then MECs with resource surplus share their resources with those that have a resource deficit. Since the allocations are from the core, the solution obtained is Pareto-optimal.  We also prove that the proposed distributed algorithms enforce \emph{truth-telling}, i.e., no MEC service provider has any incentive to misreport its capacity and native application requests. 
	%We also prove that MEC service providers have no incentive to cheat using our proposed algorithms, hence 
	
%	\item   For the strategy where all MECs first allocate resources to their native applications, and then MECs with resource surplus share their resources with those that have a resource deficit, we  also propose a family of   $\mathcal{O}(N)$ distributed algorithms that provide allocations from the core. 
	%Since the allocation is from the core, the obtained solution is Pareto-optimal and guarantees stability of grand-coalition. 
	\item We evaluate the performance of our proposed framework
	by extensive simulations. We verify the game
	theoretic properties of our proposed approach by showing
	that the game is super-additive and the core is nonempty,
	i.e., our obtained solutions are from the core
	 and satisfy properties such as \emph{individual rationality}, \emph{group rationality}, and \emph{stability}.  We also  show that the resource sharing and allocation mechanism  improves the utilities of  game players. Furthermore, our framework also improves application (user) satisfaction.
	 
\end{enumerate}
The rest of the paper is  structured as follows. %Section~\ref{sec:related} presents a review of literature related to resource allocation and sharing for edge computing. %
Section~\ref{sec:prelim} provides a primer on  MOO,  CGT, and  the core. 
 Section~\ref{sec:sysmodel} describes our system model and presents the resource sharing/allocation optimization problem.  Section \ref{sec:opt_problem} discusses the game theoretic solution  %Section~\ref{sec:gametheory} describes the game theoretic solution for the resource allocation and sharing problem. 
and Section~\ref{sec:exp_results} presents our experimental results.  Section \ref{sec:related} presents a review of relevant literature, while Section~\ref{sec:conclusion} concludes the paper.  %Table \textbf{add table} provides a  list of notations used throughout the paper.  



%\section{Related Work}\label{sec:related}
%\input{related}



==> strategy-2 arxiv/02-sysmodel.tex <==
%Any entity that has specific resources such as CPU, storage and communication serve as the building block of our system as shown in Figure~\ref{fig:system_model} . We call this basic building block of our system a \emph{domain}. The domain can be as small as a sensor and as large as a data center.  Each domain has a \emph{domain controller} that is aware of all the resources available within the domain. The domain controller only communicates an abstraction of this information to the outside world and does not share the entire information\footnote{This can be due to a number of reasons including security and privacy. For example, Amazon and Dropbox can be in a coalition to satisfy their user's needs. However, they will not provide the entire information to each other.}. Different domains can be combined to form a coalition in the presence of a \emph{coalition controller}. The coalition controller can be either a separate controller or chosen from the domain controllers.  Below we model this coalition from game theory perspective.   

 \begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{figures/newDomains}
	\caption{Our system model with multiple cloud service providers}
	\protect\label{fig:system_model}
	\vspace{-0.2in}
\end{figure}


Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of all the cloud service providers that act as players in our game. % For simplicity, we drop the $P$ in $P_n$ and represent the players only with the subscript $n$. 
We assume that each player has a set of $\mathcal{K}=\{1,2,\cdots, K\}$ different types of resources such as communication, computation and storage resources.  The $n^{th}$ service provider represents its  available resources as $C^n = \{ C_1^{(n)},\cdots, C_K^{(n)}\}$. Here $C_k^{(n)}$ is the amount of resources of type $k$ available at service provider $n$. 
%All edge clouds can report their available resources  to any central entity, coalition controller \footnote{Coalition controller can be chosen from the edge clouds.},  where ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ represents the available resources $k \in \mathcal{K}$ for the player $n \in \mathcal{N}$. 
The vector $C=\{\sum_{n \in \mathcal{N}}C_{1}^{(n)}, \sum_{n \in \mathcal{N}}C_{2}^{(n)}, \cdots ,\sum_{n \in \mathcal{N}}C_{K}^{(n)}\}$ represents  all available resources at different service providers.  Each service provider $n$ has a set of  native applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$ that ask for resources. 

The set of all applications that ask for resources from the set of service providers (coalition of service providers) is given by $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset, \; \forall i \neq j,$ i.e., each application asks only  one service provider for resources. 
%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
Every player  $n \in \mathcal{N}$ has a request (requirement) matrix $R^{(n)}$.% from every player $n \in \mathcal{N}$ 
\begin{equation}
\label{eq:R_Req}
R^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{r^{(n)}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{(n)}_{{M}_n}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r^{(n)}_{11} & \cdots  &\cdots   & r^{(n)}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{(n)}_{M_{n}1}&\cdots  &\cdots   & r^{(n)}_{{M}_n{K}}
\end{smallmatrix}\Biggr]
\end{equation}
where the $i^{th}$ row corresponds to the $i^{th}$ application while  columns represent different resources, i.e., $r_{ij}^{(n)}$ is the amount of $j^{th}$ resource that application $i \in \mathcal{M}_n$ requests.
%The vector ${C}^{(n)}$ received by coalition controller shows different available resources at edge cloud $n$. 
Request matrix $R$ is an augmentation of all the request matrices (from all the service providers)  as given below. 
\begin{equation}
\label{eq:R_Reqco}
R^{}=\Biggl[\begin{smallmatrix}
\mathbf{r^{}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{}_{{M}}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r^{}_{11} & \cdots  &\cdots   & r^{}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{}_{M1}&\cdots  &\cdots   & r^{}_{{M}{K}}
\end{smallmatrix}\Biggr]
\end{equation}
where $r_{ij}$ is the amount of $j^{th}$ resource that application $i \in \mathcal{M}$ requests.
%We assume that a subset $\mathcal{N}_1 \subset \mathcal{N}$ have resource surplus, while a subset $\mathcal{{N}}_2 \subset \mathcal{N}$ has a resource deficit. Furthermore, we also assume that for any player $i \in \mathcal{{N}}_1$, $R^{(i)}> C^{(n)},\; \forall n \in \mathcal{{N}}_2$, i.e., no single player in $\mathcal{{N}}_2$ has a resource surplus that is more than the resource deficit of a player in $\mathcal{{N}}_1$. 

The resource sharing and allocation framework, based on $R$ and  $C$, has to make an allocation decision $\mathcal{X}$ that optimizes the utilities $u_n(\mathcal{X})$ of all the service providers $n \in \mathcal{N}$.  The allocation decision $\mathcal{X}$ is  a vector $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$ that indicates how much of each resource $k \in \mathcal{K}$ is allocated to application $i$ at service provider $n \in \mathcal{N}$. The matrix $X^{(n)}$ is an augmentation of different matrices $\{X_{i\in \mathcal{M}_1}^{(n)}, \cdots,X_{i\in \mathcal{M}_n}^{(n)},\cdots, X_{i\in \mathcal{M}_N}^{(n)} \}$, where $X_{i\in \mathcal{M}_j}^{(n)}$ is the allocation decision  at service provider $n$ for the applications $i$ originally belonging to service provider $j \in \mathcal{N}$ and $X_{i\in \mathcal{M}_n}^{(n)}$, $\forall j \in \mathcal{N}, j \neq n$ is the allocation decision at service provider $n$ for applications $i$ belonging to service provider $n$ i.e., the original applications of the service provider $n$. 
Mathematically, 

\begin{equation}
\label{eq:A_n}
X^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{{M}}}^{(n)}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{{M}}1}^{(n)}&\cdots  &\cdots   & x_{{{M}}{K}}^{(n)}
\end{smallmatrix}\Biggr]
\end{equation}
where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$. 


\begin{comment}
Each player has a utility function $u_n(\mathcal{X})$ that depends on the allocation decision $X$ (details for $X$ will be given later). We assume that each player has set of $\mathcal{K}=\{1,2,\cdots, K\}$ different resources such as communication, computation and storage resources. %Each player $n \in \mathcal{N}$ has complete information about its own resources $k \in \mathcal{K}$, however it reports only abstract information to a coalition controller 
All domains report their available resources  to the coalition controller where $C^{(n)}$ represent the available resources for the domain/player $n \in \mathcal{N}$. Each domain $n$ has a set of users or applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$ that ask for resources. Also $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset \; \forall i \neq j$ represents the set of all users that ask for resources from the coalition. 

%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
The coalition controller receives a matrix $R^{(n)}$ for every player $n \in \mathcal{N}$ 
	\begin{equation}
\label{eq:R_Req}
R^{(n)}=\Biggl(\begin{smallmatrix}
\mathbf{r^{(n)}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{(n)}_{{M}_n}}
\end{smallmatrix}\Biggr) = \Biggl(\begin{smallmatrix}
r^{(n)}_{11} & \cdots  &\cdots   & r^{(n)}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{(n)}_{M_{n}1}&\cdots  &\cdots   & r^{(n)}_{{M}_n{K}}
\end{smallmatrix}\Biggr)
\end{equation}
where the $i^{th}$ row corresponds to the $i^{th}$ user while  the columns represent different resources i.e., $r_{ij}$ is the amount of $j^{th}$ resource user $i \in \mathcal{M}$ requests.

The vector ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ received by coalition controller shows different available resources at domain $n$. 
The vector $C=\{\sum_{n \in \mathcal{N}}C_{1}^{(n)}, \sum_{n \in \mathcal{N}}C_{2}^{(n)}, \cdots ,\sum_{n \in \mathcal{N}}C_{K}^{(n)}\}$ consists of all the available resources at different domains. The coalition, based on $R$ and  $C$, has to make an allocation decision $\mathcal{X}$ that optimizes the utilities $u_n(\mathcal{X})$ of the domains.  The allocation decision $\mathcal{X}$ is  a vector $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$ that shows how much of each resource $k$ is allocated to user $i$ at domains $n \in \mathcal{N}$.

\begin{equation}
\label{eq:A_n}
X^{(n)}=\Biggl(\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{|\mathcal{M}|}}^{(n)}}
\end{smallmatrix}\Biggr) = \Biggl(\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{|\mathcal{M}|}1}^{(n)}&\cdots  &\cdots   & x_{{|\mathcal{M}|}{K}}^{(n)}
\end{smallmatrix}\Biggr)
\end{equation}
where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ allocated  to user $i$ at player $n$

 Since the utilities of different domains might be different (can be conflicting as well), this leads us to a multi-objective optimization (MOO) problem. Some of the assumptions in our model are given below
\subsection{Assumptions}
The assumptions made in our model are 
\begin{enumerate}
	\item The negotiation cost among different domains is negligible
	\item All the domains communicate their information to the coalition controller
	\item The coalition controller already exists% and do not discuss the selection of the coalition controller (can be explored in the future work)
	\item Resources across different domains are additive in nature i.e., if domain $X$ and $Y$ have $2$ GB RAM each, the coalition would have $4$ GB of RAM. 
	\item Each player has a single objective
	\item The objective of the coalition is a sum of the utilities of all the players with equal weight
%	\item Any new player/domain added into the coalition will have resources available
	\item All players or domains have the same number of users or jobs
\end{enumerate}
\end{comment}








==> strategy-2 arxiv/02-sysmodel2.tex <==
%Any entity that has specific resources such as CPU, storage and communication serve as the building block of our system as shown in Figure~\ref{fig:system_model} . We call this basic building block of our system a \emph{domain}. The domain can be as small as a sensor and as large as a data center.  Each domain has a \emph{domain controller} that is aware of all the resources available within the domain. The domain controller only communicates an abstraction of this information to the outside world and does not share the entire information\footnote{This can be due to a number of reasons including security and privacy. For example, Amazon and Dropbox can be in a coalition to satisfy their user's needs. However, they will not provide the entire information to each other.}. Different domains can be combined to form a coalition in the presence of a \emph{coalition controller}. The coalition controller can be either a separate controller or chosen from the domain controllers.  Below we model this coalition from game theory perspective.   

 \begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{mec.jpg}
	\caption{Our system model with multiple MEC providers}
	\protect\label{fig:system_model}
	\vspace{-0.2in}
\end{figure}


Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of   edge cloud-service providers. % that act as players in our game. % For simplicity, we drop the $P$ in $P_n$ and represent the players only with the subscript $n$. 
We assume that each service provider has a set of $\mathcal{K}=\{1,2,\cdots, K\}$ different types of resources such as communication, computation and storage resources.  Let the available resources at service provider  $n$ be denoted by $C_{n} = \{ C_{n,1},\cdots, C_{n,K}\}$, where  $C_{n,k}$ is the amount of type $k$ resources available at  service provider $n$. 
%All edge clouds can report their available resources  to any central entity, coalition controller \footnote{Coalition controller can be chosen from the edge clouds.},  where ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ represents the available resources $k \in \mathcal{K}$ for the player $n \in \mathcal{N}$. 
%The vector $C=\{\sum_{n \in \mathcal{N}}C_{n,1}, \sum_{n \in \mathcal{N}}C_{n,2}, \cdots ,\sum_{n \in \mathcal{N}}C_{n,K}\}$ represents  all available resources at different service providers.
  Each service provider $n$ has a set of  native (local) applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$. 
The set of all applications that ask for resources from all  service providers (i.e., the grand coalition of service providers) is given by $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset, \; \forall i \neq j,$ i.e., each provider has an entirely different set of native applications. 
%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
Every provider  $n \in \mathcal{N}$ has a request (requirement) matrix $R_{n}$.% from every player $n \in \mathcal{N}$ 
\begin{equation}
\label{eq:R_Req}
R_{n}=\Biggl[\begin{smallmatrix}
\mathbf{r_{n}^1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r_{n}^{{M}_n}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r_{n,1}^{1} & \cdots  &\cdots   & r^{1}_{n,{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r_{n,1}^{{M}_n}&\cdots  &\cdots   & r_{n,K}^{{M}_n}
\end{smallmatrix}\Biggr].
\end{equation}
where the $j^{th}$ row corresponds to  application $j$, while  columns represent different resources. That is,  $r_{n,k}^{j}$ is the amount of resource $k$ that application $j \in \mathcal{M}_n$ requests from provider $n$. When the service provider  works alone\footnote{Not borrowing from or renting out its resources to any other service provider.},  its objective is to maximize its utility by allocating  resources to its native applications and improving application satisfaction. A service provider $n$ earns a non-negative \emph{monotonically non-decreasing} utility $u_n^j (x_{n,k}^j)$ by making  allocation decision $x_{n,k}^j$, i.e., allocating $x_{n,k}^j$ amount of resource $k$ to application $j\in \mathcal{M}_n$, where  $\mathbf{x}_n^j= [x_{n,1}^j, x_{n,2}^j,\cdots, x_{n,K}^j]^T$. 
 Table \ref{tab:not} summarizes the notations used throughout the paper. Below we present the optimization formulation for a single service provider. 

%\textbf{Add notation table here}


\begin{table}[]
	\centering
	\caption{List of notations used throughout the paper}
	\begin{tabular}{|p{1cm}|p{6.9cm}|}
		\hline
		\textbf{Notation}	& \textbf{Description} \\ \hline
		$\mathcal{{N}}, N, n$	& Set, number and index of game players (service providers)  \\ \hline
		$\mathcal{K}, K, k$	& Set, number and index of resources \\ \hline
		$\mathcal{M}, M, j$	& Set, number and index of applications \\ \hline
		$\mathcal{M}_{n}$	& Set of native applications at player (provider) $n$  \\ \hline
		${S}$	& A coalition of game players (providers), where $S \subseteq \mathcal{{N}}$  \\ \hline
		%$\mathcal{M}_{n}$	& Set of native applications at player $n$  \\ \hline
		$\mathcal{V}$	& Set of payoff vectors    \\ \hline
		${v}(S)$	& Value of coalition $S$    \\ \hline
		$\mathcal{G}_1$	& Set of players (providers) with resource deficit    \\ \hline
		$\mathcal{G}_2$	& Set of players (providers) with resource surplus   \\ \hline
		$C$	& Capacity vector of all game players (providers) \\ \hline
		$C_n$	& Capacity vector of player  (provider)$n$ \\ \hline
		$C_{n,k}$	& Capacity of resource $k$ at player (provider) $n$ \\ \hline
	%	$R$	& Request matrix of all game players \\ \hline
		$R_{n}$	& Request matrix at player (provider) $n$ \\ \hline
		$r_{n,k}^{j}$	& Request of application $j$ for resource $k$ from player (provider) $n$ \\ \hline
	%	${X}_{i \in \mathcal{M}_n}^{(n)}$	& Allocation decision matrix at player $n$ for its native applications \\ \hline
	%	${X}_{i \in \mathcal{M}_j}^{(n)}$	& Allocation decision matrix at player $n$ for applications of other players \\ \hline
	%	${X}^{(n)}$	& Allocation decision matrix at player $n$ for all applications (native and applications of other service providers)\\ \hline
	%	$\mathcal{X}_n$	& Allocation decision for all game players  \\ \hline
%		$X_{SO}^{(n)}$	& Single objective allocation decision at $n$  \\ \hline
		$x_{n,k}^{j}$	& Allocation decision of resource $k$ for application $j$ at player (provider) $n$ \\ \hline
	$\mathbf{x}_{n}^{j}$	& Allocation decision vector for application $j$ at player (provider) $n$ when working alone \\ \hline

	%	$u_{j}^n$	& Utility player $n$ earns by allocating resources to applications of player $j$\\ \hline
	$\mathbf{X}_n$ & Allocation decision for player (provider) $n$ in the  coalition \\ \hline 
	$\mathbf{X}$ & Allocation decision for the entire coalition  \\ \hline 
		$\mathcal{X}_n$ & Allocation decision for player (provider) $n$ in the  coalition excluding its native applications \\ \hline	
		$^{m}\mathbf{X}_n$ & Allocation decision for applications of player (provider) $m$ at player (provider) $n$ in the  coalition s \\ \hline		
			$u_{n}^j({x}_{n,k}^j)$	& Utility player (provider) $n$ earns  by allocating resource $k$ to application $j$ \\ \hline
		$u_{n}^j(\mathbf{x}_{n}^j)$	& Utility player (provider) $n$ earns  by allocating vector of  resources to application $j$ \\ \hline
		$GC$	& Grand coalition\\ \hline
		$RS$ & Request satisfiability\\ \hline
		$TU$ & Transferable utility\\ \hline
		$NTU$ & Non-transferable utility\\ \hline
		$CGT$ & Cooperative game theory\\ \hline
		$MOO$ & Multi-objective optimization\\ \hline
		$SOO$ & Single-objective optimization\\ \hline
		$MEC$ & Mobile edge cloud\\ \hline
	\end{tabular}
	\label{tab:not}
\end{table}
\subsection{Problem Formulation for Single Service Provider} \label{sec:prob}
 We  first present the resource allocation problem for a single, stand-alone provider (i.e., no resource sharing with other providers). 
For each provider  $n \in \mathcal{N}$, the allocation decisions  consist of the vectors $\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}$. The optimization problem is: 
\begin{subequations}\label{eq:opt_single}
	\begin{align}
	\max_{\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}}\quad& \sum_{j \in \mathcal{M}_n}f_n^j(\mathbf{x}_n^j), \label{eq:objsingle}\displaybreak[0]\\
	%\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \sum_{j \in \mathcal{M}_n}\sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{n,k}^{j}}, \label{eq:objsingle}\\
	\text{s.t.}\quad & \sum_{j} x_{n,k}^{j}\leq C_{n,k}, \quad \forall k \in \mathcal{K} \label{eq:singlefirst} \displaybreak[0]\\
	& x_{n,k}^{j} \leq r^{j}_{n,k}, \quad \forall\; j\in \mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecond} \displaybreak[1]\\
	&  x_{n,k}^{j} \geq 0, \quad \forall\; j\in \mathcal{M}_n, k \in \mathcal{K}. \label{eq:singlethird} \displaybreak[2]
	\end{align}
\end{subequations}
 The objective function $f_n^j(\mathbf{x}_n^j)$  is required to be a monotonic, non-negative and non-decreasing function. For illustration purposes in this paper, we assume that:%\vspace{-0.15in} 
\begin{align}
f_n^j(\mathbf{x}_n^j) =w_{1}^ju_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{n,k}^{j}}. \nonumber 
\end{align}%\vspace{-0.05in}
where the  term $ \sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{n,k}^{j}}$  captures the request satisfaction (see Definition \ref{def:rs}) and $u_n^j(\mathbf{x}_n^j)$ is the non-decreasing and non-negative utility the  service provider earns by providing the resources to applications. %Since the second term is always between $0$ and $1$, 
The weight $w_{1}^j$ is  used for \emph{scaling} so that both the terms are on the same scale. 
The first constraint in \eqref{eq:singlefirst} indicates that the allocated resources cannot exceed capacity. The second constraint  in \eqref{eq:singlesecond} indicates that the allocated resources should not exceed the required amounts.  The last constraint, \eqref{eq:singlethird}  requires the allocation to be non-negative.



The goal of this single-objective optimization problem for every provider, as mentioned earlier,  is   to  maximize its utility by allocating available resources to its native applications and improving application satisfaction. We note that this single-provider formulation does not consider the following. For example, it is possible that
 a service provider $n$ may earn a larger utility by providing
 its resources to applications of other service providers. Furthermore, provider(s)
 may not have sufficient resources to satisfy requests of all its
 native applications, while other 
 providers  may have resource
 surpluses that can be ``rented" and utilized by other providers. In this work, we focus on strategies where each service
provider allocates resources to its native applications and
then shares any remaining  resources with other service
providers who are not able to fully satisfy their native applications.
These aspects are considered in the following formulation.






\subsection{Problem Formulation for Multiple Service Providers}
Let us assume that a mobile edge service provider $n$ does not have sufficient resources to satisfy all its native applications. Suppose that service provider $m$  has a resource surplus, after allocating its resources to its native applications that can  be shared with $n$. Allowing resource sharing among such providers can
 improve resource utilization and application satisfaction.
%Therefore, allowing resource sharing among such service providers, while considering their objectives can improve resource utilization and improve application satisfaction. 
By sharing and allocating its type $k$ resources  to application $l$, service provider $m$ earns a non-decreasing and non-negative net utility $H_m^l(x_{m,k}^l)$, which in this paper is assumed to be % as follows as an illustrative example\footnote{Our framework can work with any non-negative,  non-decreasing utility.}.
\begin{align}\label{eq:1}
H_m^l( x_{m,k}^l)=w_1^l\Big(u_m^l (z_k^l+x_{m,k}^l)-u_m^l (z_k^l)  -D_m^l(x_{m,k}^l)\Big)\nonumber \\+ \Big(\frac{x_{m,k}^l}{r_{n,k}^l-z_k^l}\Big)^2, \forall l \in \mathcal{{M}}\backslash \mathcal{{M}}_m, n \in \mathcal{{N}}\backslash m.
\end{align} 
where $z_k^l= \sum_{n \in \mathcal{{N}}\backslash m}x_{n,k}^l$ is the amount of resource $k$ allocated already to application $l$ by providers other than $m$. $u_m^l (z_k^l+x_{m,k}^l)-u_m^l (z_{k}^l)$  captures the incremental increase in utility of provider $m$ due to the allocation of additional resource $x_{m,k}^l$.  $D_m^j(x_{m,k}^j)$ represents the communication cost of serving application $j \in  \mathcal{{M}}_n$ by using resource of type $k$ at  provider $m$ rather than its native service provider $n$. We assume that the communication cost is a positive monotonic non-decreasing function. The term $(\frac{x_{m,k}^l}{r_{n,k}^l-z_k^l})^2$, which takes  a value in  $[0, 1]$, is used to reduce resource fragmentation by providing a higher utility  for providing more resources at a particular provider.   

To consider each provider and its native applications, let  $F_n^{j}(\mathbf{x}_n^j)$ represent the utility  service provider $n$ earns by allocating resources to its native applications along with the increase in request satisfaction due to provision of resources to its applications at different service providers including itself.  
% as well as shared resources received by the applications from other service
   %We note that  $F_n^{j}(\mathbf{x}_n^j)$ is  a non-negative and non-decreasing function and 
   We assume:%\vspace{0.2in}
\begin{align}\label{eq:2}
F_n^{j}(\mathbf{x}_n^j) =w_1^ju_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}}\frac{\sum_{m \in \mathcal{{N}}}x_{m,k}^{j}}{r_{n,k}^{j}}.
\end{align}
% and $d_m^j$ is the distance between service provider $m$ and the native service provider of application $j$.
%By sharing its resources, player $m$ earns a utility $u_m^j (x_{m,k}^j)-C_m^j(x_{m,k}^j)$ after making an allocation decision $x_{m,k}^j$ for $j\in \mathcal{{M}}_n$,
Note that $F_n^{j}$ is  monotonic non-decreasing and non-negative. 
 Furthermore, we implicitly assume that $ u_n^j (\mathbf{x})=u_m^j (\mathbf{x}), \; \mathbf{x}\geq 0$.  The latter assumption reflects that different providers  earn the same utility when allocating the same amount of resources of the same type to a given application, either locally or remotely.  Furthermore, % \textbf{(This assumption may no longer be needed and we can relax it)}.



\begin{align}
\mathbf{x}^j= [\sum_{n \in \mathcal{{N}}}x_{n,1}^j, \sum_{n \in \mathcal{{N}}}x_{n,2}^j,\cdots, \sum_{n \in \mathcal{{N}}}x_{n,K}^j]^T. \nonumber
\end{align}
That is, the total resources allocated to any application $j \in \mathcal{M}$ is the sum of resource allocated to it across all service providers.  The resource sharing and allocation framework, based on resource requests and  capacities of service providers, has to make allocations that optimize the utilities of all the service providers $n \in \mathcal{N}$ while satisfying user requests as well.  The allocation decision is given by
%$\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{|\mathcal{M}|}$
$\mathbf{X}=\{\mathbf{X}_1, \mathbf{X}_2, \cdots, \mathbf{X}_N\}$, where $\mathbf{X}_n,\; \forall n \in \mathcal{N}$ is given by: 

\begin{equation}
\label{eq:X}
\mathbf{X}_{n}=\Biggl[\begin{smallmatrix}
\mathbf{x}^{1}_n\\ 
.\\ 
.\\ 
.\\
\mathbf{x}^{|\mathcal{{M}}|}_n
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{n,1}^{1} & \cdots  &\cdots   & x^{1}_{n,{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{n,1}^{|\mathcal{{M}}|}&\cdots  &\cdots   & x_{n,K}^{|\mathcal{{M}}|}
\end{smallmatrix}\Biggr].
\end{equation}




When service providers share resources,  each service provider aims to  maximize the sum of utilities obtained by a) allocating resources to its native applications;  b) allocating resources (if available) to  applications of other service providers;  c) improving the request satisfaction of its applications by using its
 own resources or borrowing from other service providers (when
needed and possible); and d) reducing resource fragmentation. 
In the resource sharing case, each service provider
allocates its resources by solving the following optimization problem:
% \eqref{eq:opt_higher}.  %\vspace{-0.2in}

%The above discussion leads  to the following generic optimization problem for the resource sharing case.  
%\begin{comment}
\begin{subequations}\label{eq:opt_higher}
	\begin{align}
	\max_{\mathbf{X}_n}\quad&\sum_{j \in \mathcal{M}_n} F_n^{j}(\mathbf{x}_n^j)+\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} H_n^l (\mathbf{x}_n^l),\quad \forall n \in \mathcal{{N}}, \label{eq:obj}\\%\bigg(\sum_{j \in \mathcal{M}_n}\big(u_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}}\frac{\sum_{m \in \mathcal{{N}}}x_{m,k}^{j}}{r_{n,k}^{j}}\big) +\nonumber \\
	%& \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-
	%C_n^l(\mathbf{x}_n^l)\big)\bigg) \quad \forall n \in \mathcal{{N}}, \label{eq:obj}\\ %\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in \mathcal{N},j\neq n}  u^{n}_j(\mathcal{X})\bigg) \quad \forall n \in \mathcal{N} \label{eq:obj}\\%\{u_1(\mathcal{A}),u_2(\mathcal{A}),\cdots,u_N(\mathcal{A})\} \label{eq:obj}\\%U(A)\label{eq:obj}\\
	\text{s.t.}\quad 
	& \sum_{j} x_{n,k}^{j}\leq C_{n,k}, \quad \forall\; j\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}, \label{eq:obj1} \displaybreak[0]\\
	& \sum_{m \in \mathcal{N}}x_{m,k}^{j} \leq r_{n,k}^{j}, \quad \forall\; j\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N},  \label{eq:obj2}\displaybreak[1]\\
	&  x_{n,k}^{j} \geq 0, \quad \forall\; j\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}, \label{eq:obj3} \displaybreak[2] \\
	&  u_n^l(z_k^l+ {x}_{n,k}^l) - u_n^j({z}_{k}^l)\geq D_n^l({x}_{n,k}^l),\quad \nonumber \\ & \forall l \in \mathcal{M}\backslash\mathcal{{M}}_n, k \in \mathcal{K}, n \in \mathcal{N} \label{eq:obj4}, 
	\end{align}
\end{subequations}
%\end{comment}
where  $F_n^j(\mathbf{x}_n^j)$ and $H_n^l(\mathbf{x}_n^l)$ are given in \eqref{eq:1} and \eqref{eq:2}. % into \eqref{eq:obj}, the objective function can be rewritten as:
%\begin{align}
%&\sum_{j \in \mathcal{M}_n}\big(w_1^ju_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}}\frac{\sum_{m \in \mathcal{{N}}}x_{m,k}^{j}}{r_{n,k}^{j}}\big)+\nonumber \\
%& \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-D_n^l(\mathbf{x}_n^l)\big), \quad \forall n \in \mathcal{{N}},
%\end{align}
Constraints \eqref{eq:obj1}-\eqref{eq:obj3} are similar to those for the formulation in \eqref{eq:opt_single}, except that \eqref{eq:obj4} indicates that the utility earned by sharing resources must be higher than the communication cost.

 %indicates that total resources allocated cannot be more than the capacity of service providers. \eqref{eq:obj2} means that the total amount of resources allocated to any application using the resource sharing framework cannot be more than the amount of requested resources, whereas \eqref{eq:obj3}  indicates that the allocation decision cannot be negative. The final constraint \eqref{eq:obj4} indicates that the utility earned by sharing resources is more than the communication cost.
As the utility $u_n^j,\; \forall n\in \mathcal{{N}} $ can differ for each application $j$, \eqref{eq:opt_higher} for all providers $n$ represents   a multi-objective optimization problem, which will be solved by a game-theoretic approach as follows.   



==> strategy-2 arxiv/03-opt-problem.tex <==


In this section, we first present general properties of our game and show that the resource-sharing problem for multiple providers  can be modeled as a canonical cooperative game with non-transferable utility. We then show that the core is non-empty, by proving that our canonical game is \emph{cardinally convex}\cite{sharkey1981convex}. Finally, we propose algorithms in Section \ref{sec:algorithms} to obtain allocations from the core.
%we propose a family of distributed algorithms in Section \ref{sec:algorithms} that provide allocations from the core. 

\subsection{General Game Properties}\label{sec:generalgame}


We model each service provider as a player in our game to obtain the optimal resource sharing/allocation decision. 
Let $\mathcal{N}$ be the set of players that  play the resource sharing and allocation game. The \emph{value of coalition} for the game players $S \subseteq \mathcal{N}$ is given by, \eqref{eq:payoff_function}, where $\mathcal{F}_S$ is the feasible set for resource sharing and allocation given by, \eqref{eq:obj1}-\eqref{eq:obj3} and $\mathcal{M}_S$ is the set of applications in $S$, 
\vspace{-0.1in}
\begin{align} \label{eq:payoff_function}
v({S})&=\sum_{{\substack{{n \in S}\\ {\mathcal{X} \in \mathcal{F}_S}}}}  
\bigg(\sum_{j \in \mathcal{M}_n}\big(w_1^ju_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}}\frac{\sum_{m \in {{S}}}x_{m,k}^{j}}{r_{n,k}^{j}}\big) +\nonumber \\
&  \Big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} w_1^l\big(u_n^l(\mathbf{z}^l+\mathbf{x}_n^l)-u_n^l(\mathbf{z}^l)-D_n^l(\mathbf{x}_n^l)\big)+\nonumber \\
&\sum_{k \in \mathcal{K}}\Big(\frac{x_{n,k}^l}{r_{p(l),k}^l-z_k^l}\Big)^2\Big)\bigg).
%\bigg(u_n({X}_{i \in \mathcal{M}_n}^{(n)})+ \sum_{\substack{j \in {S},\\j\neq n}} u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})+\nonumber \\
%&\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \mathcal{{S}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg).
\end{align}
%In our resource sharing and allocation framework, the payoff each service provider receives is the  sum of utilities obtained by a) allocating resources to its native applications, i.e., $u_n({X}^{(n)}_{i \in \mathcal{M}_n})$;  b) allocating resources to  applications of other service providers, i.e.,  $u_j^n({X}^{(n)}_{i \in \mathcal{M}_j}),\; \forall j\in \mathcal{N}\backslash n$; and c) satisfying requests of applications.
Here $p(l)$ indicates the native player to which application $l$ belongs. Our strategy  to achieve the aforementioned value of coalition is that each player first allocates resources to its own applications and then shares its remaining resources (if any) with  other players. 
%The payoff each player $n \in S$ receives depends on the strategy employed by the game. %$w_n$ is the weight associated with the utility $u_n$ and $\zeta_n$ is the weight affiliated with all $u_j^n$. 
%Furthermore, we assume that  resources allocated across two different edge clouds are \emph{additive}, i.e., if $2$ GB  




\begin{remark}
	
A	resource allocation and sharing problem (with multiple objectives) for the aforementioned system model  can be modeled as a canonical cooperative game with NTU. 
\end{remark}
%\begin{proof}
%To prove this, we need to show that the characteristic function of resource sharing and allocation problem satisfies the following two conditions:
This is so because the stated problem satisfies the following two
conditions.

%This is because our characteristic function of resource sharing and allocation problem satisfies the following two conditions. 
%	For a game to be canonical, we need to prove that the game  is superadditive and the payoff function is of characteristic form. 
\begin{itemize}
	\item \textbf{Characteristic form of payoff:} As the utility function in our  formulated resource sharing and allocation problem  only relies on  service providers that are part of the coalition, the game or payoff function is of characteristic form.
	\item \textbf{Superadditivity:} %Super-additivity for TU games requires $v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset$ i.e. we have to prove that the pay-off or utility for a domain in the coalition is as good as domain working alone or in a smaller coalition. 
	%	Let $u_n(X_{SO}^{(n)})$ be the utility a player $n$ earns by allocating resources to application when it is not in a coalition with any other game player. Let $U_n(X)$\footnote{$U_n(X)=w_nu_n({X}_{i \in \mathcal{M}_n}^{(n)})+\zeta_{n} \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})$} be the utility a player earns when it is part of a larger  coalition. Due to monotonicity property of the utility functions used,  for all  players $n \in \mathcal{N}$,  $u_n(X_{SO}^{(n)})\leq u_n({X})$ as $X_{SO}^{(n)}\subset {X}$. Hence, the game is superadditive.  %This is {because $X_n^{C}$ can contain much more elements due to the increase in $C$ in the coalition} where $X_n^{C}$ and $X_n^{NC}$ are the allocation decisions in  a cooperative game  and independent setting respectively for domain $n$. 
	Let $S_1, S_2 \subseteq \mathcal{N}$ where $S_1, S_2$ are non-empty and $S_1 \cap S_2 =\emptyset$. Hence, $S_1,\; S_2 \subset (S_1 \cup S_2)$. Superadditivity  follows from the monotonic utility functions. 
	%	\begin{equation}\label{eq:super}
	%	\centering 
	%	v(S_1 \cup S_2) \geq v(S_1)+v(S_2)
	%	\end{equation}
	
\end{itemize}
%\end{proof}


\begin{comment}
\begin{definition}[Convex Games]
	A coalition game is said to be convex if and only if for every player $n \in \mathcal{N}$, the marginal contribution of the player is non-decreasing W.R.T set inclusion. Mathematically, for $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash \{n\}$ 
	\begin{equation}\label{eq:convexgames}
	v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2).
	\end{equation} 
\end{definition}
\end{comment} 
\begin{definition}[Cardinally Convex Games\cite{sharkey1981convex}]
	An NTU game is said to be cardinally  convex if $\forall\; S_1,\; S_2 \subseteq \mathcal{{N}}$:%  the following holds true for $\mathcal{V}$ (see definition \ref{def:charac}):
	\begin{equation}\label{eq:convexgames}
\mathcal{V}(S_1)\cup \mathcal{V}(S_2) \subseteq \mathcal{V}(S_1 \cup S_2) \cup\mathcal{V}(S_1 \cap S_2). 
%v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2).
\end{equation} 	
	% if for every player $n \in \mathcal{N}$, the marginal contribution of the player is non-decreasing W.R.T set inclusion. Mathematically, for $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash \{n\}$ 
	%\begin{equation}\label{eq:convexgames}
	%v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2).
	%\end{equation} 
\end{definition}
whereas $\mathcal{V}$ is given in  definition \ref{def:charac}.
\begin{theorem}\label{thm:convex}
	Our canonical game is cardinally convex. 
\end{theorem}
\begin{proof}
	%	Let us consider two coalition $S_1$ and $S_2$, where $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash\{j\}$, $j \in \mathcal{N}$, and  $\mathcal{F}_{S1}$ and $\mathcal{F}_{S1}$ are the feasible sets for $S_1$ and $S_2$ respectively. We calculate $v(S_2 \cup \{j\})-v(S_1 \cup \{j\})$ in Equation \eqref{eq:convexityProof}, where $u_j^{(S_1)}$ and $u_j^{(S_2)}$ are the utilities of player $j$ in $S_1$ and $S_2$ respectively.  
	Let us consider two coalitions $S_1$ and $S_2$ that are non-empty subsets of $\mathcal{N}$. Then from super-additivity of the game,    
	\begin{equation}
	\label{eq:superADD}
	\mathcal{V}(S_1)\cup\mathcal{V}(S_2) \subset \mathcal{V}(S_1 \cup S_2).
	\end{equation}
	%This is because the larger coalition $S_1 \cup S_2$ guarantees a pay-off at least as good as the sum of payoff attained when the two coalitions $S_1$ and $S_2$ are working alone (separately) due to super-additivity of  the game. 
Furthermore, due to the non-negative and non-decreasing nature of the utility used,
		\begin{equation}
	\label{eq:superADD2}
 \mathcal{V}(S_1 \cup S_2) \subseteq \mathcal{V}(S_1 \cup S_2) \cup\mathcal{V}(S_1 \cap S_2).
	\end{equation}
The proof follows. 	
	% $\mathcal{V}(S_1 \cap S_2)\geq0$ where  $\mathcal{V}(S_1 \cap S_2)=0$ if and only if $S_1 \cap S_2 =\emptyset$. The proof follows.  
\end{proof}

\begin{remark}
	The core of any convex game $(\mathcal{N}, \mathcal{V})$ is non-empty\cite{sharkey1982cooperative} and large \cite{maschler2013}. 
\end{remark}

\begin{remark}\label{lemma:MOOGame}
	Our canonical cooperative game $(\mathcal{N}, \mathcal{V})$ with NTU can be used to obtain the Pareto-optimal solutions for the multi-objective resource  allocation for various service providers.% problem given in \eqref{eq:opt_higher}.
\end{remark}
%Below, we discuss the game theoretic solution.% for the aforementioned two strategies. 
The convexity of our game proves that the core is non-empty. However, obtaining an allocation from the core is challenging, which  we address in the following subsection. 





\subsection{Proposed Algorithms}\label{sec:algorithms}

We first propose an efficient algorithm that provides  an allocation from the core. Then, we propose a second algorithm based on polygamous matching \cite{maschler2013} that obtains an allocation from the core subject to  resource fragmentation constraints  at the cost of higher computational complexity when compared with the first algorithm. Below we discuss these algorithms in detail. 
%\subsection{Game Theoretic Solution for Strategy 2}
%The calculation of Shapley value for our convex game requires at solving at least $2^{N}-1$ optimization problems. However, 
%The strategy $2$,
 %The value of coalition is  given by \eqref{eq:payoff_function}.
 

 
 
 
 
 
 
 % uncomment below for algorithm complexity
  % by solving $L|\mathcal{{G}}_1||\mathcal{{G}}_2|$ optimization problems where $L$ is the number of iterations required for the convergence of algorithm.   
 
\subsubsection{Game-theoretic Pareto Optimal Allocation}
  We propose a  computationally efficient algorithm,  Algorithm \ref{algo:alg2}, that obtains a Pareto-optimal allocation by solving $N+|\mathcal{{G}}_2|$ optimization problems, where $\mathcal{G}_2$ represents the set of players with resource surplus. Inputs are available resources/capacities, application requests and  utilities of all game players. The algorithm outputs an allocation. In Step 1,  utilities of  players, the allocation decision,  and vectors $\boldsymbol{v}$, $\boldsymbol{A}$ and $\boldsymbol{B}$ are initialized. $\boldsymbol{v}$ stores the utility each service provider achieves when working alone.  $\boldsymbol{A}$  stores the utility of players in $\mathcal{G}_2$ whereas  $\boldsymbol{B}$ stores the utility increase due to request satisfaction of applications in resource deficit group $\mathcal{G}_1$. 
   %that are used for storing utility values for different providers.   
     Step 2 calculates every player's utility in the absence of resource sharing, i.e., the single objective optimization problem in \eqref{eq:opt_single} is solved by every player. % and the values are stored in the vector $\boldsymbol{\theta}$. 
  To consider the resources allocated in Step 2, the remaining resource capacities and requests for various applications $C, R$ are updated and stored in $C'$ and $R'$, respectively.
  Step $4$ divides players into  two groups $\mathcal{G}_1$ (resource deficit) and $\mathcal{G}_2$ (resource surplus), on the basis of updated capacities and requests. Step $5$ allocates the shared resources of players in $\mathcal{G}_2$ to players in $\mathcal{G}_1$. 
 %  Players are divided in Step $4$  on the basis of updated capacities and requests into the aforementioned two groups $\mathcal{G}_1$ (resource deficit) and $\mathcal{G}_2$ (resource surplus), respectively.   
  % In Step $5$,  we obtain resource allocation decision and calculate the utilities players in $\mathcal{G}_2$ earn by sharing their resources with players in $\mathcal{G}_1$.  
    $\boldsymbol{z}^j$  denotes the total resources
  allocated to an application $j$ previously in Step $2$ and up to the current iteration of Step
 $5$. Up to this point, a given application $j$ can receive resources from multiple players due to resource sharing.
 % $\boldsymbol{z}^j$  represents total resources allocated to application $j$ prior to the current iteration of Step $5$ and in Step $2$. 
%  In step $6$,  players in $\mathcal{{G}}_2$ are assigned a payoff for allocating resources to applications $j \in \mathcal{{M}}_{\mathcal{G}_1}$. % using the rule specified in \eqref{eq:payoffrule}, i.e., the payoff received by players in $\mathcal{{G}}_2$ for providing resources to an application $j\in \mathcal{{M}}_{\mathcal{{G}}_1}$ depends on the fraction of resources provided by individual players in $\mathcal{{G}}_2$ and the native player for application $j$. %$P_n^j$ is the payoff player $n$ receives for allocating resources to application $j$ and $P_T^j$ is the total payoff obtained from allocating resources to application $j$.
   In step $6$, the utility reflecting an  increase in application satisfaction for native applications of players in $\mathcal{G}_1$ is calculated using the allocation obtained in Step $5$. 
   Below, we prove that Algorithm \ref{algo:alg2} provides an allocation from the core. 
%We also obtain the resource allocation decision. 


%$u_j^n$'s for all the players using \eqref{eq:opt_single_j} with $C', R'$ and store them in $\boldsymbol{O_2}$. 
\begin{comment}
\begin{figure*}
	\centering
	\includegraphics[width=0.97\textwidth]{figures/utility1}
	\caption{Utility of players in different settings.}
	\protect\label{fig:utilgeneral}
\end{figure*}

\begin{figure}
	\centering
	\includegraphics[width=.6\textwidth]{figures/coalition}
	\caption{Value of coalition in different settings.}
	\protect\label{fig:coalition}
\end{figure}



\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0, $ \boldsymbol{\phi} \leftarrow$0,  $ \boldsymbol{O_1} \leftarrow$0, $ \boldsymbol{O_2} \leftarrow$0 
		\State \textbf{Step $2$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_1^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step $3$:}  Update $C$ and $R$ based on Step 2 \\  $\quad \quad \quad \;  C'\leftarrow$ $C_{updated}$,$\; R'\leftarrow$ $R_{updated}$
		\State \textbf{Step $4$:} Divide the players into two subsets $\mathcal{S}_1$ and $\mathcal{S}_2$ representing players \\ with resource deficit and resource surplus
		\State \textbf{Step $5$:}
		\For{\texttt{$n \in \mathcal{S}_1$}}
		\State $ {O_2^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single_j}}
		\State Update $C'$ and $R',\quad$ $ C'\leftarrow$ $C'$,$\; R'\leftarrow$ $R'$
		\EndFor
		\State \textbf{Step $6$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
		\State \textbf{Step $7$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{$\mathcal{O}$($N$) algorithm for obtaining Core's allocation}
	\label{algo:alg2}
\end{algorithm}
\end{comment}
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of players' utility function  $\mathbf{u}$ 
	%	\newline  \hspace*{1cm} C 
		\State \textbf{Output}: $\mathbf{X}$ 
		\State \textbf{Step $1$:}  $ \mathbf{u}(\mathbf{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0,  $ \boldsymbol{v} \leftarrow$0, $\boldsymbol{A} \leftarrow$0, $\boldsymbol{B} \leftarrow$0, $\boldsymbol{z} \leftarrow$0 
		\State \textbf{Step $2$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {v(\{n\})}\hspace*{-0.1cm}\leftarrow$\texttt{Objective function value  of   \eqref{eq:opt_single}} 
		\State $  \mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}\leftarrow$\texttt{Allocation decision of \eqref{eq:opt_single}} 
		\State {Update $z^j$'s based on the allocation  decision of \eqref{eq:opt_single} } 
		\EndFor
		\State \textbf{Step $3$:}  Update $C$ and $R$ based on Step 2 \\  $\quad \quad \quad \;  C'\leftarrow$ $C_{updated}$,$\; R'\leftarrow$ $R_{updated}$
		\State \textbf{Step $4$:} Divide the players into two subsets $\mathcal{G}_1$ and $\mathcal{G}_2$ representing players  with resource deficit and resource surplus
		\State \textbf{Step $5$:}
		\For{\texttt{$n \in \mathcal{G}_2$}}
		\State 
		$\mathcal{X}_n\hspace*{-0.1cm}=\hspace*{-0.1cm}\mathbf{X}_n\backslash\{\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}\}\hspace*{-0.1cm}\leftarrow$
		\texttt{Optimal allocation decision of  \eqref{eq:opt_single_j} $\forall m \in \mathcal{{G}}_1$ }
    \State 		 {$ {A_{n}^j}\hspace*{-0.1cm} \leftarrow$ \texttt{Utility earned by $n \in \mathcal{{G}}_2$ due to resource allocation $\mathcal{X}_n$ }}
	\State {Update } $z^j${'s based on $\mathcal{X}_n$}
		\State Update $C'$ and $R'$%,\quad$ $ C'\leftarrow$ $C'$,$\; R'\leftarrow$ $R'$
		\EndFor
	%	\State \textbf{Step $6$:} $ {A_{n}^j}\hspace*{-0.1cm} \leftarrow$ \texttt{Utility earned by $n \in \mathcal{{G}}_2$ %using \eqref{eq:payoffrule} 
		%	$\forall j \in \mathcal{M}_{\mathcal{G}_1}$}
		\State \textbf{Step $6$:}
		\For{\texttt{$m \in \mathcal{G}_1$}}
		\State $ {B_{m}} \leftarrow$ \texttt{Utility earned by  satisfying users $j\in\mathcal{M}_m$  due to allocation decision in  Step $5$}
		%	\State $ {O_2^{(j)}} \leftarrow$ \texttt{$$}
		%	\State $ {X^{(n)}}\leftarrow$\texttt{Optimal allocation decision of  \eqref{eq:opt_single_j}} 
		%	\State Update $C'$ and $R'$%,\quad$ $ C'\leftarrow$ $C'$,$\; R'\leftarrow$ $R'$
		\EndFor
		
		%	\State \textbf{Step $6$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
		%	\State \textbf{Step $6$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
		%	\State \textbf{Step $7$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{Game-theoretic Pareto optimal allocation (GPOA)}
	\label{algo:alg2}
\end{algorithm}
%\begin{equation}
%\label{eq:payoffrule}
%P_n^j= \frac{\mathbf{x}_n^j}{\sum_{n \in \mathcal{{G}}_2}\mathbf{x}_n^j+\mathbf{x}^j_{native}}\times P_T^j, \quad \forall j \in \mathcal{{M}}_{\mathcal{{G}}_1}
%\end{equation}
\begin{comment}
\begin{figure*}
	\centering
	\includegraphics[width=1.0\textwidth]{figures/utility_all.eps}
	\caption{Player utilities working alone and in the grand coalition (GC) for different simulation settings.}% with $\mu=0.01$ and $\mu=0.1$.  }
	\protect\label{fig:util_all}
\end{figure*}
\end{comment}


\begin{theorem}\label{thm:alg1}
	The solution obtained from Algorithm \ref{algo:alg2}  lies in the \emph{core}.% provided that \eqref{eq:opt_single} and \eqref{eq:opt_single_j} are solved to global optimality.  
\end{theorem}
\begin{proof}
	To prove the theorem, we need to show that a)  utilities obtained using Algorithm \ref{algo:alg2}   are individually rational and  group rational, and b) no group of players  has the incentive to leave the grand coalition to form another sub-coalition $S \subset \mathcal{N}$. %	\indent
	\newline \indent\textbf{Individual Rationality:} (See definition \ref{def:indRational}) For each player $n \in \mathcal{N}$,  $v(\{n\})$ obtained by solving   \eqref{eq:opt_single} is the utility a player  obtains by working alone in the absence of resource sharing. Because the utilities are non-negative, $A_n\geq0,\;\forall n \in \mathcal{{N}}$.
	%	The value $A_n$ for $n \in \mathcal{G}_2$ in Step $5$ is either zero or positive but will not be negative due to the non-negative utility in use. 
	 Furthermore utilities of  players in $\mathcal{G}_1$ may increase due to  increase in request satisfaction if its applications are provided additional resources by players in  $\mathcal{G}_2$ given by $B_{n}$. 
%	\begin{align}
%u_n(R,\mathcal{X})&=O_1^n+O_2^n \quad \forall n \in \mathcal{N} \nonumber \\
%u_n(R,\mathcal{X})&\geq O_1^n \quad \forall n \in \mathcal{N}\nonumber 
%	\end{align}
	 Hence  Algorithm \ref{algo:alg2} produces an  individually rational resource allocation.
	\newline \indent\textbf{Group Rationality:} The value of the grand coalition $v\{\mathcal{N}\}$ as per Equation \eqref{eq:payoff_function} is the sum of different utilities. % $u_n$'s, $u_j^n$'s and $\sum_{j \in \mathcal{M}_n}\sum_{k \in \mathcal{K}} {x_{n,k}^{j}}/{r_{n,k}^{j}}$. 
	Steps $2$, $5$ and $6$ of Algorithm \ref{algo:alg2} obtain the sum of utilities as well. Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is group rational. 
	\par Furthermore, due to super-additivity of the game and monotonic non-decreasing nature of the utilities, no group of players has the incentive to form a smaller coalition. Hence Algorithm \ref{algo:alg2} provides a solution from the core.  
\end{proof}
%\subsubsection{Properties of $\mathcal{O}(N)$ Algorithm \ref{algo:alg2}}
%Algorithm \ref{algo:alg2} is a distributed algorithm as highlighted in Remark \ref{rem:distributed}. 

\begin{remark}\label{rem:distributed}
%	Algorithm \ref{algo:alg2} is a distributed algorithm, where players  exchange information related to resource requests  and capacities. Furthermore,  information regarding the order in which players execute Step $5$  also needs to be broadcast to all game players. \textbf{Edit as per Don's comments}

Algorithm \ref{algo:alg2} is a distributed algorithm. All players first allocate resources to their native applications and then update their capacities and requests. The updated requests and capacities are broadcasted by all players to obtain $\mathcal{{G}}_1$ and $\mathcal{{G}}_2$. The order to execute Step $5$ is chosen based on some criteria (see details below).  Players in $\mathcal{{G}}_2$, after allocating resources, send the updated requests  to other players in  $\mathcal{{G}}_2$  that have not yet executed Step $5$.

%where players  exchange information related to resource requests  and capacities. Furthermore,  information regarding the order in which players execute Step $5$  also needs to be broadcast to all game players.
\end{remark}
\begin{remark}\label{rem:paretooptimality}
	Any payoff allocation from the core  generated by Algorithm 1 is Pareto-optimal.  
\end{remark}
\begin{remark}\label{rem:forlooporder}
	The allocation decision obtained using Algorithm \ref{algo:alg2} always belongs to the core irrespective of the order in which players execute Step $5$. 
%	the \texttt{for-loop} of Step $5$ is executed. 
\end{remark}\vspace{-0.3in}
\begin{subequations}\label{eq:opt_single_j}
	\begin{align}
	\max_{\mathcal{X}_n}\quad& \sum_{m\in \mathcal{G}_1}\Bigg(\sum_{j \in \mathcal{M}_m}\bigg(w_1^j\big(u_n^j({\boldsymbol{z}}^j+\mathbf{x}_n^j)-u_n^j({\boldsymbol{z}}^j)-\nonumber \displaybreak[0]\\
	&D_n^j(\mathbf{x}_n^j)\big)+\sum_{k \in \mathcal{K}}\Big(\frac{x_{n,k}^j}{r_{m,k}^j-z_k^j}\Big)^2\bigg)\Bigg),\;  \forall n \in \mathcal{G}_2 \label{eq:objsinglej}\\
	\text{s.t.}\quad & \sum_{j} x_{n,k}^{j}\leq C'_{n,k}, \; \forall k \in \mathcal{K},  \forall j \in \mathcal{M}_m,  \forall m \in \mathcal{{G}}_1, \label{eq:singlefirstj} \displaybreak[0]\\
	& x_{n,k}^{j} \leq r^{'j}_{m,k}, \quad k \in \mathcal{K},  \forall j \in \mathcal{M}_m,  \forall m \in \mathcal{{G}}_1, \label{eq:singlesecondj} \displaybreak[1]\\
	&  x_{n,k}^{j} \geq 0, \quad  k \in \mathcal{K},  \forall j \in \mathcal{M}_m,  \forall m \in \mathcal{{G}}_1, \label{eq:singlethirdj} \displaybreak[2]\\
	& u_n^j({{z}}_k^j+{x}_{n,k}^j)-u_n^j({{z}}_k^j) \geq D_n^j({x}_{n,k}^j), \;  k \in \mathcal{K},   \nonumber \\
	& \forall j \in \mathcal{M}_m, \forall m \in \mathcal{{G}}_1. \label{eq:singlefourthj}
	\end{align}
\end{subequations}
%Algorithm \ref{algo:alg2} has different variants that can provide allocations from the core. 

Based on Remark \ref{rem:forlooporder}, it is  important to note that Algorithm \ref{algo:alg2} can generate different solutions according to the order in which players execute Step $5$. Some candidate ordering schemes listed below. 

%can be enhanced into different variants that can still provide allocations from the core. 
%These variants of the algorithm  arise depending on the order in which the \texttt{for-loop} in Step $5$ is executed, i.e., the order of  players in $\mathcal{{G}}_2$ to share their surplus resources to players in $\mathcal{{G}}_1$ with resource deficit. We list some of these variants below. 
\begin{enumerate}
%	\item \textbf{Decision maker}\footnote{The decision maker can be a separate entity or one of the players which is chosen to act as the \emph{``leader''}.} \textbf{order:}  A decision maker decides the order for executing the \texttt{for-loop} in Step $5$.
	%The capacity of specific player may be given more importance by the decision maker  when compared with other payers. Among many other reasons, this can be possibly because of the reliability of the resources of a certain player when compared with others. 
    \item \textbf{Capacity ascending order (CAO):} Players in $\mathcal{G}_2$ are arranged in an ascending order on the basis of the remaining capacities of a resource $k$, which is then used for executing  Step 5.  
	\item \textbf{Capacity  descending order (CDO):} Players in $\mathcal{G}_2$ are arranged in a descending order on the basis of the remaining capacities of a resource $k$, which is then used for executing  Step 5.  %The remaining capacity of players in $\mathcal{G}_2$ is used to descendingly sort them   and then the for-loop in Step $5$ is executed accordingly. 
	
	%The players in $\mathcal{G}_2$, on the basis of their remaining capacity, are arranged in a descending order. The \emph{for-loop} in Step $5$ is then executed in the obtained descending order.
	\item \textbf{Random Order:} The order in which players execute  Step $5$ is random. 
\end{enumerate}


While all these variants provide allocations from the core, finding the most beneficial order for the \texttt{for-loop} in Step $5$ requires evaluating all possible combinations of possible orders for executing the for-loop. 
Since Algorithm \ref{algo:alg2} always provides an allocation from the core,
it is desirable to identify the order of surplus players considered in Step $5$ that also considers physical constraints such as
resource fragmentation across multiple players (service providers).
Toward this goal, we present below a matching-based resource
sharing algorithm that further reduces resource fragmentation while
providing an allocation from the core.





\subsubsection{Polyandrous-Polygamous Matching for Resource Sharing}
Our proposed algorithm is based on polyandrous polygamous matching \cite{baiou2000many} that matches players (service providers) in $\mathcal{{G}}_1$ to $\mathcal{{G}}_2$ with the goal of maximizing utility for players in  $\mathcal{{G}}_2$ and reducing  resource fragmentation for supporting native applications from players  in $\mathcal{{G}}_1$. The idea behind our matching algorithm, inspired from \emph{two-sided markets} \cite{maschler2013}, for reducing resource fragmentation is as follows. 
%Players in $\mathcal{{G}}_1$ are the sellers (due to resource deficit, they need to "sell" their applications to MECs in $\mathcal{{G}}_2$) whereas the players in 
Players in $\mathcal{{G}}_1$ have specific preferences for which  players in $\mathcal{{G}}_2$ they would like to obtain resources from. 
 %can share their resources to satisfy applications of players in $\mathcal{{G}}_1$, i.e., $\mathcal{{G}}_1$ players prefer to delegate their applications to player(s) in $\mathcal{{G}}_2$ that can  preferably satisfy  most of the requests, resulting in reduced resource fragmentation.  
 On the other hand, players in $\mathcal{{G}}_2$ aim to maximize their utilities. As our framework relies on  monotonic non-decreasing utilities, the objectives of players in  $\mathcal{{G}}_1$ and $\mathcal{{G}}_2$ can be mapped to each other, i.e., the more  resources players in $\mathcal{{G}}_2$ share with players in $\mathcal{{G}}_1$, the higher  will their utilities  be and the lower  the resource fragmentation will be. Therefore, during each round, resources of one player in $\mathcal{{G}}_2$ are assigned to applications of a player in $\mathcal{{G}}_1$ that produces the largest increase in its utility. This  means that a $\mathcal{{G}}_2$ player will provide as many resources as possible (increasing its utility) that in turn should reduce resource fragmentation for applications in $\mathcal{{G}}_1$. From resource fragmentation perspective, our scheme will transform into \emph{polygamous}/many-to-one matching \cite{maschler2013} or \emph{stable marriage}/one-to-one matching\cite{gale1962college} in the best case scenario.   
%are the sellers (due to resource deficit, they need to "sell" their applications to MECs in $\mathcal{{G}}_2$) whereas the players in 
Below, we discuss the different steps of the algorithm. 
 \par 
In Algorithm \ref{algo:algPoly}, all  variables are initialized in Step $1$.  $\boldsymbol{z}$ is a vector that stores  allocations for  every application $j \in \mathcal{{M}}$ across different players.  In Step $2$, all game players $n \in \mathcal{N}$ allocate resources to their native applications. Request matrices and capacity vectors are updated in Step $3$, and  players are divided into two groups $\mathcal{{G}}_1$ and $\mathcal{{G}}_2$ in Step $4$.  Here $\boldsymbol{A}$ and $\boldsymbol{B}$ records utilities of   players in $\mathcal{{G}}_2$ and $\mathcal{{G}}_1$, respectively. Step $5$ is  the core of  the algorithm. In Step $5a$, Algorithm \ref{algo:matrixConstruction} is used to construct a matching matrix $\mathcal{J}$. % as follows. 
%\paragraph{Constructing the matching matrix $\mathcal{J}$:}
The elements of matching matrix $\mathcal{J}$  ($m$ rows and $n$ columns) are obtained by solving and obtaining the objective function value of the the problem in \eqref{eq:opt_matching} for every possible pair of $(m\in\mathcal{G}_1, n \in \mathcal{{G}}_2)$. \eqref{eq:opt_matching} maximizes the incremental utility a player in $\mathcal{{G}}_2$ earns by sharing its resources with a player in $\mathcal{{G}}_1$, whereas the second summation term is used to reduce resource fragmentation. 
%The objective function \eqref{eq:objmatching} aims to maximize the incremental utility a player $n\in\mathcal{{G}}_2$ earns by sharing its resources with application of $m \in \mathcal{{G}}_1$. 
\eqref{eq:matchingfirst} indicates that the allocated resources cannot exceed the capacity. \eqref{eq:matchingsecond} indicates that the allocation cannot be more than the required resources. \eqref{eq:matchingthird} shows that the allocation decision is non-negative whereas \eqref{eq:matchingfourth} indicates that the incremental increase in utility cannot be less than the communication cost.% We also store the  resources allocated  in the matrix $\mathcal{R}$. 

%Each player $n \in \mathcal{G}_2$ calculates the 
%\textbf{Discuss the construction of matching matrix.}

Algorithm \ref{algo:matrixConstruction} also provides  total amount of resources used for each element of  $\mathcal{J}$  and allocation decision $^{m}X_n$ that captures how resources are allocated to all applications $j \in \mathcal{{M}}_m$ for $m \in \mathcal{{G}}_1$ at player $n \in \mathcal{{G}}_2$. %The matching matrix is constructed by solving \eqref{eq:opt_matching} for each $m \in \mathcal{{G}}_1$ and $\mathcal{{G}}_2$. %, and then assigning payoffs using \eqref{eq:payoffrule2}, where  $\boldsymbol{z}^j$ captures the resources allocated to application $j$ at different players in $\mathcal{{G}}_2\backslash n.$ 
In $5b$, the largest element in $\mathcal{J}$, given by $\mathcal{J}_{m,n}$,  is used to match $m$ to $n$, i.e., the player $n$ (with resource surpluses) shares its resources with the player $m$ (with resource deficits).
If there are multiple maximum values, then the one that uses smallest number of resources is used to choose the matching.  In $5c$, applications $j \in \mathcal{{M}}_m$ are assigned to $n \in \mathcal{{G}}_2$. In $5d$, $\boldsymbol{A}_n$ is updated with the  utility of player $n \in \mathcal{G}_2$ based on the assignment in $5c$. Similarly,  $\boldsymbol{B}_m, \mathcal{X}_n$ and $\boldsymbol{z}^j$ are updated to reflect the increase in application satisfaction,  resources allocated by $n$ to different applications and resources allocated to $j \in \mathcal{{M}}_m$, respectively. Requests and capacities are updated in $5e$ whereas $5f$ updates elements of $\mathcal{{G}}_1$ and $\mathcal{{G}}_2$ if required. 

%We propose  \emph{Polygamous Matching based Pareto Optimal Allocation} (PMPOA),
%We first consider the case when the resource deficit players prefer that the resources allocated to them by resource surplus players are  not highly fragemented across different players in $\mathcal{G}_2$. For such a case, we first propose \emph{Polygamous Matching based Pareto Optimal Allocation} (PMPOA), 
%a \emph{polygamous matching} \textbf{(add reference to the game theory book)} based algorithm that provides an allocation from the core as given in Algorithm \textbf{(add algorithm)}.  The input into the algorithm are available resources/capacities, application requirements and the utilities of all game players. The output of the algorithm is $\mathcal{X}$.  In Step 1, the utilities of the players, the allocation decision,  and vectors $\boldsymbol{v}$, $\boldsymbol{O}^1$ and $\boldsymbol{O}^2$ are initialized. In Step 2, every player's utility is calculated without any resource sharing, i.e., the single objective optimization problem is solved by every player and the values are stored in the vector $\boldsymbol{O}^1$. Then $C, R$ are updated and stored in $C'$ and $R'$, respectively. 

%\paragraph{Properties of Algorithm \ref{algo:algPoly}}


\begin{definition}{Objection to a matching\cite{maschler2013}:}
	A player $m \in \mathcal{{G}}_1$ and  $n \in \mathcal{{G}}_2$ object to a matching $M$ if they both  prefer being matched to each other than to whom  they are matched by $M$. 
\end{definition}

\begin{definition}{Stable matching\cite{maschler2013}:}
A matching $M$ is stable if there is no pair $m \in \mathcal{{G}}_1$ and   $n \in \mathcal{{G}}_2$ that objects to a matching. 
\end{definition}



%\begin{definition}{Stable matching\cite{maschler2013}}
%A matching $M$ is stable if in every case that player $m \in \mathcal{{G}}_1$ prefers another  player $n' \in \mathcal{{G}}_2$ to the player $n \in \mathcal{{G}}_2$ to which player $m$ is matched, 
%\end{definition}
\begin{theorem}
	The polyandrous-polygamous matching in Algorithm \ref{algo:algPoly} is stable. 
\end{theorem}
\begin{proof}
	We prove this by contradiction. Assume that the matching $M$ obtained from Algorithm \ref{algo:algPoly} is not stable and there exists  a pair $(m \in \mathcal{{G}}_1, n \in \mathcal{{G}}_2)$ that objects to the matching. $M$ has originally matched $m \in \mathcal{{G}}_1$ to $n'$ and $n \in \mathcal{{G}}_2$ to $m'$. 
	The objection by $n$ means that it can achieve a higher utility by being matched with $m$ when compared with the current match $m' \in \mathcal{{G}}_1$. However, this is not possible as  $m'$ was matched with $n$ based on the maximization problem given in \eqref{eq:opt_matching}, i.e., $m'$ provides  the highest utility to $n$ for its resources. % obtained using Algorithm \ref{algo:algPoly}. 
	%Similarly, the objection by  $m\in \mathcal{{G}}_1$ to the matching means that it can be allocated larger amount of resources by being matched with $n$ when compared with the current match $n' \in \mathcal{{G}}_2$.  However,  $m$ was matched with $n'$ because $n'$ provided the largest amount of resources to $m$ and $m$ in return  provided $n'$ with the larger utility (due to non-decreasing nature of the utility used). 
	Hence, our assumption is wrong and the matching is stable. 
	
	% Algorithm \ref{algo:algPoly} matches players $m \in \mathcal{{G}}_1$ with  $n \in \mathcal{{G}}_2$ using the maximization problem in \eqref{eq:opt_matching}. 
	 
	 
	 %considering the objectives of both parties, i.e., providing as many resources as possible (reducing resource fragmentation) for $m$ and causing the largest increase in utility of $n$ (\eqref{eq:opt_matching} is a maximization problem), no pair $(m, n)$ can object to the matching. Hence, the matching is stable. 
\end{proof}
\begin{remark}\label{rem:alg2}
	Algorithm \ref{algo:algPoly} provides an allocation from the core.% provided that \eqref{eq:opt_single} and \eqref{eq:opt_matching} are solved to global optimality. %as it guarantees individual and group rationality along with stability of the coalition.
\end{remark}
\vspace{-0.1in}
\begin{remark}
The  optimization problems in \eqref{eq:opt_single}, \eqref{eq:opt_single_j} and \eqref{eq:opt_matching} are non-convex. The hardness of these problems depend on the parameters such as the utility functions, requests and capacities. Therefore, it is difficult to evaluate the hardness of these problems, but the instances we consider  in Section \ref{sec:exp_results} are easily solved using existing solvers.
In general, certain  non-convex optimization problems can usually be solved to  optimality by proving that the \emph{strong duality} holds \cite{boyd2004convex},  and then solving the convex dual of these non-convex problems. Detailed discussions on strong duality can be found in \cite{boyd2004convex} whereas \cite{tychogiorgos2013non} presents the necessary and sufficient conditions for strong duality of non-convex problems. If the optimal solutions are not found for  \eqref{eq:opt_single}, \eqref{eq:opt_single_j} or \eqref{eq:opt_matching}, then the allocation will not be from the core. 
\end{remark}

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of players' utility function  $\mathbf{u}$ 
		%	\newline  \hspace*{1cm} C 
		\State \textbf{Output}: $\mathbf{X},$  $\mathbf{u}(\mathbf{X})$
		\State \textbf{Step $1$:}  $ \mathbf{u}(\mathbf{X}) \leftarrow0$,  $ \mathbf{X} \leftarrow0$,  $ \boldsymbol{v} \leftarrow0$, $[\mathcal{J}]_{|\mathcal{{G}}_1|\times |\mathcal{{G}}_2|}\leftarrow\mathbf{0}, \boldsymbol{z}\leftarrow\mathbf{0}$  
		\State \textbf{Step $2$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {v(\{n\})}\leftarrow$\texttt{Objective function value  from  Equation \eqref{eq:opt_single}} 
		\State $ \mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}\hspace*{-0.12in}\leftarrow$\texttt{Allocation decision from \eqref{eq:opt_single}} 
			\State {Update $z^j$'s based on the allocation  decision of \eqref{eq:opt_single} } 
		\EndFor
		\State \textbf{Step $3$:}  Update $C$ and $R$ based on Step 2 \\  $\quad \quad \quad \;  C'\leftarrow$ $C_{updated}$,$\; R'\leftarrow$ $R_{updated}$
		\State \textbf{Step $4$:} Divide the players into two subsets $\mathcal{G}_1$  and \hspace*{0.5in} $\mathcal{G}_2$ representing players  with resource deficit and \hspace*{0.55in}resource surplus \\$\quad\quad  \quad \quad \boldsymbol{A} \leftarrow0$, $\boldsymbol{B} \leftarrow0$
		\State \textbf{Step $5$:} 
		\NoDo
		\While  $\quad \mathcal{{G}}_1\neq \emptyset\quad  ||\quad \mathcal{{G}}_2 \neq \emptyset$
		\State
		%{Construct matching matrix $\mathcal{J}_{|\mathcal{{G}}_1|\times |\mathcal{{G}}_2|}$ using Algorithm \ref{algo:matrixConstruction}}
		\textbf{Step $5a$: }{$[\mathcal{J}]_{|\mathcal{{G}}_1|\times |\mathcal{{G}}_2|}\leftarrow$  Algorithm \ref{algo:matrixConstruction} for constructing\\ matching matrix}
	%	\State
	\State \textbf{Step $5b$: }
		\If  {Multiple maximum values in $[ \mathcal{J}]$}\\
		 {\hspace*{0.35in} Choose one with the lowest $\mathcal{R}_{m,n}$}
		\Else{}\\
	 { \hspace*{0.4in}Obtain the row $m$ and column $n$ of the  maximum \hspace*{0.4in} value in  $[\mathcal{J}]$}
		\EndIf
		\State {\textbf{Step $5c$: }Assign all $j \in \mathcal{{M}}_m, m \in \mathcal{{G}}_1$ to $n \in \mathcal{{G}}_2$ }
		\State {\textbf{Step $5d$: }Update $\boldsymbol{A}_n, \boldsymbol{B}_m, \mathcal{X}_n $ and $\boldsymbol{z}^j$ using the preceding assignment}
	%	\State {$\boldsymbol{\theta}_n\leftarrow$Update utility of $n \in \mathcal{{G}}_2, \boldsymbol{\zeta}^j$}
		\State\textbf{Step $5e$: } Update $C_n$  and $R_m$
		\State \textbf{Step $5f$: }
		\If  \texttt{ $C_n=0,$}\\
		\quad \quad \quad {$\;\mathcal{{G}}_2=\mathcal{{G}}_2\backslash n$}
		\EndIf
			\If  \texttt{ $R_m=0,$}\\
		\quad \quad \quad {$\;\mathcal{{G}}_1=\mathcal{{G}}_1\backslash m$}
		\EndIf
		\EndWhile
	\end{algorithmic}
	\caption{Polyandrous-Polygamous Matching based Pareto Optimal Allocation (PPMPOA)}
	\label{algo:algPoly}
\end{algorithm}

%\begin{equation}
%\label{eq:payoffrule2}
%P_n^j= \frac{\mathbf{x}_n^j}{\boldsymbol{\zeta}^j+\mathbf{x}_n^j+\mathbf{x}^j_{native}}\times P_T^j, \quad \forall j \in \mathcal{{M}}_{\mathcal{{G}}_1}
%\end{equation}
\begin{subequations}\label{eq:opt_matching}
	\begin{align}
	\max_{^{m}\mathbf{X}_n}\quad& \sum_{j \in \mathcal{M}_m}\Big(w_1^j\big(u_n^j({\boldsymbol{z}}^j+\mathbf{x}_n^j)-u_n^j({\boldsymbol{z}}^j)-D_n^j(\mathbf{x}_n^j)\big)+\nonumber \\
	& \sum_{k \in \mathcal{K}}\Big(\frac{x_{n,k}^j}{r_{m, k}^j-{z}_k^j}\Big)^2\Big),%\mathcal{X}) %+\sum_{i \in {M}_j}\sum_{k \in \mathcal{K}}\frac{x_{ik}^{(n)}}{r_{ik}^{(j)}}\bigg)
\label{eq:objmatching}\\
	\text{s.t.}\quad & \sum_{j} x_{n,k}^{j}\leq C'_{n,k}, \; \forall k \in \mathcal{K},  \forall j \in \mathcal{M}_m,  \label{eq:matchingfirst} \displaybreak[0]\\
	& x_{n,k}^{j} \leq r^{'j}_{m,k}, \quad k \in \mathcal{K},  \forall j \in \mathcal{M}_m, \label{eq:matchingsecond} \displaybreak[1]\\
	&  x_{n,k}^{j} \geq 0, \quad  k \in \mathcal{K},  \forall j \in \mathcal{M}_m \label{eq:matchingthird} \displaybreak[2]\\
	& u_n^j({{z}}_k^j+{x}_{n,k}^j)-u_n^j({{z}}_k^j) \geq D_n^j({x}_{n,k}^j), \;  k \in \mathcal{K},  \nonumber \\
	&\forall j \in \mathcal{M}_m. \displaybreak[2] \label{eq:matchingfourth}
	\end{align}
\end{subequations}
%\vspace{-0.2in}
%\paragraph{Properties of Algorithm }

\begin{lemma}
	Our resource sharing framework improves request satisfaction. 
\end{lemma}
\begin{proof}
	Let the average application request satisfaction for the non-resource sharing case be given by $RS_{n,1}$, where $RS_{n,1}$ is obtained following the resource allocation decision in Step $2$ of Algorithms \ref{algo:alg2} and \ref{algo:algPoly}, $\forall n \in \mathcal{{N}}$. As players in $\mathcal{{G}}_2$ share their resources with 
	players in $\mathcal{{G}}_1$,  average user satisfaction as a result of the allocation,  given by $RS_{n,2}$ is also  positive, i.e., $>0$. Hence,  user satisfaction achieved using our framework is given by $RS_{n}=RS_{n,1}+RS_{n,2}$, where $RS_{n}\ge RS_{n,1}$.  
\end{proof}
%\vspace{-0.3in}
\subsection{Strategy-Proof Incentive}
In this section, we answer the question: \emph{Is there an incentive for a single player or group of players to cheat and report incorrect capacities and application requests  to other players?} That is, will misreporting the capacities or application requests improve the payoff a player or group of players receive? 
The answer is no as given by the following Theorem. 
%Of course, it is possible to have a policing mechanism that enforces truthfulness among game players. However, it is interesting to see if our algorithms can enforce truthfulness without the need for any policing mechanism. 
\begin{theorem}
	When the service providers use Algorithms \ref{algo:alg2} and \ref{algo:algPoly} for resource sharing and allocation, no player or group of players has any incentive to cheat and misreport  capacities  and application requests, i.e., each player $n \in \mathcal{{N}}$ can achieve the highest payoff by truthfully reporting its capacity and requests.
\end{theorem}
\begin{proof}
Assume a player $n \in \mathcal{{N}}$ improves its  utility $\mathcal{U}_n$ by misreporting its capacity  and application requests, i.e.,   $\mathcal{U}'_n>\mathcal{U}_n$ where $\mathcal{U}'_n$ is the utility obtained by cheating and $\mathcal{U}_n$ is the utility obtained by truthful reporting. Each player receives its payoff for providing resources to its own applications first and then sharing the remaining resources (if any) with the applications of other service providers. Player payoff improves once  resources are provided and user requests are satisfied. 
    \begin{figure*}[h!]
	\centering
	\includegraphics[width=1.2\textwidth]{three3}	%\vspace{-0.5in}
	\caption{Performance of our framework with Algorithm \ref{algo:alg2} for $3$ player - $3$ application settings.}% and $\mu=0.01$.  }
	\protect\label{fig:sat11}
	\vspace{-0.1in}
\end{figure*}

\begin{figure*}[h!]
	\centering
	\includegraphics[width=1.2\textwidth]{three20}%	\vspace{-0.5in}
	\caption{Performance of our framework with Algorithm \ref{algo:alg2} for $3$ player - $20$ application settings.}% and $\mu=0.01$.  }
	\protect\label{fig:sat12}
	\vspace{-0.1in}
\end{figure*}
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ $\mathbf{u}, \boldsymbol{z}$ 
		%	\newline  \hspace*{1cm} C 
		\State \textbf{Output}: $\mathcal{J}, \mathcal{R},^{m}\hspace*{-0.05in}\boldsymbol{X}_n$
		\For{\texttt{$n \in \mathcal{G}_2$}}
		\For{\texttt{$m \in \mathcal{G}_1$}}
		\State \texttt{$\mathcal{J}_{m,n}\leftarrow$ Payoff for allocation \hspace*{0.4in} decision from \eqref{eq:opt_matching} }
		\State \texttt{$\mathcal{R}_{m,n}\leftarrow$ Resources allocated in \eqref{eq:opt_matching} }
		\EndFor
		\EndFor
	\end{algorithmic}
	\caption{Constructing matching matrix $\mathcal{J}$ }
	\label{algo:matrixConstruction}
\end{algorithm}
The larger the amount of resources provided and requests satisfied, the higher the obtained payoff will be. There are two cases for cheating:
\begin{itemize}
	\item \textbf{Under-reporting\footnote{Reporting a lower value than the actual value.} the capacity and application requests:} In this case, the player will not receive the  payoff possible by satisfying  its applications and fully utilizing its capacity by allocating resources to its own applications and applications of other players. This contradicts the assumption that $\mathcal{U}'_n>\mathcal{U}_n$. Hence, the player has no incentive to under-report its capacity and application  requests. % and the player will receive a payoff $\mathcal{U}'_n$ which will be less than $\mathcal{U}_n$. 
	\item \textbf{Over-reporting\footnote{Reporting a larger value than the actual value.}  the capacity and application requests:}  Since the payoff depends on the actual amount of resources provided and requests satisfied rather than the reported capacity and application requests, the highest payoff possible for the player is $\mathcal{U}_n$ contradicting our assumption that  $\mathcal{U}'_n>\mathcal{U}_n$.     	\vspace{-0.1in}
\end{itemize}

\begin{comment}
There exits four different sub-cases for cheating:
\begin{enumerate}
	\item Reporting a larger capacity vector and smaller request matrix: A player reporting larger capacity vector and smaller request matrix will share 
	\item Reporting a larger capacity vector and larger request matrix:
	\item Reporting a smaller capacity vector and smaller request matrix:
	\item Reporting a smaller capacity vector and larger request matrix:
\end{enumerate}
\end{comment}
\end{proof}
%Furthermore, carefully observing  Step $5$ in Algorithm \ref{algo:alg2} will show that the order for the \emph{for-loop} can provide us with different variants of resource allocation. Therefore, below we discuss two different sub-classes of possible implementations of Step $4$.
\begin{comment}
\paragraph{Decision maker enforced hierarchy}
For decision maker enforced hierarchy,  the order for the players to solve \eqref{eq:opt_single_j} is decided by a decision maker. The decision maker can be a separate entity or one of the players which is chosen to act as the \emph{``leader''}. Among many, the three possible scenarios  that can be used to decide the order of players in Step $5$ are:
\begin{enumerate}
	\item Request based hierarchy (RBH): The request for resources by applications of a specific player may be given more importance by the decision maker (can be due to any possible reason) when compared with other payers. Therefore,  the DM assigns order of players for Step $5$ in Algorithm \eqref{algo:alg2} on the basis of satisfying the requests of applications of players arranged in descending order on the basis of the ``importance''. 
	\item Capacity based hierarchy (CBH): The capacity of specific player may be given more importance by the decision maker  when compared with other payers. Among many other reasons, this can be possibly because of the reliability of the resources of a certain player when compared with others. 
	\item Decision maker's decision (DMD): In the last scenario,   the decision maker decides the order for the step $5$ on the basis of personal preferences or some particular protocol other than RBH and CBH.
\end{enumerate}
\paragraph{Quantity enforced hierarchy}
The second sub-class of schemes that can be used for the \emph{for-loop} in Step $5$ (for the order in which players run \eqref{eq:opt_single_j}) is based on either the quantity of resources requested or the remaining available capacities as discussed below:
\begin{enumerate}
	\item Request based ascending order (RBAO): The players, on the basis of remaining requests of the applications, are arranged in an ascending order. 
	\item Request based descending order (RBDO): The players, on the basis of  remaining requests of the applications, are arranged in an descending order. 
	\item Capacity based ascending order (CBAO): The players, on the basis of their remaining capacity, are arranged in an ascending order. 
	\item Capacity based descending order (CBDO): The players, on the basis of their remaining capacity, are arranged in an descending order. 
\end{enumerate}
The final scheme is randomly choosing the players for Step $5$, which we refer to as random scheme (RS). 
\begin{remark}\label{rem:convexcore}
	All the aforementioned schemes provide an allocation from the core. Since the core is a convex set, any convex combination of the allocation obtained through any two of the aforementioned schemes will also lie in the core. 
\end{remark}
\end{comment}
%The order in which the 
%We identify two broad classes of algorithms 



%In the next section, we evaluate the performance of our resource sharing and allocation framework. 








==> strategy-2 arxiv/03-opt-problem2.tex <==
In this section, we first present the resource allocation problem for a single service provider (no resource sharing with other service providers). Then we present the MOO problem for resource sharing and allocation. %For a single domain $n \in \mathcal{N}$ (without being part of coalition), the optimization problem is given in Equation~\eqref{eq:opt_single}
For a single cloud  $n \in \mathcal{N}$ (not  part of a coalition), the allocation decision matrix $X_{SO}^{(n)}$, where $SO$ stands for single objective,  is given by: 

\begin{equation}
\label{eq:X_n}
X_{SO}^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{{M}_n}}^{(n)}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{{M}_n}1}^{(n)}&\cdots  &\cdots   & x_{{{M}_n}{K}}^{(n)}
\end{smallmatrix}\Biggr].
\end{equation}
%where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$. 



The optimization problem is: %given in Equation~\eqref{eq:opt_single}
\begin{subequations}\label{eq:opt_single}
	\begin{align}
	\max_{{X}_{SO}^{(n)}}\quad& u_n({X}_{SO}^{(n)})+ \sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}} \frac{x_{ik}^{(n)}}{r_{ik}^{(n)}} \quad \forall n \in \mathcal{N}, \label{eq:objsingle}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}_n, \label{eq:singlefirst} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq r^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecond} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}. \label{eq:singlethird} \displaybreak[2]
	\end{align}
\end{subequations}
The goal of this single objective optimization problem for every service provider is   to  maximize its utility by allocating available resources only to its own applications. $\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}} {x_{ik}^{(n)}}/{r_{ik}^{(n)}}$ captures the satisfaction of resource requests by applications.  %The first constraint \eqref{eq:singlefirst} indicates that the allocated resources to all the users $i \in \mathcal{M}_n$ cannot be more than the capacity. The second constraint \eqref{eq:singlesecond} indicates that the allocated resources cannot be more than the required resources, while the final constraint \eqref{eq:singlethird} indicates that the allocation cannot be negative.  
\par Next, we present the resource allocation problem for different service providers that share their resources with each other. In the resource sharing case,  each service provider aims to  maximize sum of utilities obtained by a) allocating resources to its native applications, i.e., $u_n({X}_{i \in \mathcal{M}_n}^{(n)})$;  b) allocating resources to  applications of other service providers, i.e.,  $u_j^n({X}_{i \in \mathcal{M}_j}^{(n)}),\; \forall j\in \mathcal{N}\backslash n$; and c) satisfying requests of applications. This leads to: 
%For the cooperative case, we aim to maximize the utility of our coalition in Equation~\eqref{eq:opt_higher}.  First constraint in Equation~\eqref{eq:obj1} indicates that the allocated resources cannot be more than the capacity. The second constraint \eqref{eq:obj2}  indicates that the allocated resources cannot be more than the required resources. The last constraint \eqref{eq:obj3}  implies that allocation decision can't be negative. 
\begin{subequations}\label{eq:opt_higher}
	\begin{align}
	\max_{\mathcal{X}}\quad&  \bigg(w_nu_n({X}_{i \in \mathcal{M}_n}^{(n)})+\zeta_{n} \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})+\nonumber \\
	&\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \mathcal{{N}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg) \quad \forall n \in \mathcal{N}, \label{eq:obj}\\ %\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in \mathcal{N},j\neq n}  u^{n}_j(\mathcal{X})\bigg) \quad \forall n \in \mathcal{N} \label{eq:obj}\\%\{u_1(\mathcal{A}),u_2(\mathcal{A}),\cdots,u_N(\mathcal{A})\} \label{eq:obj}\\%U(A)\label{eq:obj}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K},  \forall n \in \mathcal{N}, \forall i \in \mathcal{M}, \label{eq:obj1} \displaybreak[0]\\
	& \sum_{j \in \mathcal{N}}x_{ik}^{(j)} \leq r^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N},  \label{eq:obj2}\displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}. \label{eq:obj3} \displaybreak[2]
	\end{align}
\end{subequations}
The first constraint in both optimization problems, \eqref{eq:opt_single}  and \eqref{eq:opt_higher}, indicates that the allocated resources cannot be more than the capacity. The second constraint  in \eqref{eq:singlesecond} and \eqref{eq:obj2} indicates, that the allocated resources should not be more than the required resources.  The last constraint, \eqref{eq:singlethird} and \eqref{eq:obj3},  indicates that allocation decision cannot be negative. 

%The utility $u_n({X}_{i \in \mathcal{M}_n}^{(n)})$ given in \eqref{eq:obj}, that each player receives, is a payment that all users $i \in \mathcal{M}_n$  who use the resources pay the player. %Users of other domains $j \in \mathcal{N}\backslash n $ that use resources of domain $n$  will be charged at a rate that player $j$ would have charged the user $i \in \mathcal{M}_j$, had the request been fulfilled by player $j$. Hence, 
%$u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})$ is the utility that domain $n$ receives for sharing its resources with domain $j$. 
$w_n$ is the weight associated with the utility $u_n$ and $\zeta_n$ is the weight affiliated with all $u_j^n$. 
%\begin{itemize}
% so that each enclaves first facilitates its own users and then assign the remaining resource to the users of other enclaves. $w_n +w'_{n}=1$  where $w_n > w'_{n}$. E.g., $w_n=0.8$ and $w'_{n}=0.2$ would mean that each enclave has an incentive to first satisfy its own users (higher utility) and then share the excess resources for other users $j \in \mathcal{N}\backslash n $
%	\item The utility $u_n(\mathcal{X})$ in Equation~\eqref{eq:opt_higher} that each player receives can be thought of as a payment that all users $ \in \mathcal{M}_n$  who use the resources pay the player. The remaining available resources at domain $n$ 	can be used by users of other domains $j \in \mathcal{N}\backslash n $ that will be charged at a rate that player $j$ would have charged the user $i \in \mathcal{M}_j$ had the request been specified by player $j$. $u^{n}_j(\mathcal{X})$ is the utility that domain $n$ receives for sharing its resources with player $j$. There are different ways to capture this profit. However, for now, we can say that it would be equivalent to whatever domain $j$ would have earned had it satisfied the requests itself (however it can't as it does not have resources, so it borrows resources from domain $n$ and assigns all the profit it gains from the users to player $n$).
%	\item  $w_n$ is the weight assigned to the utility of player $n$. $\zeta_n$ is the weight assigned to the utility $u^{n}_j(\mathcal{X})$. 
%\end{itemize}
In this paper, we assume that utility of the service providers is a non-decreasing monotone function. %This is because in  cloud computing system,  the more the resources provided, the higher is the gain or utility for the service provider.
% It is highly unlikely that the utility of any service provider will decrease with an increase in the amount of resources allocated. 
 We also assume that a subset $\mathcal{N}_1 \subset \mathcal{N}$ of service providers has resource surplus, while a subset $\mathcal{{N}}_2 \subset \mathcal{N}$ has a resource deficit. %Furthermore, we also assume that for any player $i \in \mathcal{{N}}_1$, $R^{(i)}> C^{(n)},\; \forall n \in \mathcal{{N}}_2$, i.e., no single player in $\mathcal{{N}}_2$ has a resource surplus that is more than the resource deficit of a player in $\mathcal{{N}}_1$.  

\subsection{Game Theoretic Solution}
As mentioned earlier, %To obtain the solution for the MOO problem in \eqref{eq:opt_higher}, 
we model each cloud service provider as a player in our game to obtain the solution for the MOO problem in \eqref{eq:opt_higher}. Let $\mathcal{N}$ be the set of players that can play the resource sharing and allocation game. The \emph{value of coalition} for the game players $S \subseteq \mathcal{N}$ is given by \eqref{eq:payoff_function}, where $\mathcal{F}_S$ is the feasible set. 
% The characteristic function $v(S)$ in \eqref{eq:payoff_function} captures the \emph{value of coalition} of game players in $S \subseteq \mathcal{N}$, where $\mathcal{F}_S$ is the feasible set. 

%The characteristic function $v(S)$ in \eqref{eq:payoff_function} for our game  with feasible set $\mathcal{F}_S$, that solves  problem in~\eqref{eq:opt_higher}. 
%\begin{figure*}[!t]
%	\normalsize
\begin{align} \label{eq:payoff_function}
v({S})&=\sum_{{\substack{{n \in S}\\ {\mathcal{X} \in \mathcal{F}_S}}}}    %{\substack{\text{$n \in \mathcal{N}$} \\ \text{$C_{k}= \sum_{n \in \mathcal{N}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in \mathcal{N}$}\\ \text{$\sum_{j \in \mathcal{N}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}$}}}  
\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{\substack{j \in {S},\\j\neq n}} u^{n}_j(\mathcal{X})+\nonumber \\
&\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \mathcal{{S}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg).
\end{align}
%	\hrulefill
%	\vspace*{-4pt}
%\end{figure*}
 The payoff each player $n \in S$ receives depends on players' strategies as mentioned earlier. 



%\begin{remark}
%	The characteristic function in Equation~\eqref{eq:payoff_function} is for the grand coalition $\mathcal{N}$. For any $S \subseteq \mathcal{N}$, the characteristic function will be 
%\end{remark}

%\begin{figure*}[!t]
%	\normalsize
%\begin{align} \label{eq:payoff_s_function}
%v({S})=\sum_{\substack{\text{$n \in {S}$} \\ \text{$C_{k}= \sum_{n \in {S}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {S}$}\\ \text{$\sum_{j \in {S}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S}$}}} \bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in S,j\neq n} u^{n}_j(\mathcal{X})\bigg)
%\end{align}
%	\hrulefill
%	\vspace*{-4pt}
%\end{figure*}


\begin{theorem}
%	A Cooperative game $(\mathcal{N}, v)$ of $\mathcal{N}$ players and $v$ payoff function that can be used to solve the multi-objective optimization problem given in \eqref{eq:opt_higher}, is canonical\footnote{for monotonically non-decreasing utilities/pay-off function} with Transferable utility
Resource allocation and sharing problem (with multiple objectives) for the aforementioned system model  can be modeled as a canonical cooperative game with NTU. 
\end{theorem}
\begin{proof}
To prove this, we need to show that the characteristic function of resource sharing and allocation problem satisfies the following two conditions:
%	For a game to be canonical, we need to prove that the game  is superadditive and the payoff function is of characteristic form. 
	\begin{itemize}
		\item \textbf{Characteristic form of payoff:} As the utility function in a resource sharing and allocation problem  only relies on the service providers that are part of the coalition, the game or payoff function is of characteristic form.
		\item \textbf{Superadditivity:} %Super-additivity for TU games requires $v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset$ i.e. we have to prove that the pay-off or utility for a domain in the coalition is as good as domain working alone or in a smaller coalition. 
	%	Let $u_n(X_{SO}^{(n)})$ be the utility a player $n$ earns by allocating resources to application when it is not in a coalition with any other game player. Let $U_n(X)$\footnote{$U_n(X)=w_nu_n({X}_{i \in \mathcal{M}_n}^{(n)})+\zeta_{n} \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})$} be the utility a player earns when it is part of a larger  coalition. Due to monotonicity property of the utility functions used,  for all  players $n \in \mathcal{N}$,  $u_n(X_{SO}^{(n)})\leq u_n({X})$ as $X_{SO}^{(n)}\subset {X}$. Hence, the game is superadditive.  %This is {because $X_n^{C}$ can contain much more elements due to the increase in $C$ in the coalition} where $X_n^{C}$ and $X_n^{NC}$ are the allocation decisions in  a cooperative game  and independent setting respectively for domain $n$. 
	For any $S_1, S_2 \subseteq \mathcal{N}$ where $S_1 \cap S_2 =\emptyset$, $S_1,\; S_2 \subset (S_1 \cup S_2)$. The proof follows from definition of monotone utilities.
	%Let $S_1, S_2 \subseteq \mathcal{N}$ and $S_1 \cap S_2 =\emptyset$. Hence, $S_1,\; S_2 \subset (S_1 \cup S_2)$. The proof follows from definition of monotone utilities. 
%	\begin{equation}\label{eq:super}
%	\centering 
%	v(S_1 \cup S_2) \geq v(S_1)+v(S_2)
%	\end{equation}
	
	\end{itemize}
\end{proof}
%\vspace{-0.3in}
\begin{definition}[Convex Games]
	A coalition game is said to be convex if and only if for every player $n \in \mathcal{N}$, the marginal contribution of the player is non-decreasing W.R.T set inclusion. Mathematically, for $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash \{n\}$ 
	\begin{equation}\label{eq:convexgames}
	v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2).
	\end{equation} 
\end{definition}
%\vspace{-0.2in}
\begin{theorem}\label{thm:convex}
	Our canonical game is convex. 
\end{theorem}
\begin{proof}
	Let us consider two coalition $S_1$ and $S_2$, where $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash\{j\}$, $j \in \mathcal{N}$, and  $\mathcal{F}_{S1}$ and $\mathcal{F}_{S2}$ are the feasible sets for $S_1$ and $S_2$ respectively. We calculate $v(S_2 \cup \{j\})-v(S_1 \cup \{j\})$ in Equation \eqref{eq:convexityProof}, where $u_j^{(S_1)}$ and $u_j^{(S_2)}$ are the utilities of player $j$ in $S_1$ and $S_2$ respectively.  
	
	\begin{figure*}[!t]
		\normalsize
		\begin{align}\label{eq:convexityProof}
		& \sum_{\substack{\text{$n \in {S_2}$},\\ \text{$\mathcal{X} \in \mathcal{F}_{S2}$}}}
		\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{\substack{k \in {S_2}\cup j,\\ k\neq n}} u^{n}_k(\mathcal{X})+ \sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {{S}_2}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{\substack{n \in S_2,\\ n \neq j}} u^{j}_{n}(\mathcal{X})+\sum_{i \in \mathcal{M}_j}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {{S}_2}}x_{ik}^{(l)}}{r_{ik}^{(j)}} - \nonumber \\ 
	&	\Bigg(\sum_{\substack{\text{$n \in {S_1}$},\\ \text{$\mathcal{X} \in \mathcal{F}_{S1}$}}}
		\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{\substack{k \in {S_1}\cup j , \\k \neq n}} u^{n}_k(\mathcal{X})+\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {{S}_1}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg) + 
		  w_j u_j ^{(S_1)}(\mathcal{X}) + \zeta_j\sum_{\substack{n \in S_1,\\ n \neq j}} u^{j}_{n}(\mathcal{X})+ \sum_{i \in \mathcal{M}_j}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {{S}_1}}x_{ik}^{(l)}}{r_{ik}^{(j)}}\nonumber \Bigg)\\ 
		&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$},\\ \text{$\mathcal{X} \in \mathcal{F}_{S2}\backslash\mathcal{F}_{S1}$}}}
		\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{\substack{k \in {\{S_2 \backslash S_1\}},\\ k \neq n}} u^{n}_k(\mathcal{X})+\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {\{S_2\backslash S_1\}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}    \bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) 
		+ \zeta_j\sum_{\substack{n \in S_2,\\ n \neq j}} u^{j}_{n}(\mathcal{X}) - w_j u_j ^{(S_1)}(\mathcal{X}) -  \nonumber \\
		& \quad \zeta_j\sum_{\substack{n \in S_1, \\ n \neq j}} u^{j}_{n}(\mathcal{X})+\sum_{i \in \mathcal{M}_j}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \{S_2\backslash S_1\}}x_{ik}^{(l)}}{r_{ik}^{(j)}}\nonumber \\%-\sum_{i \in \mathcal{M}_j}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in {{S}_1}}x_{ik}^{(l)}}{r_{ik}^{(j)}} \nonumber \\
		& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{\substack{n \in S_2,\\ n \neq j}} u^{j}_{n}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{\substack{n \in S_1,\\ n \neq j}} u^{j}_{n}(\mathcal{X})+\sum_{i \in \mathcal{M}_j}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \{S_2\backslash S_1\}}x_{ik}^{(l)}}{r_{ik}^{(j)}}  \nonumber \\
		& \geq v(S_2)- v(S_1)
		\end{align}
		\hrulefill
	%	\vspace*{-9pt}
	\vspace{-0.3in}
	\end{figure*}
	
	
	The last inequality in \eqref{eq:convexityProof} follows from the fact that $ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\geq 0$ (monotonicity of the utility).
\end{proof}

\begin{remark}
	The core of any convex game $(\mathcal{N},\mathcal{V})$ is non-empty and large \cite{sharkey1982cooperative}. 
\end{remark}

\begin{lemma}\label{lemma:MOOGame}
	Our canonical cooperative game $(\mathcal{N}, \mathcal{V})$ with NTU can be used to obtain the Pareto-optimal solutions for the multi-objective optimization problem given in \eqref{eq:opt_higher}.
\end{lemma}


While the existence of core, i.e., core being non-empty, guarantees the grand coalition is stable, finding a suitable allocation from the core is challenging particularly when the core is large (our game). Algorithm \ref{algo:alg1} provides an allocation from the core\footnote{Provided that the aforementioned assumptions hold.}, which we prove below after briefly discussing the algorithm. We first solve the single objective optimization problem \eqref{eq:opt_single} for all players $n \in \mathcal{N}$. We then solve the problem in \eqref{eq:opt_higher2} that provides the allocation from the core. $v(\{n\})$ in \eqref{eq:objh2} is the payoff a player $n$ receives when working alone.  Algorithm \ref{algo:alg1} requires solving $|\mathcal{{N}}|+1$ optimization problems. 


\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0%,  $ \boldsymbol{v} \leftarrow$0, $ \boldsymbol{O_2} \leftarrow$0, 
		\State \textbf{Step $2$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {v(\{n\})}\leftarrow$\texttt{Optimal objective function value in  \eqref{eq:opt_single}} 
	%		\State $ {X_{SO}^n}\leftarrow$\texttt{Optimal allocation decision from  \eqref{eq:opt_single}} 
		\EndFor
		\State \textbf{Step $3$:}   $ {\mathcal{X}}\leftarrow$\texttt{Optimal allocation decision  from  \eqref{eq:opt_higher2}} \\\quad \quad \quad \quad
		$ {\mathbf{u}(\mathcal{X})}\leftarrow$\texttt{Payoff vector from  \eqref{eq:opt_higher2}} %Solve \eqref{eq:opt_higher2}  to obtain ${X}^n$ and $v_n(\mathcal{{N}}), \forall n \in \mathcal{{N}}$       % Update $C$ and $R$ based on Step 2 \\  $\quad \quad \quad \;  C'\leftarrow$ $C_{updated}$,$\; R'\leftarrow$ $R_{updated}$
	%	\State \textbf{Step $4$:} Divide the players into two subsets $\mathcal{S}_1$ and $\mathcal{S}_2$ representing players \\ with resource deficit and resource surplus
	%	\State \textbf{Step $5$:}
	%	\For{\texttt{$n \in \mathcal{S}_1$}}
	%	\State $ {O_2^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single_j}}
	%	\State Update $C'$ and $R',\quad$ $ C'\leftarrow$ $C'$,$\; R'\leftarrow$ $R'$
	%	\EndFor
	%	\State \textbf{Step $6$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
	%	\State \textbf{Step $7$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{Game-theoretic Pareto optimal allocation }
	\label{algo:alg1}
	%\vspace{-0.5in}
\end{algorithm}

 \begin{theorem}\label{thm:alg1fromcore}
	The allocation decision obtained using Algorithm \ref{algo:alg1} lies in the core. 
\end{theorem}
\begin{proof}
	To prove the theorem, we need to show that the allocation decision obtained using Algorithm \ref{algo:alg1}:  a) is individually rational; b) is group rational; and c) no players  have the incentive to leave the grand coalition and form another sub-coalition $S \subset \mathcal{N}$. %	\indent
	\newline \indent\textbf{Individual Rationality:} For each player $n \in \mathcal{N}$, the solution obtained using \eqref{eq:opt_higher2} is individual rational due to the constraint in \eqref{eq:objh2}. 
	%	the solution $O_1^n$ obtained by solving the optimization problem in Equation \eqref{eq:opt_single} is the utility a player will obtain by working alone, i.e., it is $v\{n\}$. The value $O_2^n$ in Step 4 is either zero or positive but cannot be negative due to the nature of utility used, i.e., 
	%	\begin{align}
	%	u_n(R,\mathcal{X})&=O_1^n+O_2^n \quad \forall n \in \mathcal{N} \nonumber \\
	%	u_n(R,\mathcal{X})&\geq O_1^n \quad \forall n \in \mathcal{N}\nonumber 
	%	\end{align}
	Hence the solution obtained as a result of Algorithm \ref{algo:alg1} is individually rational.
	\newline \indent\textbf{Group Rationality:} The value of the grand coalition $v\{\mathcal{N}\}$ as per Equation \eqref{eq:objh1} is the sum of utilities of all players that they achieve from the pay-off vector  $\mathcal{V}(\mathcal{N})\subseteq \mathbb{R}^{|\mathcal{N}|}$. Hence the allocation obtained from Algorithm \ref{algo:alg1} is group rational.  %Steps 2, 4 and 5 of Algorithm \ref{algo:alg2} obtain the sum of the utilities as well. Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is group rational rational. 
	\par Furthermore, due to super-additivity of the game and monotonic non-decreasing nature of the utilities, no subgroup of players have an incentive to form a smaller coalition. Hence Algorithm \ref{algo:alg1} provides a solution from the core.  
\end{proof}

\begin{subequations}\label{eq:opt_higher2}
	\begin{align}
	\max_{\mathcal{X}}\quad& \sum_{n \in \mathcal{{N}}} \bigg(w_nu_n({X}_{i \in \mathcal{M}_n}^{(n)})+\zeta_{n} \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})+\nonumber \\
	&\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \mathcal{{N}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg),\label{eq:objh1}\\ 
	\text{s.t.}\quad & \texttt{constraints in \eqref{eq:obj1}-\eqref{eq:obj3}},  \nonumber \\
& \bigg(w_nu_n({X}_{i \in \mathcal{M}_n}^{(n)})+\zeta_{n} \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})+\nonumber \\
&\sum_{i \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\frac{\sum_{l \in \mathcal{{N}}}x_{ik}^{(l)}}{r_{ik}^{(n)}}\bigg) \geq  {v(\{n\})}, \forall n \in \mathcal{N}\label{eq:objh2}. 
%&   \texttt{ \eqref{eq:objh1} $\geq$  \eqref{eq:objsingle}}, \forall n \in \mathcal{N}.
	\end{align}
\end{subequations}


 

In the next section, we evaluate the performance of our resource sharing and allocation framework. 


==> strategy-2 arxiv/04-exp-results.tex <==
%\begin{figure*}[h!]
	%	\centering
%	\includegraphics[width=1.2\textwidth]{figures/1.eps}	\vspace{-0.5in}
%	\caption{Performance of our framework with Algorithm \ref{algo:alg2} for various $3$ player-application settings.}% and $\mu=0.01$.  }
%	\protect\label{fig:sat01}
%	\vspace{-0.1in}
%\end{figure*}






We evaluate the performance of  proposed  resource sharing and allocation framework for  several parameter settings as shown in Table \ref{tab:settings}, where $\mathcal{{G}}_1$ and $\mathcal{{G}}_2$ represent the set of service providers with resource deficits and surpluses respectively. 
Each player has three different types of resources ($K=3$), i.e., storage, communication and computation. Without loss of generality, the model can be extended to include other types of resources. 
We use linear and sigmoidal utilities for all the players given below. %(see ~\eqref{eq:ut1}) for all  players. %However, the results  hold for any monotone non-decreasing utility.
\begin{align}\label{eq:utlinear}
u_n^j({x}_{n,k}^j)=a{x}_{n,k}^j+c
\end{align}
\begin{align}\label{eq:ut1}
u_n^j({x}_{n,k}^j)=\frac{1}{1+e^{-\mu(x_{n,k}^{j}-r^{j}_{n,k})}} %\quad \forall n \in \mathcal{N}. 
\end{align}
$\mu$ is chosen to be $0.01$ whereas the constants $a$ and $c$ were randomly generated. %  to capture the requirements of different applications. 
%either $0.01$  or $0.1$ to capture the requirements of different applications. 
Requests $R_{n}$ and capacities $C_{n}, \forall n \in \mathcal{N}$ are randomly generated for each setting within a pre-specified range. %\footnote{The larger the number of applications in the simulation settings, the larger is range for random number generation.}. 
To show the advantage of resource sharing, we allocate larger capacities to certain players that   share  available resources with other domains and assist other players in meeting demand in order to increase their utilities.   


\begin{table}[]
	\centering
	\caption{Simulation network settings.}
	\begin{tabular}{|l|l|l|l|}
		\hline
		\textbf{Setting}   & \bf{Parameters} & \textbf{$\mathcal{G}_1$}& \textbf{$\mathcal{G}_2$} \\ \hline
		\textbf{1} & $N=3, M_n=3,\forall n \in \mathcal{N}$   & \{1\}&  \{2, 3\}               \\ \hline
		\textbf{2} & $N=3, M_n=20,\forall n \in \mathcal{N}$     & \{1\}&    \{2, 3\}           \\ \hline
		\textbf{3} & $N=6, M_n=6,\forall n \in \mathcal{N}$         &\{1, 2, 3\}  &   \{4, 5, 6\}         \\ \hline
		\textbf{4} & $N=6, M_n=20,\forall n \in \mathcal{N}$           &\{1, 2, 5\} &     \{3, 4, 6\}   \\ \hline
	\end{tabular}
%	\vspace{-0.1in}
	\label{tab:settings}
\end{table}
\begin{comment}
\begin{figure*}
	\centering
	\includegraphics[width=1.0\textwidth]{figures/sat_all_01.eps}
	\caption{Improvement in user request satisfaction for various player-application settings.}% and $\mu=0.01$.  }
	\protect\label{fig:sat01}
	%	\vspace{-0.1in}
\end{figure*}
\end{comment}
  \begin{figure*}[h!]
	\centering
	\includegraphics[width=1.2\textwidth]{six6}%	\vspace{-0.5in}
	\caption{Performance of our framework with Algorithm \ref{algo:alg2} for  $6$ player - $6$ application settings.}% and $\mu=0.01$.  }
	\protect\label{fig:sat13}
	\vspace{-0.1in}
\end{figure*}


\begin{figure*}[h!]
	\centering
	\includegraphics[width=1.2\textwidth]{six20}%	\vspace{-0.5in}
	\caption{Performance of our framework with Algorithm \ref{algo:alg2} for  $6$ player - $20$ application settings.}% and $\mu=0.01$.  }
	\protect\label{fig:sat14}
	\vspace{-0.1in}
\end{figure*}
Simulations were run in \texttt{Matlab R2019b} on a \texttt{Core-i7} processor with \texttt{16 GB RAM}. To solve the optimization problems, we used the \texttt{OPTI-toolbox}\cite{currie2012opti}. Below, we provide detailed experimental results for both algorithms. 
\subsection{Results for Algorithm \ref{algo:alg2}}
%\subsection{Results for strategy 1}
\subsubsection{Verification of game-theoretic properties}%\vspace{-.05in}
In Table \ref{tab:coalition}, we present results  for a 3-player 20-application game that verify different game theoretic properties  such as individually rationality, group rationality,  super additivity and show that the obtained allocation lies in the core. Player $1$ has a resource deficit while players $2$ and $3$ have  resource surpluses. 
 The payoffs all players receive in the grand coalition  are at least as good as they would receive working alone. This shows that the solution obtained using Algorithm \ref{algo:alg2} for the grand coalition is individually rational. Similarly, the value of coalition is the sum of payoff all players receive, hence our solution is group rational. Furthermore, as the coalition size increases, coalition value  increases. Hence, the grand coalition has the largest value, which shows the super additive nature of the game. Also,  no set of players has any incentive to divert from the grand coalition and form a smaller coalition. Hence, the grand coalition is stable and the allocation we obtain using Algorithm \ref{algo:alg2} lies in the core. There are two different results for the grand coalition, i.e., $GC^1$ or  $\{1, 2, 3\}$ and $GC^2$ or $\{1, 3, 2\}$ which shows that  changing the order of \texttt{for-loop}  in Step $5$ of Algorithm \ref{algo:alg2} only changes the utility achieved by players in $\mathcal{{G}}_2$. However, btoh  allocations   lie in the  core.  %    However, the value of the coalition remains the same in both cases. This shows that both the solutions are from the core.  
 Similar results are seen for other settings given in Table \ref{tab:settings}, and hence are omitted here due to space constraints.  For $\{1, 2, 3\}$, player $2$ precedes player $3$ in Step $5$ (of Algorithm \ref{algo:alg2}) while player $3$ precedes player $2$ in Step $5$ for the grand coalition in $\{1, 3, 2\}$. From the results, it is evident that having  player $2$ execute Step $5$ in Algorithm \ref{algo:alg2} before player $3$ is preferable to the order player $3$ before player $2$. % in the \texttt{for-loop} of Step $5$ of Algorithm \ref{algo:alg2} is the best order for the \texttt{for-loop}. 
 However, it is impossible to know that in advance and we need to try all possible combinations. 

 
 \begin{comment}
\begin{figure*}[h!]
	%	\centering
	\includegraphics[width=1.2\textwidth]{figures/2.eps}
	\caption{Performance of our framework with Algorithm \ref{algo:alg2} for various $6$ player-application setting.}% and $\mu=0.01$.  }
	\protect\label{fig:sat02}
	\vspace{-0.1in}
\end{figure*}
\end{comment}
\begin{table}[]
	\caption{Player payoff in different coalitions for a $3$ player - $20$ application game}
	\begin{tabular}{|l|l|l|l|l|}
		\hline
		\textbf{Coalition}       & \textbf{Player 1} & \textbf{Player 2} & \textbf{Player 3} & \textbf{Value of coalition}  \\ \hline
		\textbf{\{1\}}               & 108.74           & 0.00              & 0.00              & 108.74                 \\ \hline
		\textbf{\{2\}}               & 0             & 120            & 0              & 120                   \\ \hline
		\textbf{\{3\}}               & 0              & 0              & 120             & 120                   \\ \hline
		\textbf{\{1, 2\}}              & 111.51
		         & 131.01         & 0              & 242.52                \\ \hline
		\textbf{\{1, 3\}}              & 112.04           & 0              & 130.75            & 242.79               \\ \hline
		\textbf{\{2, 3\}}              & 0              & 120          & 120           & 240                 \\ \hline
		\textbf{\{1, 2, 3\}$^{1}$} & 114.39       & 131.01             &   122.75        & 368.15            \\ \hline
		\textbf{\{1, 3, 2\}$^{2}$} & 114.39       & 120            & 130.75           & 365.14            \\ \hline
	\end{tabular}
	\label{tab:coalition}
	%	\vspace{-0.35in}
\end{table}

\subsubsection{Efficacy of the resource sharing framework}
Figures \ref{fig:sat11} and \ref{fig:sat12} show the efficacy of our resource sharing framework using Algorithm \ref{algo:alg2} and compare it with a setting in which the MECs are working alone for the 3 players and different application settings given in Table \ref{tab:settings}. We evaluate the impact of the proposed framework on MEC utility, request satisfaction, and resource utilization. It is evident that MECs with resource deficits are able to improve their application satisfaction and utilities (due to increase in application satisfaction) whereas MECs with resource surpluses improve their utilities by sharing their resources, which in turn increases  resource utilization.
For $GC^1$ results in the 6 player-6 application setting, player 4 and 5 precede player 6 in Step $5$ of Algorithm \ref{algo:alg2} whereas in $GC^2$, player 6 precedes players $4$ and $5$. For $GC^1$ results in the $6$ player-20 application setting, players 3 and 4 precede player 6 whereas in $GC^2$, player $6$ precedes players 3 and 4  in step 5 of Algorithm \ref{algo:alg2}. The utility function distributions among players vary for $GC^1$ and $GC^2$, however, both allocations are in the core and are Pareto optimal.  Figures \ref{fig:sat13} and \ref{fig:sat14} show the performance of Algorithm 1 in the 6 player, 6 and 20 application settings, respectively. It is evident from the results that resource sharing improves utility of MECs with resource surplus and user satisfaction of resource deficit MECs. 

%\begin{comment}

%\end{comment}

\begin{figure*}
	%	\centering
	\includegraphics[width=1.2\textwidth]{matching}
	\caption{Performance of our framework with Algorithm \ref{algo:algPoly} for $6$ player-$6$ application settings.}% and $\mu=0.01$.  }
	\protect\label{fig:sat03}
	\vspace{-0.1in}
\end{figure*}
\begin{figure}
	%	\centering
	\includegraphics[width=0.95\textwidth]{frag}
	\caption{Resource fragmentation for Algorithms \ref{algo:alg2} and \ref{algo:algPoly} in 6 player-6 application setting.}% and $\mu=0.01$.  }
	\protect\label{fig:sat04}
	\vspace{-0.1in}
\end{figure}

\begin{comment}

\paragraph{Player utilities}
Figure \ref{fig:util_all} shows the utilities of game players in different simulation settings. It is evident from the figure that  utilities of players in grand coalition (GC), with two different ways of running the \emph{for-loop} in Step $5$ of Algorithm \ref{algo:alg2}, and all simulation settings  drastically improve using our game theoretic algorithms. This shows that   service providers can greatly benefit by employing a resource sharing scheme.  However, it is worth mentioning that the improvement greatly depends on parameters such as resource surplus, deficit, and utilities. For the 3-player games, $GC^1$ ($\{1, 2, 3\}$) represents the scenario where player $2$ preceded player $3$ in Step $5$ of Algorithm \ref{algo:alg2},   whereas $GC^2$ ($\{1, 3, 2\}$) represents the scenario where player $3$ preceded player $2$ in Step $5$. The utilities of players $2$ and $3$ improve in the grand coalition as they share their resources with player $1$, while player $1$'s utility improves due to the increase in its application satisfaction.
 % $GC^1$  %For the $3$-player game with $3$ and $20$ applications, players $2$ and $3$ have a resource surplus while player $1$ has resource deficit. 
 For the $6$-player game with $6$ and $20$ applications, we see that players with resource surplus improve their utilities in the grand coalition when compared with working alone by sharing their resources with players with resource deficits. For the $6$-player game with $6$ applications per player, the \emph{for-loop} order in $GC^1$ is $\{6, 4, 5\}$ %as follows: player $6 \longrightarrow 4 \longrightarrow 5$ 
 whereas the order for $GC^2$ is $\{4, 5, 6\}$. % $4 \longrightarrow 5 \longrightarrow 6$.
  For the $6$-player game with $20$ applications per player, the \emph{for-loop} order in $GC^1$ is $\{6, 4, 3\}$ %%as follows: player $6 \longrightarrow 4 \longrightarrow 3$ 
  whereas the order for $GC^2$ is $\{4, 3, 6\}$. % $4 \longrightarrow 3 \longrightarrow 6$.
  Players with resource deficit benefited from the coalition by increasing its user satisfaction. For all the experiments,  we see that in $GC^1$ and $GC^2$, the utilities that players with resource surpluses receive are different in both schemes. However, as shown earlier, the value of  the coalition remains same. 




\paragraph{User satisfaction}
Satisfying user requests is important for edge service providers as it is mandated by the SLA. Furthermore, it helps in retaining their users (customers) resulting in long-term profits. Figure \ref{fig:sat01} shows the average user request satisfaction in different player-application settings. It is evident from the figure that all  edge service providers with resource deficits exhibit a low user satisfactions. However, once the edge service providers in $\mathcal{{G}}_1$ join the coalition, their user satisfactions improve as edge providers in $\mathcal{{G}}_2$ share their excess resources with edge service providers with resource deficits. Request satisfaction in the grand coalition is 100\% for all  edge service providers  in our simulations. It is worth mentioning that the amount of improvement in user satisfaction depends on the capacity of edge service providers  in $\mathcal{{G}}_2$ and the requests of users belong to service providers in $\mathcal{{G}}_1$. We also only show the request satisfaction for $GC^1$ ($\{6, 4, 3\}$) since the user satisfaction rate for both $GC^1$ and $GC^2$ in our simulation are the same, i.e., 100\% for all service providers. % For a $3-$ player game with $3$ and $20$ applications respectively, player $1$ has a resource deficit and is not able to satisfy all of its user's request when operating alone. Players $2$ and $3$ have a resource surplus so they can satisfy their users even working alone. When all the three players work in a coalition, the request satisfaction for all three players is 100\%. Similarly, for a $6-$player game with $6$ and $20$ applications respectively, we see that players who could not satisfy their applications alone are able to satisfy all their user requests by joining the coalition and ``renting" resources from the players that have a resource surplus. It is worth mentioning that resource sharing can drastically improve user satisfaction. However, the extent of improvement depends on the nature of the utility function. 


\paragraph{Resource utilization}
Figure \ref{fig:ut01} shows the resource utilizations of different players in various simulation settings.  For all player-application settings, it is evident that  resource utilizations for players in $\mathcal{{G}}_2$ increase in the grand coalition when compared with working alone as it rents its resources to players in $\mathcal{{G}}_1$. However, the resource utilization in the grand coalition varies for $\mathcal{{G}}_2$  service providers in  $GC^1$ and $GC^2$ due to aforementioned order of  $\emph{for-loop}$ in Step $5$ of Algorithm \ref{algo:alg2}. 

%For a $3-$player game with $3$ and $20$ applications respectively, we see that the resource utilization for player $2$ and $3$ (players with resource surplus)  increases in the grand coalition when compared with working alone. This is because these players rent out their resources to other players that may need them resulting in an increased utility. Player $1$ with resource deficit had 100\% resource utilization rate working alone. However, resource utilization for player $1$ in grand coalition either may remain the same or reduce, since its users' requests may be satisfied by other players. Similar results are seen for a $6-$player game with $6$ and $20$ applications  as evident from the figure. 

\begin{figure*}
	%\centering
	\includegraphics[width=1.0\textwidth]{figures/ut_all_01.eps}
	\caption{Resource utilization for various player-application settings.}% and $\mu=0.01$.  }
	\protect\label{fig:ut01}
	%	\vspace{-0.1in}
\end{figure*}



%\subsection{Results for strategy 2}



\par It is evident from our results that  resource sharing and allocation is beneficial for cloud service providers. By allowing different cloud service providers to cooperate, the utility of  service providers increases and resources are utilized in an optimal manner. All the  service providers in
 the game have the incentive to work together and use their resource capacities in the best possible way. 
\end{comment}

\subsection{Results for Algorithm \ref{algo:algPoly}}
Figure \ref{fig:sat03} presents the results for Algorithm \ref{algo:algPoly}. It is evident that Algorithm \ref{algo:algPoly} improves the utilities and application satisfaction of different MECs (compared with MECs working alone). To highlight the decrease in resource fragmentation due to  Algorithm \ref{algo:algPoly}, we compare it with Algorithm \ref{algo:alg2}.  Figure \ref{fig:sat04} shows the percentage of resources allocated to applications of different MECs in $\mathcal{{G}}_1$ by MECs in $\mathcal{{G}}_2$ using Algorithms \ref{algo:alg2} and \ref{algo:algPoly}.  
 Using Algorithm \ref{algo:alg2} for resource sharing in the 6 player 6 application setting ($GC^1$),
applications of MEC 1 are allocated resources at MEC 4 and 6, whereas applications of both MEC 2 and MEC 3 receive resources from MECs 4, 5, 6. 
 %MEC 4 provides resources to  applications of MEC 1, 2 and 3, whereas applications of MEC 3 are provided resources by MEC 4 and 5. 
%Resources to  applications of MEC 2 are provided by MEC 4, 5 and 6. 
%This indicates that resources provided to applications of MECs in $\mathcal{{G}}_1$ are fragmented.
 For the same setting and using Algorithm \ref{algo:algPoly}, resources to applications of MEC 1 are provided by MEC 4  and 6. Resources to applications of MEC 2 and 3 are provided by MEC 4 and 5, respectively. 
%whereas MEC 5 provides resources to  applications of MEC 3.  Resources to applications of MEC 2 are provided by MEC 4 and 6. 
This shows that resources fragmentation significantly reduces by Algorithm \ref{algo:algPoly} when compared with Algorithm \ref{algo:alg2} at the cost of added computational complexity.

%\begin{comment}

%\end{comment} 

The experimental results show that the proposed resource sharing framework can benefit MECs.  While Algorithm \ref{algo:alg2} is computationally more efficient,  it may result in comparatively larger resource fragmentation. On the other hand, Algorithm \ref{algo:algPoly}  reduces resource fragmentation  at the cost of computational complexity.  



==> strategy-2 arxiv/05-conclusions.tex <==
%Resource allocation and sharing is a fundamental research problem particularly after the advent of IoT, MTC and Big Data. In this paper, we proposed a cooperative game theory based generic resource allocation and sharing framework that guarantees stability and fairness to the resource providers. We showed that any multi-objective resource allocation and sharing problem can be solved to Pareto-optimality by using concepts of \emph{core} and Shapley value from CGT. Through experimental results, we showed that resource sharing among resource providers can provide higher gains and satisfy a higher number of jobs or applications that ask for resources.
In this paper, we have proposed a cooperative game theory based resource sharing and allocation framework for edge clouds. We showed that for  monotonic, non-decreasing and non-negative positive utilities, resource sharing  among edge clouds can be modeled as a cardinally convex canonical  game. We have proved that the core exists and proposed  two efficient  algorithms that  provide allocation from the core. Hence, the obtained solutions are Pareto optimal and the grand coalition of the edge service providers is stable. Furthermore, we have reduced resource fragmentation using the matching based algorithm that also provides an allocation in the core. 
Experimental results show that  utilities of all service providers and   user satisfaction are improved,  when compared with  edge clouds working alone, using our framework. 


 %and the Shapley value lies inside the core, which is why we used Shapley value to obtain Pareto optimal and fair allocations. For the special case where each service provider allocates resources to its own users and then allocates the remaining resources to the users of other service providers, we proposed a $\mathcal{O}(N) $ algorithm that provides allocation decision from the core. Simulation results showed that our proposed framework improves utility obtained by cloud service providers in both the general and special case. 



==> strategy-2 arxiv/preli.tex <==
%In this section, we present a discussion of Multi-Objective Optimization (MOO), cooperative game theory, and the core. % as they are used later in the paper.
In this section, we give a brief overview of Multi-Objective Optimization (MOO), cooperative game theory, and the core.


\subsection{Multi-Objective Optimization}
 Multi-Objective Optimization (MOO) identifies a vector $\boldsymbol{x}^*=[x_1^*,x_2^*,\cdots ,x_t^*]^T$ that optimizes a vector function
	\begin{equation}\label{eq:vectorobjective}
	\centering 
	\bar{f}(\boldsymbol{x})=[f_1(\boldsymbol{x}),f_2(\boldsymbol{x}),\cdots,f_N(\boldsymbol{x})]^T
	\end{equation}
	such that 
	\begin{align}\label{eq:constraints}
	\centering 
	& g_i(\boldsymbol{x})\geq 0, \; i=1,2,\cdots,m, \\
	&h_i(\boldsymbol{x})=0\;\; i=1,2,\cdots,p. \nonumber
	\end{align}
	where $\boldsymbol{x}=[x_1,x_2,\cdots ,x_t]^T$ is a vector of $t$ decision variables and the feasible set is denoted by $F$.
The fundamental difference between a single objective optimization (SOO) and MOO is that MOO involves a vector of objective functions rather than a single objective function. Hence, the resulting solution is not a single point, but 
 a \emph{frontier} of solutions known as \emph{Pareto frontier} or \emph{Pareto boundary} (see \cite{cho2017survey} for details). Some basic definitions related to MOO are: 
 \begin{comment}
\begin{definition}{Strongly Pareto non-dominated solution:}
%	\small
	A feasible solution $x$, for a minimization problem, is strongly Pareto non-dominated, if there is no $y\in F$ such that $f_n(\boldsymbol{y})\leq f_n(\boldsymbol{x})$ $\forall n=1,2,\cdots,N$ and $f_n(\boldsymbol{y})<f_n(\boldsymbol{x})$ for at least one $n$ \footnote{Means that there is no other feasible solution that can improve some objectives without degrading at least one other objective.}.
\end{definition}
\begin{definition}{Weakly Pareto non-dominated solution:}
%	\small
	A feasible solution $x$, for a minimization problem, is weakly Pareto non-dominated, if there is no $y\in F$ such that $f_n(\boldsymbol{y})<f_n(\boldsymbol{x})$ $\forall n=1,2,\cdots,N.$
\end{definition}
\end{comment}
%\begin{definition}{Pareto Efficiency/Optimality:}
%	A state in which resources cannot be reallocated to make any individual gain more without hurting any other objective. 
%\end{definition}
\begin{definition}{Pareto Improvement or Pareto Dominated Solution:}
	Given an initial allocation, if we can achieve a different 	allocation that improves at least one individual function  without degrading any other, then the initial allocation is called \emph{Pareto improvement}.
\end{definition}


\begin{definition}{Pareto Optimality:}
	For any minimization problem,  $\boldsymbol{x}^*$ is $Pareto\; Optimal$ if the following holds for every $\boldsymbol{x} \in F$,
	\begin{align}\label{eq:paretoptimality}
	\bar{f}(\boldsymbol{x}^*)\leq\bar{f}(\boldsymbol{x}). 
	\end{align}
	where %$\bar{f}(\boldsymbol{x})=[f_1(\boldsymbol{x}),f_2(\boldsymbol{x}),\cdots,f_N(\boldsymbol{x})]^T$ and  
	$\bar{f}(\boldsymbol{x}^*)=[f_1(\boldsymbol{x}^*),f_2(\boldsymbol{x}^*),\cdots,f_N(\boldsymbol{x}^*)]^T$.
\end{definition}
 \begin{comment}
\begin{definition}{Strong Pareto Optimality:}
	A feasible solution $x$ is strongly Pareto optimal, if it is strongly Pareto non-dominated. 
\end{definition}
\begin{definition}{Weak Pareto Optimality:}
	A feasible solution $x$ is weakly Pareto optimal, if it is weakly Pareto  non-dominated. 
\end{definition}
\end{comment}

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{opt.jpg}
	\vspace{-0.20in}
\caption{MOO with two objective functions}
\protect\label{fig:pareto}
\end{figure}

Figure~\ref{fig:pareto} shows a  MOO problem with two objective functions $f_1$ and $f_2$.  The boundary $\overleftrightarrow{ab}$ is the Pareto frontier  as it consists of all the Pareto optimal solutions. 

\subsection{Cooperative Game Theory}
Cooperative game theory provides a set of analytical tools that assist in understanding the behavior of rational players in a cooperative setting \cite{han2012game}. Players can have agreements among themselves that affect  strategies as well as utilities  obtained by the game players. Coalition game, a type of cooperative game, deals with the formation of  coalitions, namely groups of two or more cooperating players. Formally,
%Cooperative games are primarily of two types: bargaining theory and coalition games. Bargaining theory deals with the bargaining processes that arise among  players when creating an agreement, while coalition games deals with the formation of  coalitions, namely groups of two or more cooperating players. Formally,

\begin{definition}{Coalition Game \cite{han2012game}:}\label{def:charac}
Any coalition game with \emph{non-transferable utility} (discussed below)  can be represented by the pair $(\mathcal{N},\mathcal{V})$ where $\mathcal{N}$ is the set of players that play the game, while $\mathcal{V}$ is a set of payoff vectors such that \cite{roger1991game}:

% the value $v$ of the game must satisfy the following properties for any coalition $S$\cite{roger1991game}.
\begin{enumerate}
	\item $\mathcal{V}(S), \forall S \subseteq \mathcal{N}$ should be a closed and convex subset of $\mathbb{R}^{|\mathcal{N}|}$.%, where $\mathcal{V}(\mathcal{{N}})$
	\item $\mathcal{V}(S)$ should be comprehensive, i.e., if we are given payoffs $\mathbf{x} \in \mathcal{V}(S)$ and $\mathbf{y} \in \mathbb{R}^{|S|}$ where $\mathbf{y}\leq \mathbf{x}$, then $\boldsymbol{y} \in \mathcal{V}(S)$. In other words, if the members of coalition $S$ can achieve a payoff allocation $\mathbf{x}$, then the players can change their strategies to achieve an allocation $\mathbf{y}$ where $\mathbf{y}\leq \mathbf{x}$. 
	\item The set $\{\mathbf{x}| \mathbf{x} \in \mathcal{V}(S) \;$ and $\; x_n \geq z_n, \forall n \in S \}$, with $z_n = \max\{y_n|\mathbf{y} \in \mathcal{V}(\{n\}) \}\le \infty \; \forall n \in \mathcal{N}$ should be a bounded subset of $\mathbb{R}^{|S|}$. In other words, the set of vectors in $\mathcal{V}(S)$ for a coalition $S$ where the coalition members receives a payoff at least as good as working alone (non-cooperatively) is a bounded set. 
\end{enumerate} 


%the characteristic (mapping) function that determines the utilities or payoffs game players in $\mathcal{N}$ receive. 
\end{definition}

\begin{definition}{Utility:}
The payoff or gain a player receives in the game is known as utility.  
\end{definition}

\begin{definition}{Value of a coalition:}
The sum of utilities of the coalition members is known as the value ${v}$ of a coalition.
%The total utility of any coalition is known as the value ${v}$ of a coalition. 
\end{definition}

\begin{definition}{Non-Transferable Utility (NTU)\cite{han2012game}:}
	If the total utility of any coalition cannot be  assigned a single real number  or if there is a rigid restriction on  utility distribution among players, then the game has a \emph{non-transferable} utility. In other words, the payoff each player receives and the value of coalition depend on the game strategy. Utility cannot be transfered freely among the players. 
	
%	in any manner among the game players, then the game has a \emph{transferable} utility. 
\end{definition}

\begin{definition}{Characteristic function:}
	The characteristic function for any coalition game with NTU is a function that assigns  a set of payoff vectors, $\mathcal{V}(S) \subseteq \mathbb{R}^{|S|}$, to game players where each element of the payoff vector $x_n$ represents a payoff that player $n \in S$ obtains  given a strategy selected by the player $n$ in the coalition $S$.   % a mapping $v: 2^{\mathcal{N}} \mapsto \mathbb{R}$ with $v(\emptyset)=0$.
%	The characteristic function for any coalition game with TU is a mapping $v: 2^{\mathcal{N}} \mapsto \mathbb{R}$ with $v(\emptyset)=0$.
\end{definition}

\begin{definition}{Characteristic Form Coalition Games \cite{han2012game}:}
	A coalition game is said to be of \emph{characteristic} form, if the value of coalition $S \subseteq \mathcal{N}$ depends only on  the members of the coalition. (This means that players that are not part of the game don't impact the value of coalition.)
\end{definition}





\begin{definition}{Superadditivity of NTU games:}
A canonical game with NTU is said to be superadditive if the following property is satisfied. 
\begin{align}\label{eq:superadditivity}
  & \{x \in \mathbb{R}^{S_1\cup S_2}|(x_n)_{n \in S_1} \in \mathcal{V}(S_1), (x_m)_{m \in S_2}\nonumber \\
& \in \mathcal{V}(S_2)   \}   \subset \mathcal{V}(S_1 \cup S_2) \;  \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, S_1 \cap S_2 =\emptyset. 
%v(S_1 \cup S_2 )\geq v(S_1)+v(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset.
\end{align}
where $x$ is a payoff allocation for the coalition  $S_1 \cup S_2$. 

\end{definition}

That is,  if any two disjoint coalitions $S_1$ and $S_2$ form a large coalition $S_1 \cup S_2$, then the coalition $S_1 \cup S_2$ can always give its members the payoff that they would have received in the disjoint coalition  $S_1$ and $S_2$. It is worth mentioning that $\mathcal{V}$ is the set of payoff vectors while ${v}$ is the sum of payoffs  for all coalition players. %that all players get in a particular payoff vector (coalition).  
%i.e., formation of large coalitions is always desired and the players do not lose any utility (when compared with working alone) by joining the coalition. 
\begin{definition}{Canonical Game:}
A coalition game is canonical if it is superadditive and in characteristic form.
\end{definition}
The \emph{core} is a  widely used concept for dealing with canonical games as discussed below. 

\subsection{Core}
To help us explain the core, we first define some terms   \cite{han2012game}.

\begin{definition}{Group Rational:}\label{def:groupRational}
	A payoff vector $\textbf{x}\in \mathbb{R}^\mathcal{N}$ for distributing the coalition value $v(\mathcal{N})$ to all players is group-rational if $\sum_{n \in \mathcal{N}}x_n=v(\mathcal{N})$.
\end{definition}

\begin{definition}{Individual Rational:}\label{def:indRational}
	A payoff vector $\textbf{x}\in \mathbb{R}^\mathcal{N}$ is individually rational if every player can obtain a payoff no less than acting alone (not in a coalition), i.e., $x_n \geq v(\{n\}), \forall n\in \mathcal{N}$.
\end{definition}

\begin{definition}{Imputation:}
	A payoff vector that is both individual and group rational is  an imputation. 
\end{definition}

\begin{definition}{Grand Coalition:}
The coalition formed by all game players $\mathcal{N}$ is the grand coalition.
\end{definition}

Based on the above definitions, we can  define the core of an NTU canonical coalition game as:

\begin{definition}{Core\cite{han2012game}:}
	For any NTU canonical game $(\mathcal{N}, \mathcal{V})$, the core $C_{NTU}$ is the set of imputations in which no coalition $S\subset\mathcal{N}$ has any incentive to reject the proposed payoff allocation and deviate from the grand coalition to form the smaller  coalition $S$ instead. Mathematically, this is 
	\begin{align}\label{eq:coreTU}
	\mathcal{C}_{NTU}&= \{ \mathbf{x} \in \mathcal{V}(\mathcal{N}) | \forall S \subset \mathcal{N}, \nexists \mathbf{y} \in \mathcal{V}(S) \; such\; that \; y_n > x_n, \nonumber \\
	&  \forall n \in S    \}.
	%\bigg \{ \mathbf{x}: \sum_{n \in \mathcal{N}}x_n=v(\mathcal{N}) \; and \; \sum_{i \in S} x_i \geq v(S)\; \forall\; S\subseteq \mathcal{N}.\bigg\}
	\end{align}
\end{definition}
\begin{remark}\label{rem:paretocore}
	Any payoff allocation from the core is Pareto-optimal as evident from definition of the core. Furthermore, the grand coalition formed is stable, i.e., no two players will have an incentive to leave the grand coalition to form a smaller coalition. 
\end{remark}
However, the core is not always guaranteed to be non-empty. If the core is non-empty, it will be a convex set \cite{shapley1971cores}, whereas a convex set consists of infinite convex combinations of the points within the set \cite{boyd2004convex}. Therefore, a non-empty core  is large and finding a payoff allocation (vector) in the core is not easy.    
\begin{definition}{User/Application Request Satisfaction:}\label{def:rs}
	The extent to which a request for resources is satisfied.  Mathematically, if $r$ is the requested amount and $x$ is the provisioned amount, then application request satisfaction is given by $x/r$. 
\end{definition}
%\begin{definition}{Local Optimality:}
%\textbf{To be added}
%\end{definition}
%\begin{definition}{Global Optimality:}
%\textbf{To be added}
%\end{definition}
%, where very large means infinite number of points.  
%Therefore, finding a payoff allocation (vector) in the core is not easy. %Furthermore,  allocation from the core may not always be fair to all the players. There exists one allocation known as the Shapley value, which exhibits desirable properties. 
%Therefore, below we describe the Shapley value, which can help address these limitations in certain cases. 


%For solving NTU canonical games using the core, the value v of the NTU game must
%satisfy the following conditions, for any coalition S



%\subsection{Shapley Value}
 %Now that we have the answer to the question about non-emptiness of the core, we divert our attention to the selection of any pay-off allocation from the core. As evident, the core for our problem is quite large. Therefore, selecting a suitable core allocation can be difficult \cite{han2012game}. 
 %\emph{Shapley value} \cite{shapley1988value} can be used to address the aforementioned  shortcomings of the core. For the characteristic function $v$ (the characteristic function is also called the game \cite{han2012game}), Shapley proposed an allocation $\phi_n(v)$ that satisfies the following axioms \cite{la2004game}:
 %\begin{enumerate}
 %	\item \emph{Efficiency Axiom}: $\sum_{n \in \mathcal{N}}\phi_n(v)=v(\mathcal{N})$. This axiom, in essence, is  group rationality.
 %	\item \emph{Symmetry Axiom}: If any two players $m$ and $n$ are such that $v(S \cup \{n\})=v(S \cup \{m\})$, then for every coalition $S\backslash(m,n)$, $\phi_n(v)=\phi_m(v)$. This axiom indicates that if any two players/domains have similar contributions in a coalition, their assigned payoffs must be the same as well.
 %	\item \emph{Dummy Axiom}: If any player $n$ is such that $v(S)=v(S \cup \{n\})$, then for every coalition $S\backslash n$, $\phi_n (v)=0$. Dummy axiom indicates that players that do not contribute to the value of coalition will not get any payoff. 
 %	\item \emph{Additivity Axiom}: If $j$ and $k$ are any two games, then $\phi(u+v)=\phi(u)+\phi(v)$. This axiom indicates that $\phi$ is a unique mapping over the space of the coalitional games.
 %\end{enumerate}
 %Based on the above axioms, Shapley  showed that there exists a unique function $\phi$ defined on all games that satisfies the aforementioned axioms \cite{la2004game}. The function is given by:
 
% \begin{equation}\label{eq:shapleyvalue}
 %\phi_n(v)=\sum_{S\subseteq \mathcal{N}\backslash n}\frac{|S|! (|\mathcal{N}|-|S|-1)!}{|\mathcal{N}|!}\bigg[ v(S \cup \{n\}) -v(S) \bigg]
 %\end{equation} 
%The above function shows the average margina

==> strategy-2 arxiv/related.tex <==




There have been a number of solutions proposed in the literature related to resource allocation in edge computing \cite{you2017energy,wang2017computation,sardellitti2015joint,xu2017zenith,he2018s,zhang2017computing,xu2018game,liu2017incentive,zafari2018game}. Xu et al. \cite{xu2017zenith} propose a novel model for allocating resources in an edge computing setting where the allocation of distributed edge resources is decoupled from service provisioning management at the service provider side. The authors develop an auction-based resource sharing contract establishment and resource allocation that maximizes the utilities of service providers and edge computing infrastructure providers.  He et al. \cite{he2018s} relax the long-held assumption that storage resources are not shareable and study the optimal allocation of both shareable and non-shareable resources in a mobile edge computing setting. The authors consider the joint problem of service placement and request scheduling, and propose constant-factor approximation algorithm as the problem is proven to be NP-hard. Liu et al. \cite{liu2017incentive}  model the interaction among cloud service operators and edge service owners as a Stackelberg game for maximizing the utilities of both cloud and edge service providers. The authors obtain the optimal payment along with the computation offloading strategies. Zhang et al. \cite{zhang2017computing} propose an optimization framework, formulated as a Stackelberg equilibrium,  for edge nodes, data service operators and service subscribers that provides optimal resource allocation in a distributed manner. Xu et al. \cite{xu2018game} propose a secure caching scheme in heterogeneous networks for multi-homed subscribers that relies on a trust mechanism for verifying the reliability of edge computing-enabled small cell base stations. The authors also propose a Chinese reminder theorem  based protocol for preserving privacy. A Stackelberg game is used to model the interaction between the mobile users and the edge cloud and the goal is to maximize  utilities of both users and service providers. 
\par Our work in this paper differs from \cite{he2018s,xu2017zenith,xu2018game,liu2017incentive,zhang2017computing} as we consider  objectives of different service providers and allow resource sharing among  edge cloud service providers.  In \cite{zafari2019game}, we consider the strategy where the players do not differentiate between their own applications and applications of other players, and propose a centralized algorithm that provides an allocation from the core. 
This work is an extension of our earlier work in  \cite{zafari2018game}, where we model the resource sharing among mobile edge clouds as a canonical cooperative game with transferable utility (TU). However, in this work, we  model the problem as an NTU game which is more generic than the TU game \cite{roger1991game}. Unlike \cite{zafari2018game}, we do not rely on Shapley value, due to high complexity for obtaining a solution. Furthermore, we have not included application  satisfaction  and resource fragmentation as part of the resource sharing game in \cite{zafari2018game}. 




